Discovery and Contextual Data Cleaning with Ontology Functional Dependencies

Functional Dependencies (FDs) define attribute relationships based on syntactic equality, and, when usedin data cleaning, they erroneously label syntactically different but semantically equivalent values as errors. We explore dependency-based data cleaning with Ontology Functional Dependencies(OFDs), which express semantic attribute relationships such as synonyms and is-a hierarchies defined by an ontology. We study the theoretical foundations for OFDs, including sound and complete axioms and a linear-time inference procedure. We then propose an algorithm for discovering OFDs (exact ones and ones that hold with some exceptions) from data that uses the axioms to prune the search space. Towards enabling OFDs as data quality rules in practice, we study the problem of finding minimal repairs to a relation and ontology with respect to a set of OFDs. We demonstrate the effectiveness of our techniques on real datasets, and show that OFDs can significantly reduce the number of false positive errors in data cleaning techniques that rely on traditional FDs.

==> Comments.tex <==
\noindent {\textbf{Lukasz's comments:}} \\

\rebut{\textbf{1.} Intro: it's not clear to me why contributions 5 and 6 are separate contributions.}

%\fei{they do sound similar so let's merge.} 
\blue{Merged and DONE.}

\rebut{\textbf{2.} Section 2.1: I agree with Comment(Fei): what is a synonym node?  I thought a node in an ontology expresses a single entity belonging to some class E, and we defined synonyms(E) as the set of synonyms of E.}


\ans{Remove the term synonym node in the paper, and describe it with synonym class synonyms(E).}
\fei{Is this done everywhere in the paper?}
\eat{\fei{You need to highlight all your changes for these comments, where is the new text in Sec. 2.1?} }

\rebut{\textbf{3.} Theorem 12 seems incorrect (each minimal repair is tau constrained).  What if we have to make at least tau+1 data edits in order to make zero ontology edits?}


\ans{We missed the definition about the value range of $\tau$ as what you did in the relative trust paper, and we added it.} 
\fei{I think Lukasz is asking a broader question here about whether this stmt. makes sense for all minimal repairs in general.  E.g., if $\tau = 2$ but a minimal repair requires 3 data edits, then your stmt. is false, in general.}
\fei{Clarify change here in the paper.}

\rebut{\textbf{4.} Section 6.1: It's not obvious to me that beam search is correct.  If we're expanding the b best nodes at any point in time, we may expand nodes with very many elements and ignore potential minimal repairs. Potential solution to the above: suppose adding A to the ontology fixes 5 tuples and adding B fixes 5 tuples.  Claim: adding A and B together fixes at least 5 and at most 10 tuples.  Is this true?  If so, can we use this observation to prioritize the search space (or perhaps use it in A* search)?}

\ans{To obtain the Pareto-optimal set of solutions for ontology repair, one approach is to exhaustively consider all possible $k$-combinations from the ontology repair candidates set, and select the solution that leads to the minimum number of data repairs for each $k$ value. However, we prove this approach has exponential complexity. Then we propose the beam search based approach, and we claim that it is a heuristic approach. You are correct, we cannot guarantee selecting top-b best nodes in each level will always lead to the minimal solution. However, in the experiments we can evaluate the trade-off between repair accuracy and running time to show the efficient of this approach.}

\ans{Firstly, it is hard to know exact how many tuples are fixed by adding a node. There is an alternative way may work, we can estimate the maximum number of necessary data modifications for zero ontology repair, denoted by $X$. Then we add a node $A$ to the ontology, and estimate the maximum number of necessary data modifications, denoted by $Y$. Then we can somehow measure the positive impact of adding $A$ to the ontology, which is $X-Y$.}

\ans{Secondly, I don think the claim is true, i.e., suppose adding A to the ontology fixes 5 tuples and adding B fixes 5 tuples, adding A and B together may fixes more than 10 tuples. For example, consider there is a set of tuples cannot be fixed by adding either A or B, but only can be fixed by adding both of them. In this case, singly adding either one can fix zero tuple, but adding them together can fix a set of tuples.}
\fei{I think Lukasz is looking for a more intelligent way to navigate the search space.  Your approach is somewhat blindly considering all the candidates and just greedily taking the top-b, but can we be more smart to filter the nodes considered?  I don't understand your last sentence, the assumption is that A or B will fix 5 tuples, so your first assumption already goes against this.}

\rebut{\textbf{5.} Is Algorithm 5 correct?  I don't see how it traverses the lattice or how Cand(S) is initially populated.}

\ans{Before we used two For-loop to traverse the lattice, which is not obvious. We revised the Algorithm 5 and included the initiation of Cand(S). }

\rebut{\textbf{6.} Section 6.2: it would be good to clarify how an FD conflict graph is different than an OFD conflict graph.  Is it more expensive to build?  Do we still get a 2-approximation if we use approximate vertex cover?}

\ans{For Q1: In the FD case, we can build the CH by checking the violations between all pairwise tuples for each FD, i.e., if two tuples violate an FD, then add an edge to connect these two tuples in the CH. In the OFD case, each equivalence class may have multiple senses. To build the CH, we have to consider all the possible sense combinations for all the equivalence classes. For example, we have two equivalence classes $eq_1$ and $eq_2$, $eq_1$ has 3 senses while $eq_2$ has 4 senses. Then we need to build $3 \times 4 = 12$ CH. Another difference is that in FD case, if there is an edge between two tuples in CH, we record the violating FD of them; while in OFD case, for each edge in the CH, we also record the potential ontology repair associate with the violating OFD. }

\fei{You need to describe this according to what each node and edge represents in the CH for each case.  Then state what is the overhead difference of OFD.  No need to give example here, state the facts, and why it's more computationally challenging, and what techniques you have done to address this overhead.  Your answer is way too long to put into the paper.  Once you select a fixed sense in your Q2, what is the difference bw an FD-based CH?}

\ans{For Q2: We cannot traverse all the senses for each equivalence class to build CH in the OFD case, since the combinations are exponential. So we propose an algorithm in Section 6.2 to select sense for each equivalence class based on the maximum coverage, and we still get a 2-approximation after selecting the sense.}

\rebut{\textbf{7.} Section 6: it would be good to state explicitly how we can re-use previous computation when producing repairs for different values of tau (see section VII of the relative trust paper with George and Ihab).}

\ans{This part we need a discussion. I have a question about the scope of our work.}
\fei{How can we be smart and efficient in computing repairs?}


\rebut{\textbf{8.} I don't understand figure 3. It seems to imply that a data repair is produced first (via a CH), and passed to the ontology repair module to search for k-combinations.  It's the other way round.  The ontology repair module traverses the space of possible repairs and computes the CH for selected repairs.  Based on this, we find minimal ontology repairs and find the corresponding data repairs from the CH.}

\ans{The second way that you described is correct, we address it by adding step numbers in figure 3.}

\rebut{\textbf{9.} section 7.3: "the complexity of error detection in FD based data repair is O(N)". Is this true?  How do we detect FD errors in linear time wrt the number of tuples?}

\ans{FD based data repair: for a single FD, the complexity of error detection is $O(N)$. Firstly, for the given FD, we use $O(N)$ time to partition the whole data into different equivalence classes. Secondly, for each equivalence class, if the RHS values are not equal, then the tuples in the equivalence class are in errors. The second step also can be done in $O(N)$ time. If we have multiple FDs $\Sigma$, then the complexity of error detection in FD based data repair is $O(N \times |\Sigma|)$.}

\ans{Synonym OFD based data repair: for a single synonym OFD, the only addition complexity compare to single FD based data repair is that we have to go through all the synonym classes $synonym(E)$ of all senses for each equivalence class. Then the complexity becomes $O(N \times |synonym(E)| \times |senses|)$, which in Section 4.4 we claimed that the complexity of data verification step for synonyms is linear. For multiple synonym OFDs $\Sigma$, the complexity is $O(N \times |synonym(E)| \times |senses| \times |\Sigma|$).}

\ans{Inheritance OFD based data repair: for a single inheritance OFD, similar to synonym OFD (go through all the synonym classes of all senses for each equivalence class), we have to go through all the LCA trees of all senses for each equivalence class. Let us denote the number of LCA trees as $K$, and $K$ is in the same order with the number of nodes in the ontology. Then the complexity is $O(N \times K \times |senses|)$. For multiple inheritance OFDs $\Sigma$, the complexity is $O(N \times K \times |senses| \times |\Sigma|$).}

\ans{Based on the analysis above, if I am correct, then we can claim that the complexity of error detection in OFD based data repair is linear w.r.t. the number of tuples $N$.}
% \fei{What does it mean to have the condition "if there are no errors"?  So you are saying there is no additional overhead to check OFD errors in general?  Remember these statements must hold in general cases.}

\noindent {\textbf{Jarek's comments:}} \\

\rebut{\textbf{1.} I think we should build the story of ontology repair into a more general problem of knowledge-base repair, with ontology repairs as just one of the applications of the more general problem. Talk in general that knowledge-base are represented as graphs etc.}

\ans{}


\rebut{\textbf{2.} we can share our proposal with students to incorporate motivation about knowledge-bases repairs into intro to make the paper stronger (this is also related to a comment above).}

\ans{}

\rebut{\textbf{3.} following Lukasz comment about error detection complexity, if it is truly linear, then this is improvement on our data discovery paper in CIKM, where part of the solution is data verification step. We should unify these results between these sections. For is-a in 4.4 we claim cubical and for synonyms linear. Can it be done better for is-a and it is linear as stated in Section 7? (or Sec. 7 applies only to synonyms, I think this is part of the confusion in the question by Lukasz)}

\ans{Similar to Lukasz's \#9 comment.}
\fei{The complexity to check satisfiability for FDs, OFDs (syn, and inh) needs to be made clear in one paragraph at the start of a section.}

\rebut{\textbf{4.}  should not problem statement currently in section 5.1 be somewhere earlier in the paper? }

\ans{We agree with you and tried to do that. However, to mention this problem statement, we have to define minimal repair and $\tau$-constrained repair first. In this case, we have to move the whole Section 5.1 earlier. We are not sure about the best position, so we just keep it here for now.}

\fei{Let's move a more general version of the statement to Section 2.2 where all problem statements are clear for the reader.  We can refine and elaborate more in Section 5.}

\rebut{\textbf{5.}  Can we replace values in Fig 4 and 5 and examples eg., Example 6.1 with some real values, to make it easier to follow for readers and more applicable? Currently I do not see any real-world example with senses for the scenario of data cleaning (that we came up and have in slides for one of our meetings). 
Synthetic dataset makes it dry and reviewers may start to believe that this problem is purely theoretical.}

\ans{Will change to the real example after we confirm with the theoretical parts in Section 6.1.}

\rebut{\textbf{6.}  I would make main complexity results theorems.}

\ans{Sure, we can do that after the complexity is confirmed.}

\rebut{\textbf{7.} I think contributions 3, 4 can be merged into one as we have to many of them. I would also specify upfront that this paper is an extensions of our CIKM paper and specify, which contributions are new, to make it easier for reviewers to judge extra 30\%.}

\ans{}


\rebut{\textbf{8.}  contributions 6, 7 and abstract can be rewritten to emphasize more novelty of the problem and solution. That previous work focused mostly on data repairs and here we introduce a new problem of data vs knowledge-base repairs that was not studied before with data-driven knowledge-base repairs based on the evidence in the data. (See for example Unified Model and Continuous Data Cleaning how data vs. ICs repairs were motivated.)}

\ans{}

\rebut{\textbf{9.} following Lukasz comment on vertex-cover, I would specify more details what are the biggest changes in that algorithm for the data-repair to work, what are the differences to make the problem not straightforward (so reviewers do not attack us). This is can be done via description and/or via example.}

\ans{Similar with Lukasz's \#6 comment.}


==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> cleaning_v0.tex <==
\section{Data Cleaning with OFDs} \label{sec:cleaning}

\eat{
\begin{enumerate}
\item First 2 paragraphs in this section: motivate the need for (contextual) cleaning. esp. after discovery of OFDs and how they can become stale. Refer back to cleaning Example in Sec. 1, and extend example with discussion of the scope of repairs from Prelim section, highlight properties of our solution/algorithm.
\item Give overview of repair solution.
\item Give Data and ontology repair algorithm details. 
\item Optimizations + Complexity
\end{enumerate}
}

%\fei{Need a good running example throughout these upcoming sections.}
As application requirements, domain semantics change, the data evolve, and ontologies may become incomplete.  Misalignment arises between a data instance $I$, an ontology $S$, and a set of OFDs $\Sigma$.  In this section, we study the problem of how to compute repairs to re-align $I, S$, and $\Sigma$.  Data naturally change due to updates and changes in domain semantics.  This change in semantics also leads to ontology incompleteness as new concepts and ontological relationships are introduced.  For example, new uses of medical drugs lead to new prescriptions to treat new and different illnesses.  While OFDs may also evolve, we argue that repairs to the data $I$ and ontology $S$ are more common in practice, and hence, our current focus.  When stale OFDs do occur, \fastofd can be used to discover the latest set of OFDs that hold over the data.  Formally, we modify $I$ and $S$ to produce $I'$ and $S'$, such that a repaired version of $I$, $I' \models \Sigma$, w.r.t. a modified version $S'$ of $S$.  
\eat{In this work, we focus on repairs to the ontology $S$ and data instance $I$, and consider repairs to $\Sigma$ in future work.} \eat{Similar to past work that propose repairs to the FDs by appending attribute(s) to the antecedent (making it more selective), we can consider repairs to each OFD $\phi \in \Sigma$~\cite{CM11,BIGG13}.  The distinction and overhead in repairing OFDs requires us to evaluate a set of candidate attributes under multiple senses.   must be found (w.r.t. an ontology $S$) covering all values in the appended attribute(s).  We defer the study of OFD repairs as future work, and focus on repairs to $I$ or $S$ in this section.}

%**************
\eat{\blue{\textbf{OFD Repair Problem:}}  \blue{
Given a relation instance $I$ and an ontology $S$, synonym and inheritance OFDs $\phi_{1}, \phi_{2} \in \Sigma$, respectively, where $I \not\models \Sigma$ \textit{w.r.t.} $S$.  We investigate the repair problem that seeks a set of \textbf{minimal repairs} such that for each repair $(I', S')$, $I' \models \Sigma$ \textit{w.r.t.} $S'$. 
}}

%*************************************
%\subsection{Types of Repairs} \label{sec:reptype1}
%\fei{Describe the type of OFDs we are considering are those with no overlap between LHS and RHS to preserve the equivalence classes for a chosen sense.  This underlying assumption of maintaining the equivalence classes is needed to preserve the utility of the sense selection. }

%\subsection{Synonym OFDs}
Recall that synonym OFDs require finding a sense under which all the values in the consequent of the OFD are semantically equivalent.  In contrast, inheritance OFDs require finding an LCA within a distance of $\theta$ of all descendant consequent values.  \eat{Several candidate LCAs may be evaluated according to maximal coverage, or information loss.}  Handling incompleteness w.r.t. an inheritance OFD can lead to structural changes in the ontology to accommodate newly inserted values.  These changes affect the validity of information in dependent applications, according to the update frequency.  We argue that such changes are less likely in practice than missing synonyms, as applications prefer \emph{minimal} repairs, to minimize downstream impact.   For example, medical ontologies are large with complex relationships such that topology changes significantly hinder manageability and maintenance.  In this work, we therefore focus on repairing synonym OFDs.

\eat{
We have introduced two classes of OFDs: synonym and inheritance.  A synonym OFD: $X \rightarrow_{syn} A$ is satisfied if there exists a sense under which all the $A$-values of tuples in $x \in \Pi_{X}(I)$ are synonyms.  i.e., there exists a sense that reconciles all the $A$-values within an equivalence class $x$ to be semantically equivalent.  In contrast, satisfying an inheritance OFD $X \rightarrow_{inh} A$, requires that for each $x$, the $A$-values of all tuples in $x$ are descendants of an LCA, which is within a distance of $\theta$ in $S$.  Clearly, there are many possible LCAs for a given $x$, and the problem is how to select a good LCA?  We may use criteria such as maximal coverage of the $A$-values, or minimal information loss.  We defer this study of inheritance OFDs to future work, and focus on repairing $I$ and $S$ w.r.t. synonym OFD only.
}
%\fei{Point here is just a focus on synonym OFDs, but need more justification why inh is not considered.}

OFDs interact when two or more dependencies share a common set of attributes.  This attribute overlap may occur over the antecedent or consequent attributes.  For example, consider two synonym OFDs: $\phi_1: X_{1} \rightarrow_{syn} A$ and $\phi_2: X_2 \rightarrow_{syn} B$, where $A \in X_2$.  \blue{If we update $t[A]$ to $t'[A]$, this may change the distribution of values in $X_2$, and may invalidate already performed repairs.  This requires re-evaluating existing repairs w.r.t equivalence classes in $X_2$, which can lead to an exponential number of repair combinations to consider.}  Another source of conflict occurs when two OFDs share the same consequent value $A$, e.g., $A = B, A \not \in \{X_1, X_2$\}, such that an update to $A$ affects both $\phi_1$ and $\phi_2$.  \eat{We focus on this latter case, i.e., repairs of synonym OFDs with possible overlap in the consequent attributes, as space of repairs is fixed w.r.t. the distribution of values in $A$.  We defer the study of overlap between $A$ and $X_2$, as next steps since this requires re-evaluation of the equivalence classes w.r.t. $X_2$, and efficient navigation of possibly exponential number of repairs, and sense re-selection.} \blue{Our proposed techniques handle this latter case, and when $A \in X_2$, and the updated value $t'[A]$ does not change the distribution of values in $X_2$, i.e., $t'[A]$ is a synonym of $t[A]$.}
%Henceforth, we use the terms \emph{synonym FD} and \emph{synonym OFD} interchangeably. 


%For a selected senese, this can invalidate repairs that were made to $\phi_2$ already.  To simplify the problem, we propose techniques that select a sense assuming fixed equivalence classes for a set of OFDs.  To ensure this property holds, either synonym OFDs do not overlap, or if they do, the overlap occurs only in the RHS attribute. 
%}  

%\blue{As shown in Example~\ref{ex:motivating}, selecting different senses to interpret a given equivalence class leads to different ontology repairs and data repairs, and then all the repairs have to be applied based on the selected sense. However, repairing data for one OFD may change the equivalence classes of another OFD if those two OFDs have interaction, which in further may change the selected sense for the impacted equivalence classes. For example, consider two OFDs: $\phi_1: A \rightarrow B$ and $\phi_2: B \rightarrow C$, repairing RHS (attribute $B$) for $\phi_1$ would split or merge equivalence classes for $\phi_2$. Thus, to simplify the problem, we only consider the OFDs with no overlap between LHS and RHS attributes to preserve the equivalence classes for a selected sense. Besides that, we only discuss repair violations w.r.t. a set of synonym OFDs and we will consider inheritance OFDs in the future work. This is because inheritance ontology has a more complex relationship between nodes compare to that of synonym ontology. Repairing values in an inheritance ontology would change the hierarchy and the relationship between the values.}

% \blue{\zheng{(In this paragraph, I want to describe how inheritance OFDs reduce to synonym OFDs.)} For a given inheritance OFD, we can reduce it to a synonym OFD with the following approach: for each equivalence class in the inheritance OFD, we consider an LCA tree (with a given $\theta$) of the corresponding inheritance ontology (under a specific sense) as the same as a synonym class of a synonym ontology, i.e., all the values in the LCA tree are synonyms. Based on the above reason, we only discuss repairs w.r.t. synonym OFDs in the following sections.}

%*************************************
%Possible Repairs} \label{sec:reptype1}
\subsection{Types of Repairs}
\eat{In this section, we discuss about different types of repairs in our framework. Since data evolves over time and the ontology may be out-of-date, we only consider data and ontology repair to resolve OFD violations. We do not modify or re-discover the OFDs when the violations occur, since discovering a new set of OFDs that are adaptive to the current data and ontology is expensive.}

% \fei{**Disclaimer: I am not revising the writing, only the content and if the intuition is clear, and arising questions a reader may have.}
%\fei{Define what it means to be a repair, and that we assume a distance function dist() exists.  Need to define what dist. is for each type of repair below.}

\noindent \textbf{Data Repair.}  Consider a synonym OFD $\phi$: $X \rightarrow_{syn} A$, and an equivalence class $x \in \Pi_{X}(I)$ where there exists at least two tuples $t_1, t_2 \in x$, such that $t_1[A]$ and $t_2[A]$ are not synonyms under some sense $\lambda$.  Without loss of generality, we consider updates to $t_1[A]$ where the domain of repair values are values in $S$ under sense $\lambda$ to ensure all $t[A]$ values in $x$ are synonyms. We consider repairs to values in the consequent attributes, i.e., values in attribute $A$. 


%We consider all the tuples in $x$ are violations. Assume that $t_i (1 \leq i \leq n)$ is the tuple whose $A$-value does not exist in $S$ under $\lambda$. To repair such a violation, we would update $t_i[A]$ to be equal to any value that exists in the ontology under $\lambda$.}

%That is, that there does not exist an interpretation (sense) where all the $A$-values of tuples in $x$ are synonyms (are not descendants of an LCA within a distance of $\theta$ in $S$). 
Let $\mathcal{P}(I)$ denote the set of all possible data repairs of $I$. For a repair $I'$ of $I$, we use $dist(I, I')$ to denote the difference between $I$ and $I'$, which is measured by the number of cells whose values in $I$ are different from  the values of the corresponding cells in $I'$, i.e.,  $dist(I, I') = |\Delta(I,I')|$.
% \begin{enumerate}[nolistsep]
%     \item \emph{To repair such a violation, we can change the $A$ values to be the same using a value from domain(A). Repair the $A$ values to be the same using a value from domain(A).} Without loss of generality, consider tuples $t_1, t_2 \in x$, where $t_1$[$A$] $\neq$ $t_2$[$A$], we would update $t_1$[$A$] to be equal to $t_2$[$A$].  We will do this when there is sufficient evidence in the equivalence class $x$ to conclude that $t_2$[$A$] is the correct value.  \fei{This defn is more from traditional FD repair, and not in the context of replacing to a canonical value for syn or inh OFDs.  Discuss how inh OFD reduces to syn OFDs. I note that the above only considers repairs to RHS.}
%     \item \emph{Repair the $A$ values to a variable.}  Similar to past work that propose V-instance (variable) repairs~\cite{MinCost1}, when there is insufficient evidence to repair to a value from the domain($A$), we insert a variable $v$ that can be assigned to a set of values to satisfy $\phi$.  V-instance repairs can arise when the $A$-values overlap among two or more OFDs, where multiple repair values are possible according to different interpretations w.r.t. each OFD. 
% \end{enumerate}


\eat{ %fei: summarized above to be clear the types of data repair, gave idea what V-instance repair means
\noindent\textbf{Data Repair.} We consider data repair as changing the values of the cells in $I$, but not deleting and inserting the tuples to resolve the violations. Suppose we have an equivalence class $x=\{t_1,...,t_n\}$ with an synonym OFD $\varphi_i: X \rightarrow_{syn} A$ (resp. inheritance OFD $\phi_j: X \rightarrow_{inh} A$ with the threshold $\theta$). $x$ is in violation based on $\phi_i$ (resp. $\phi_j$) w.r.t an ontology $S$ if there is no sense in $S$ that all $t_i[A]$  are synonymous (resp. there is no LCA in $S$ that all $t_i[A]$ are descendant of it within a distance of $\theta$) for $i \in \{1,2,...n\}$. 

To resolve the violations by using data repair, we use the notion of V-instance\cite{MinCost1} in which we can assign variables to each cell. In this work, we will  instantiate each cell in a specific way later based on the the ontology $S$ and the domain of the attribute. In V-instance, we have two types of changes to each cell in order to resolve the violation: (1) changing the cell value to a constant in the domain when there is enough information for doing so \eat{(for the attribute $A$, we consider the domain as $Domain(A)$ and for the attribute $X_i \in X$, the domain is $Domain(X_i)$)}, (2) changing the cell value to a variable when there is no suggestion to resolve the violation.
For the attribute $A$ of an OFD, we consider the domain of the ontology as a potential data repair. For a synonym OFD, for each equivalence class $x$, the domain of repair includes all the values that exist in $x$ and they are synonym based on a specific sense (we discuss the details of finding the sense in Section \ref{sec:minimallyrepair}). Similarly, for an inheritance OFD, for each equivalence class $x$, the domain of repair includes all the values that exist in $x$ and they are descendant of an LCA within a distance of $\theta$. This new domain of repair which does not exist in FD based data repair, comes from the definition of the OFDs. In OFDs, there is no violation in an equivalence class of an synonym OFD (resp. inheritance OFD) if all the values of the RHS attribute are synonym (resp. descendant of an LCA within a distance of $\theta$) under a specific sense.
%\orange{We have changed the whole paragraph to make it more clear.}
%\fei{What does this mean?  What specific way?  Based on what in the domain?  Here you just talk about a value in a cell can change, and where do the changes occur, LHS or RHS?  Why only synonym OFDs? What is a V-instance repair?  This has not been explained.} 
%\cyan{We briefly explained how V-instance algorithm works.}
}

%\textcolor{purple}{How do we distinguish when type (1) vs. (2) repair occurs?  From our meeting, what is the justification for values from S?  How do you deal with the consequences from interating OFDs?}

%
\noindent\textbf{Ontology Repair.} 
\blue{We consider updates to $S$ that add new values to a node w.r.t. a given sense $\lambda$ to preserve existing knowledge, which is often curated by domain experts.  We use $\mathcal{P}(S)$ to denote the set of possible ontology repairs to $S$.  For a repair $S'$ of $S$, we define distance, $dist(S, S') = |\Delta(S,S')|$, i.e., as the number of new values, also referred to as \emph{concepts}, in $S'$ that are not in $S$.  
%We seek repairs to $S$ that minimize $dist(S, S')$.
}

\eat{For example, a new drug is added to the class of \lit{diltiazem} drugs under the FDA sense.  In Section~\ref{sec:sense},  we introduce an algorithm to select a sense $\lambda$ under which we evaluate repairs to $S$ and $I$ such that $I' \models \Sigma$.  We take a conservative approach, and consider only insertions to $S$ }
%We defer deletions and updates to $S$ as future work.

  \eat{This measure does not differentiate among the individual candidates, e.g., adding concept \lit{a} vs. \lit{b} under sense $\lambda$ can alter how values $t[A]$ are interpreted, and the resulting number of errors.  If value \lit{a} occurs more frequently than \lit{b} among the error tuples, then \lit{a} will lead to a greater reduction in the number of errors.  Towards this goal, more sophisticated distance functions can be incorporated that consider criteria such as: (i) the number of resolved errors w.r.t. $S$ vs $S'$; (ii) the information content of each candidate repair value w.r.t. $I$; and (iii) the distance between the data distributions w.r.t. $S$ vs. $S'$.  }


%to obtain an $S'$ whereTo resolve the violation mentioned aforesaid, we would also consider ontology repair by adding $t_i$[$A$] to $S$ under $\lambda$. \fei{X} OFDs are interpreted w.r.t. a specific sense, and naturally repairs to $S$ must also be considered w.r.t. a sense.  In Section~\ref{sec:selectsense}, we describe our approach to selecting a suitable sense.  Note that we take a more conservative approach towards ontology repairs to preserve the knowledge that is often curated by domain expertise, and do not consider deletion of nodes or edges in $S$.}

%\blue{We use $\mathcal{P}(S)$ to denote the set of all possible ontology repairs of $S$. For a repair $S'$ of $S$, we define the distance between two ontologies as follows. We use a vector $\Delta(S, S') = (u_1, u_2, ..., u_t)$ to denote all the values exist in $S'$ but not exist in $S$ under a specific sense. To measure the distance between $S$ and $S'$, we use a weighting function $w(U)$ ($U\in\Delta(S,S')$) to determine the relative penalty of adding a set of values $U$. We consider the weighting function is non-negative and monotone, i.e., for any two value sets $U$ and $V$, $U \subseteq V$ implies $w(U) \leq w(V)$.   To simplify the problem, we consider $w(U)$ as the number of values in $U$. \fei{so what is there to sum in f(U) then?} However, we can distinguish between values in $U$ based on their features by using other definitions of $w(U)$. For example, consider two values $u_i$ and $u_j$ that could be added to $S$, where $u_i$ exists only once in one equivalence classes, while $u_j$ exists many times in different equivalence classes. Intuitively, adding $u_j$ to the ontology should be more expensive that adding $u_i$ because it has more impacts to other equivalence classes. \fei{I don't understand last sentence.} In general, the more informative a set of values is, the more expensive it is when being added to the ontology. For example, we can use the entropy of $U$, $H(U)=-\Sigma P(u_i)log_b P(u_i)$, to measure the information captured by a set of values $U$, where $P(u_i)$ denotes the average probability of the value $u_i$ exists in the data across all the equivalence classes. We use $dist(S, S')$ to denote the number of new nodes added from $S$ to $S'$, i.e., $dist(S, S') = |\Delta(S,S')|$.} \fei{Does it not matter where you add the node?  Are all insertions considered equally? What is the distance b.w S and S' for different values added to the ontology?  Looking at the values added, e.g., key values as per FD case.}


%\noindent\blue{\textbf{Minimal Repair.}
%\label{def:minimal} %Our solution focus on a subset of repairs that are Pareto-optimal w.r.t. two distance functions: $dist(I, I')$ that measures the distance between two database instances, and $dist(S, S')$ that measures the distance between two ontologies. We define such repairs as minimal repairs as follows.}

\noindent \textbf{Minimal Repair. }
%\cyan{As OFDs are interpreted w.r.t. a sense, our evaluation of repairs must also be done w.r.t. a specific sense $\lambda$.  Hence, our recommended repairs are also interpreted w.r.t. $\Sigma$ for a selected $\lambda$, and we discuss in Section~\ref{sec:selectsense} how such a $\lambda$ is chosen. 
The universe of repairs, $U$, represents all possible pairs ($S', I'$) such that $S' \in \mathcal{P}(S)$ and $I' \in \mathcal{P}(I)$ and $I' \models \Sigma$ w.r.t. $S'$.  
%\blue{As mentioned before, each equivalence class is associated with a sense to interpret it, and selecting different senses may lead to different data and ontology repairs. We defined the \emph{minimal repair} based on the selected sense (the details of how to select a sense is mentioned in Section~\ref{sec:selectsense}) for each equivalence class as follows.}
% The space of repairs consists of
We want to find minimal repairs in $U$ that do not make unnecessary changes to $S$ or $I$ in a Pareto-optimal sense.
%, keeping in mind that making more changes to $S$ can allow us to make fewer changes to $I$ and vice versa.

\begin{definition}\label{def:minimal} (\emph{Minimal Repair}). 
We are given an instance $I$, OFDs $\Sigma$, and an ontology $S$, where $I \not\models \Sigma$ \textit{w.r.t.} $S$.   A repair ($S'$, $I'$) $\in U$ is minimal \eat{under a sense $\lambda$} if $\nexists (S'', I'') \in U$ such that $dist(S,S'') < dist(S,S')$ and $dist(I,I'') < dist(I,I')$.
%$(S'', I'') \prec (S', I')$.
\end{definition}

For example, suppose $U$ contains three repairs: the first one makes two changes each to $S$ and $I$, the second one makes two changes to $S$ and three changes to $I$, and the third one makes one change to $S$ and five changes to $I$.  Here, the first and the third repair are minimal.

\eat{
Let the pair (vector with two components) ($|S'|$, $|I'|$) represent the number of repairs in $S'$ and $I'$, respectively.  We define the concept of dominance for two vectors as follows.
\begin{definition}\label{def:dominance}
We define vectors $\mathcal{X} = (x_1, ... , x_m)$ and $\mathcal{Y} = (y_1, . . . , y_m)$, and say $\mathcal{X}$ dominates $\mathcal{Y}$, denoted by $\mathcal{X} \prec \mathcal{Y}$, iff for
$i \in {1,..., m}, x_i \leq y_i$, and at least one element $x_j$ in $\mathcal{X}$ is strictly less than the corresponding element $y_j$ in $\mathcal{Y}$.
\end{definition}
}
%\blue{
%A repair ($S', I'$) is considered Pareto-optimal if there does not exist any other repair that dominates it.  Specifically, $(S_i', I_i')$ dominates $(S_j', I_j')$, denoted $(S_i', I_i') \prec (S_j', I_j')$, if $\{\forall i,j | (dist(S, S_i') \leq dist(S, S_j')), (dist(I, I_i') \leq dist(I, I_j'))\}$, and $\{\exists k | (dist(S, S_i') < dist(S, S_k')) \vee (dist(I, I_i') < dist(I, I_k'))\}$. 
% }
 


%\blue{\begin{example} \label{ex:dominate}
%Real example.
% Consider two synonym OFDs $\phi_1: A \rightarrow C$ and $\phi_2: B \rightarrow C$ over table Figure~\ref{fig:ecg}(a).  Figure~\ref{fig:ecg}(b) shows the ontology with seven senses over attribute $C$, the values in each sense are synonyms. Based on the definition in Section~\ref{sec:prelim}, there are four equivalence classes: $x_2 = \{t_1 - t_4\}$, $x_4 = \{t_5 - t_{10}\}$, $x_1 = \{t_1 - t_7\}$, $x_3 = \{t_8 - t_{10}\}$. If we select sense $\lambda_2$ for $x_4$, consider the following two types of repairs: (i) $Rep_1:$ we repair the ontology by adding the value $c_3$ to the ontology as an equivalent medication to $c_2$ and $c_4$.  Addition to that, we update the value $t_{8}$[C] to either $c_2$ or $c_4$. In this case, we apply one ontology repair and one data repair, denoted by $(1,1)$; (ii) $Rep_2:$ we repair the ontology by adding the value $c_5$ and to the ontology. Addition to that, we update $t_{9}$[C] and $t_{10}$[C] to $c_2$ or $c_4$. In this case, we apply one ontology repair and two data repairs, denoted by $(1,2)$. Based on Definition~\ref{def:minimal}, $Rep_1$ dominates $Rep_2$.
%\end{example}}



%\fei{It would be preferable to have a running example that we can use for the rest of the paper, starting here.  Show a table, and OFDs, instead of having the reader context switch between different examples. This is hard to follow and visualize.}

% Original 
%Given an instance $I$, a set of OFDs $\Sigma$, and an ontology $S$, where $I \not\models \Sigma$ \textit{w.r.t.} $S$ with a set of senses $\Lambda$. Each equivalence class $x \in \Pi_{X}(I)$ is interpret by a selected sense $\lambda \in \Lambda$ (details in Section~\ref{sec:selectsense}). A repair ($I'$, $S'$) is minimal if there is no other repair ($I''$, $S''$) for the selected senses of all the equivalence classes such that $dist(S, S'')$ is smaller than $dist(S, S')$ and $dist(I, I'')$ is smaller than $dist(I, I')$,  where $I', I'' \in \mathcal{P}(I)$ and $S', S'' \in \mathcal{P}(S)$.

% \begin{definition}\label{def:minimal} (\emph{Minimal Repair}). 
% Given an instance $I$, a set of OFDs $\Sigma$ and an ontology $S$, where $I \not\models \Sigma$ \textit{w.r.t.} $S$ with a set of senses. A repair ($I'$, $S'$) is minimal if there is no other repair ($I''$, $S''$) for all the senses such that $dist(S, S'')$ is smaller than $dist(S, S')$ and $dist(I, I'')$ is smaller than $dist(I, I')$,  where $I', I'' \in \mathcal{P}(I)$ and $S', S'' \in \mathcal{P}(S)$.
% \end{definition}
%\fei{I don't think we solve this problem for all senses as stated above.  We only do this for one chosen sense.  Please confirm.} \zheng{Before, I thought we should define minimal repair in a very general way, i.e., we should define it by considering all the senses. And consider selecting the sense before repairing is just our solution.      Based on your suggestion, I added some sentences to justify why we need select a sense for an equivalence class, and also modified Definition 6.}
 
%Note that we seek minimal repairs to $I$ and $S$ under a selected sense $\lambda$.  We present details of our sense selection algorithm in Section~\ref{sec:selectsense}. 
 
%\fei{I don't think we can say that the chosen $\lambda$ leads to  minimal repair among ALL senses.  What can we say about our chosen sense $\lambda$ and the minimal solution we get?  This is important to state here!} 
%\zheng{I will address these comments after Sec.7 is confirmed.}

\eat{
\noindent \textbf{$\tau$-constrained Repairs.}
In existing work, Beskales et. al, restrict the number of allowed data repairs to be within a given threshold $\tau$~\cite{BIGG13}.  The goal is to compute a $\tau$-\emph{constrained repair}, $(S', I') \in U$, where $dist(I, I') \leq \tau$, and $dist(S, S')$ is minimal across all repairs in $U$. To find such $\tau$-constrained repairs requires varying $\tau$ from 0 to the minimum number of required updates to $I$ to satisfy $\Sigma$ w.r.t. $S$, denoted as $\delta_{opt}(S, I)$.  Given this, Beskales et. al. show that: (i) each $\tau$-constrained repair is a minimal repair, and (ii) all minimal repairs can be obtained by varying $\tau$ in the range $[0, \delta_{opt}(S, I)]$~\cite{BIGG13}.  
}
\eat{
There has been a wealth of work on finding repairs to data~\cite{}, and repairs to FDs~\cite{} such that the data is consistent w.r.t. the FDs.  Beskales et. al.  define a space of repairs that range from updating only $I$ and keeping $S$ as is, to updating only $S$ and leaving $I$ unchanged.  To balance the relative trade-off between these two sides, they introduce a trust parameter $\tau$ that limits the number of data repairs to be less than $\tau$~\cite{BIGG13}.  The idea is to seek a repair, called a $\tau$-\emph{constrained repair}, $(S', I') \in U$, where $dist(I, I') \leq \tau$, and $dist(S, S')$ is minimal across all repairs in $U$. 
To find such $\tau$-constrained repairs requires varying $\tau$ from 0 to the minimum number of required updates to $I$ to satisfy $\Sigma$ w.r.t. $S$, denoted as $\delta_{opt}(S, I)$.  Given this, Beskales et. al. show that: (i) each $\tau$-constrained repair is a minimal repair, and (ii) all minimal repairs can be obtained by varying $\tau$ in the range $[0, \delta_{opt}(S, I)]$~\cite{BIGG13}.  
 \fei{Need to state the point of this description - because we apply a similar notion of $\tau$-constrained repairs.}
}
%\blue{Given an instance $I$, a set of OFDs $\Sigma$, an ontology $S$ with multiple senses, and a threshold $\tau$, we limit the maximum number of cell changes that can be performed while obtaining $I'$ to a threshold $\tau$, and to obtain an ontology $S'$ such that $dist(S, S')$ is minimal and $I' \models \Sigma$ w.r.t $S'$.  We call such a repair $(I', S')$, a $\tau$-constrained repair, if there is no other repair ($I''$, $S''$) for all the senses \fei{Do we guarantee this when we select senses that it's minimal across all senses?} such that $dist(S, S'')$ is smaller than $dist(S, S')$ and $dist(I, I'')$ is smaller than $\tau$. }

\eat{\blue{We map between minimal repairs and $\tau$-constrained repairs as follows: each $\tau$-constrained repair is a minimal repair, and all minimal repairs can be obtained by varying $\tau$ in the range $[0, \delta_{opt}(\Sigma, I)]$. Let $(I'', S'')$ be the minimal repair with the smallest $dist(I, I'')$ that is strictly greater than $dist(I, I')$. If such a repair does not exist, let $(I'', S'')$ be $(\emptyset, \emptyset)$. In the similar spirit to~\cite{BIGG13}, we define the range of $\tau$ is as follows.
\begin{equation}\label{eq:tau}
\tau \in
\left\{
     \begin{array}{lr}
     \left[dist(I, I'), dist(I, I'')\right) & if (I'', S'') \neq (\emptyset, \emptyset) \\
     \left[dist(I, I'), \infty \right) & if (I'', S'') = (\emptyset, \emptyset).
     \end{array}
\right.
\end{equation}}

\blue{Given the above, each $\tau$-constrained repair is a minimal repair, and each minimal repair $(I', S')$ corresponds to a $\tau$-constrained repair, where $\tau$ belongs to the range defined in Equation~\ref{eq:tau}.}
}%\fei{You are missing discussion on the range of $\tau$, what it means to be $\tau$-constrainted repair, and the intuition of this.  What is the range of allowable $\tau$ values?}


% \begin{equation}
% \tau \in 
% \left\{
% \begin{aligned}
%  \left[dist(I,I'), dist(I, I'') \right) & , & if (I'', S'') \neq (\emptyset, \emptyset), \\
%  \left[dist(I,I'), \infty \right) & , & if (I'', S'') = (\emptyset, \emptyset).
% \end{aligned}
% \right.
% \end{equation}

% Fei: Problem statement doesn't occur so late in the
%\noindent \blue{\textbf{Problem Statement.}
%Our problem is to compute a set of repairs ($S', I'$) such that each repair is a $\tau$-constrained repair.  \fei{What about the pareto-optimal set?}


\eat{For inheritance OFDs, decreasing the path length threshold $\theta$ may change the LCA for an equivalence class, and the tuples that are not covered by the LCA my decrease or keep the same. Thus, the required minimum number of data repair is monotonically non-decreasing as $\theta$ decreases. Since the total minimum number of data repair is limited by $\tau$, we need to apply more ontology repairs for a given $\tau$ as $\theta$ decreases.}

%************************************************
\subsection{\ofdclean}
\label{sec:framework}

OFDs enrich the semantic expressiveness of FDs via ontological senses, which allow for multiple interpretations of the data.  In traditional FDs, senses do not exist, and there is only one interpretation.  For a set of OFDs $\Sigma$, the problem of finding a minimal repair to $S$ and to $I$ requires evaluating candidate senses for each equivalence class w.r.t. each $\phi \in \Sigma$, and assigning a sense to each class.   \eat{pecifically, since each $\phi: X \rightarrow A$ induces a set of equivalence classes $\Pi_X$, the corresponding values in $A$ for each $\Pi_X$ have a unique interpretation (sense).}  \blue{Interactions between repairs occur due to overlapping attributes among OFDs.  Updating a data value or adding a new concept to an ontology w.r.t. $\phi_1$ can increase or decrease the number of repairs w.r.t. another OFD $\phi_2$.  Exhaustive enumeration of all exponentially possible sense assignments is not feasible.}  
%Finding a minimal repair (Defn.~\ref{def:minimal}), requires managing the interplay between changes in the ontology $S$ and in the data instance $I$.  For example, finding an instance $I'$ close to $I$ depends on $S'$.  Similarly, finding an $S'$ close to $S$ depends on $I'$.  
 
 
 %With overlapping consequent attributes among OFDs, a sense that leads to a minimal number of repairs for one OFD may not be the best for another.  An alternative would be to propose a minimal repair for each sense, but this would not be feasible in practice for a large number of senses.  
To manage this complexity and interaction, we propose an algorithm to efficiently navigate and select the most promising candidate senses.  We take a greedy, two-step approach. First, we compute an initial sense assignment for each equivalence class that \blue{minimizes the number of repairs to the ontology and to the data (locally) w.r.t. each OFD and each equivalence class}.  Secondly, we \blue{go beyond a single OFD to} consider interactions among $\phi \in \Sigma$ where attribute overlap occurs, such that repairing values w.r.t. $\phi_1$ may increase or decrease the number of errors in $\phi_2$.  We model the overlapping tuples between $\phi_1$ and $\phi_2$ as two distributions w.r.t. their assigned senses.  We refine the sense assignment such that the number of necessary updates to transform one distribution to the other is minimized.  We evaluate these OFD interactions according to the (decreasing) distance between the equivalence class distributions.  Lastly, with a computed sense assignment, our problem reduces to finding a minimal repair of $S$ and to $I$ such that it satisfies $\Sigma$.  

Existing constraint-based repair algorithms are insufficient as they do not consider senses~\cite{CM11, BIG10, GMPS13}.  We propose \ofdclean, a framework that includes ontology and data repair with sense assignment to minimize the number of changes to $I$, and $S$.  \ofdclean is amenable to both synonym and inheritance OFDs.  Intuitively, we modify $S$ to obtain an $S'$ as close as possible to $S$, while ensuring that a repair $I'$ exists that is as close as possible to $I$ and satisfies $\Sigma$.  We compute $I'$ such that it's close to $I$, and the number of changes is less than \blue{a threshold $\tau$.  We call such repairs $\tau$-\emph{constrained repairs}.}

%To manage this interaction, while ensuring $dist(I, I') \leq \tau$, we adopt a similar philosophy to repairing FDs by Beskales et. al. that consists of two steps~\cite{BIGG13}.  First, we modify $S$ to obtain an $S'$ as close as possible to $S$, while ensuring that a repair $I'$ exists that is as close as possible to $I$ and satisfies $\Sigma$.  Secondly, we compute $I'$ such that it's minimal from $I$, and the number of changes is less than $\tau$.

%To compute $S'$, we need to determine the minimum number of modifications to $I$ to produce an $I' \models \Sigma$ w.r.t. $S'$.  Unfortunately, computing the exact minimum number of cells to change in $I$ to satisfy more than one FD is known to be NP-hard~\cite{KSS09}.  Since OFDs subsume FDs, the same hardness results apply when repairing $I$ w.r.t. $\Sigma$ for more than one OFD. Beskales et. al., show that an upper-bound exists on the minimum number of required cell changes via a constant $P$~\cite{BIGG13}. For OFD repair, we define $P = min\{|Z|, |\Sigma|\}$, where $|Z|$ denotes the number of unique right-hand-side (RHS) attributes in $\Sigma$. We seek $P$-approximate $\tau$-constrained repairs, where a $P$-approximate $\tau$-constrained repair $(S', I')$ is a repair in $U$ such that $dist(I,I') \leq \tau $, and there is no other repair $(S'', I'') \in U$ such that $(dist(S, S''), P \cdot dist(I, I'')) \prec (dist(S, S'), \tau)$. 

%\fei{Need to give an overview of the bound and type of repairs are are searching for.  If you are claiming that you are looking for $\tau$-constrained repairs, and these are minimal, then it has to be clear here how you are finding the minimal repairs.  Are they P-approximate, $\tau$-constrained?}\zheng{Added more details.}

%************************************************
\subsection{Framework Overview}
Figure~\ref{fig:repairframework} provides an overview of \ofdclean.  Given $I, S$ and $\Sigma$, \ofdclean identifies inconsistencies in $I$ w.r.t. $\Sigma$ and $S$, and returns a set of minimal repairs ($I', S'$) such that $I' \models \Sigma$ w.r.t. $S'$.   \eat{Our framework extends the data repair algorithm proposed by Beskales et. al.~\cite{BIGG13}, to consider repairs to $S$ and $I$, such that modified $I' \models \Sigma$ w.r.t. a repaired $S'$.} 
%We address the following challenges not considered in prior work: \eat{that computes near-optimal repairs to the data and to the FDs~\cite{BIGG13} assuming a bounded number of $\tau$ data repairs. Considering $k$ modifications (attribute insertions) to an FD, Beskales propose a space of Pareto-optimal solutions for each $k$, and where the number of data repairs are bounded by $\tau$.  In our problem setting, we must address the following two challenges not considered in prior work:}  (1)
We require $I$ and each $\phi \in \Sigma$ to be interpreted w.r.t. a sense $\lambda$. We evaluate candidate senses, and select a $\lambda$ for each equivalence class $x$.  \ofdclean execution proceeds along two main modules. 
%during error detection and cleaning;  (2) we consider repairs that add new values to $S$ (we do not consider deletions).\eat{evaluate all $A$-values in $x$ that are not in $S$ as candidates for an ontology repair, and select one as the repair value for insertion into $S$.}  

\eat{Your modules in text here do not match the number in the figure, and not all steps in the figure are described.  If you're going to talk about modules how are these identified in Figure 3?  Looks like you have 6 modules.  However, two blocks are bold, but Selecting senses is not.}

\eat{Beskales et. al.~\cite{BIGG13} proposed a data cleaning framework that generates multiple suggestions for how to modify the data and/or the FDs in a minimal and non-redundant way, corresponding to various levels of relative trust between data and FDs.  They defined the relative trust by setting a parameter $\tau$ to specify the maximum number of allowed data changes (i.e., the smaller the $\tau$, the greater the trust in the data). Firstly, they give an efficient algorithm for finding minimal modifications to a set of FDs such that no more than $\tau$ data modifications will be required to satisfy the modified FDs.  The algorithm prunes the space of possible FD modifications using $A^*$ search combined with a novel heuristic that estimates the distance to an optimal set of FD modifications. Then they give an algorithm that computes the required data modifications with the following steps (1) build a conflict graph $G$ for the data instance $I$ and FDs $\Sigma$ by following \cite{Arenas01}, which shows the violations between the tuples in $I$ w.r.t $\Sigma$. In the conflict graph, there is a node for each tuple and if there exist a violation between two tuples $t_1$ and $t_2$, then there will be an edge connects the nodes $t_1$ and $t_2$. (2) compute the minimum vertex cover of $G$ by using an approximation algorithm \cite{Garey79}, which helps to find the upper bound of the necessary minimum data repair that is needed to clean the data. Finally, to find all Pareto-optimal solutions of data and FDs repair, they repeatedly make one constraint repair by adding an attribute to the RHS of an FD in $\Sigma$ to build the new set of FDs $\Sigma'$, and then calculate the minimum data repair based on the regenerated conflict graph of $I$ and $\Sigma'$.}

\noindent \textbf{Sense Assignment.} Let $\phi: X \rightarrow_{syn} A$ be a synonym OFD, where for each 
equivalence class $x \in \Pi_{X}$, $x$ is interpreted w.r.t. an assigned sense $\lambda_x$.  \eat{This requires us to select one interpretation during error detection and repair  Finding an optimal data repair, under one interpretation, for a set of FDs is already NP-hard~\cite{BFFR05}, hence, considering all sense assignments for all $x$ is not practically feasible.} Given $I, S$, and $\Sigma$, for each $\phi \in \Sigma$,  we compute $\lambda_x$ for each $x \in \Pi_{X}$ such that $(I', S')$ is minimal and $I' \models \phi$. We denote the set of all senses across all $x$ for $\phi$ as \lambdaphi $ = \cup_{x \in \Pi(X)} {\lambda_x}$.   
%that minimizes the number of data and ontology repairs and are dominate, assuming only the existence of $\phi$.    



Intuitively, we compute $\lambda_x$ for every $x \in \Pi_{X}$ to obtain an interpretation that can achieve a minimal repair.  We take a local greedy approach to consider only $\phi$ when computing \lambdaphi.  After this initial assignment, we model the interactions among the OFDs in $\Sigma$, via their overlapping equivalence classes, and locally refine the initial sense assignment.  We quantify interactions and conflicts by comparing the difference between the distributions represented via a pair of equivalence classes.  \eat{For each $x \in \Pi_{X}$, for every $\phi \in \Sigma$, we assign a sense $\lambda$ to x, where $\lambda_x \in \Lambda_{\phi}$. }  The final assignment of senses for all $\phi \in \Sigma$ is denoted as $\Lambda(\Sigma) = \cup_{\phi}$ \lambdaphi.

%This  w.r.t. Given a set of senses $\Lambda$, we introduce a greedy-based algorithm (Section~\ref{sec:selectsense}) to select the sense $\lambda \in \Lambda$ that minimizes the number of changes to cells and ontology repairs that participate in errors across multiple OFDs. Our approach globally consider the interactions between equivalence classes, and as the results, each equivalence class will be assigned a sense.} 

%Selecting different senses to interpret a given equivalence class $x$ may lead to different ontology repairs and data repairs. To globally find the suitable senses for all the equivalence classes (i.e., the selecting senses lead to $\tau-$constrained repair), the exhaustive approach finds the solution by traversing all the possible senses combinations for all the equivalence classes, which is expensive and complexity is $O(|x|^{|sense|})$. Here, $|x|$ is the number of equivalence classes in $I$ and $|sense|$ is the number of senses in $S$.  In this module, we propose a heuristic solution to select sense for each equivalence class, which avoids traversing all the senses combinations of equivalence classes, and the details are shown in Section~\ref{sec:selectsense}.}

%\fei{Many of the concepts explained here do not have the right context.  We have not spent time talking much about repair w.r.t. equiv. class, why we only consider ontology repairs to new data values, what does each node in lattice represent, what is the challenge here and why model as a lattice?  Many of these details are not appreciated until we let the reader know what we are trying to do and why it's hard.  Simplified text.  I have tried to re-write to make the motivation of ontology repair more clear and explain why we only consider new values and additions.  How we do it is left to later.}

\noindent \textbf{Compute Repairs.}   \eat{An ontology $S$ may become outdated as new domain concepts are introduced (but not added to $S$).  For example, new medications are introduced after research and clinical trials, used by patients, but not updated in ontologies.  In such cases, we seek to repair $S$ by adding these concepts to $S$ to re-align with the data.}  
Given $\Lambda(\Sigma)$,  {\sf Compute Repairs} computes the set of minimal repairs by first generating the set of ontology repair candidates that appear in an equivalence class $x$, but not in $S$.  It then considers different combinations of these candidates, up to a given value $k$, by traversing a set containment lattice.  We optimize the traversal of the lattice by adopting a beam-search strategy, which selects the top-$b$ candidates to expand at each level of the lattice~\cite{lowerre}.  

To compute the necessary data repairs to achieve consistency, we consider updates to the consequent attribute $A$ from the domain of $A$ and synonyms of $A$ in $S$ under the selected sense.  We select candidate repairs that make at most $\tau$ updates.  %In our implementation, we use the data repair algorithm from Beskales et. al~\cite{BIGG13}.  
%However, our framework is amenable to any data repair algorithm that accepts input candidates (e.g., synonyms) for evaluation.
%takes as input the candidate attribute(s), and candidate repair values.

%attribute domain, and the synonyms in $S$ for  ...\fei{Do we do anything different than besakales or do I just say we apply their algorithm?  What is new or different to say here?}  \cyan{There are two differences compare to their work: (1) we only repair RHS attribute values; (2) when update a cell value, we also consider the synonym values exist in the ontology under the selected sense. Apart from these two points, the others are same.} and verify that the number of data repairs are within $\tau$. 

\eat{
\fei{see questions below and summarized above.}\textcolor{gray}{
(1) find all ontology repair candidates, denoted by $|Cand(S)|$, that that are not captured by each equivalence class w.r.t. the selected sense via synonymous; (2) search each $k$-combinations ($k = 0, 1, ..., |Cand(S)|$) of ontology repair candidates to evaluate the minimal number of data repairs that is required. To effectively enumerate the combinations of candidate values to add to $S$, we model the sets of values as a set-containment lattice (Section~\ref{sec:beamsearch}), and traverse the lattice using a beam-search strategy~\cite{lowerre}; (3) To evaluate the minimal number of data repairs, we adopt and extend \fei{What is your extension that you say you extend?} the FD repair algorithm from Beskales et. al.~\cite{BIGG13} to OFDs. We model error tuples within each equivalence class using a conflict graph, and annotate the graph edges with the violated OFDs and sense(s).  Beskales et. al. show that the minimum number of required data changes to $I$ to achieve consistency can be approximated by computing the minimum vertex cover of the conflict graph;  (4) for each $k$-combinations of ontology repair candidates, we first compute $S'$ by inserting the corresponding ontology repair candidates into $S$ such that the candidates lead to the minimal number of data repairs and the number is less than $\tau$. After that, we adapt data repair algorithm \fei{what adapation?} to compute the repair value for a cell from the current attribute domain or from synonyms in $S$ under the selected sense.}  \fei{If this is simply applying their alg. I will just say this.} 
}
%Ontology repair module consists of three sub-modules: (1) \lit{Find candidates}. For each equivalence class $x \in \Pi_{X}(I)$, and all violating tuples $t_{err} \in x$, let $Cand(S)$ represent all error values $t_{err}$[A] in $I$ but not in $S$, i.e., these values consist of ontology repair candidates for insertion into $S$; (2) \lit{Search $k$-combinations}. We model the repair search via a set-containment lattice where we start the search at the (empty) root node, and nodes at level-$k$ contain $k$ values to be added to the ontology.  A node at level $k$ is created by appending a value to a node at level $k-1$.  We traverse the lattice using a beam search~\cite{lowerre} by expanding and exploring the most promising nodes, up to a fixed number $b$, called the beam size.  The idea is to select the top-$b$ best nodes to explore.  For each visited node (candidate ontology repair), we simulate adding the repair values to $S$ to obtain $S'$ and pass this to the data repair module, which approximates the minimal number of data repairs needed given $S'$;  (3) \lit{Find ontology repair}. We select the ontology repair with the fewest number of data repairs, and add this to the set of Pareto-optimal solutions.  


%\fei{Please re-write the below to be higher level giving the intuition.  What you have presented, again, is not well understood.  What is the conflict hypergraph, ppl may not have read the other paper, what is V-instance repair?  Describe your process generally.  See my above text on ontology repair.  Moved complexity to end of all algorithms (before experiments).}

% \noindent \cyan{\textbf{Data Repair.} \eat{Data may change and become stale as time evolves. In this case, \emph{Data Repair} modules propose a data repair approach to resolve the violations. }  We adopt and extend the FD repair algorithm from Beskales et. al.~\cite{BIGG13} to OFDs.  In \emph{Build Conflict Graph (CG)}, we model error tuples within each equivalence class using a conflict graph, and annotate the graph edges with the violated OFDs and sense(s).  Beskales et. al. show that the minimum number of required data changes to $I$ to achieve consistency can be approximated by computing the minimum vertex cover of the conflict graph.  In each iteration, after applying a certain of ontology repairs, the results of the minimum number of necessary data repairs will be passed to the \emph{Ontology Repair} module.  Lastly, in \emph{Find Repair}, we adapt the FD repair algorithm to compute the repair value for a cell from the current attribute domain or from synonyms in $S$ under the selected sense.}

%\fei{What is the novelty in contribution here for the data repair algorithm?  It sounds like you annotate the edges with the sense, and you consider a repair domain that includes synonyms (an expanded domain).  These sound like rather minor changes. Are there more significant algorithm contributions we can mention here?  What are the changes you had to made to consider only RHS repairs?  What is the change in complexity?  I'm looking for what the contributions and distinctions are in the data repair algorithm.}


% \blue{
% In the \lit{Build CH} sub-module, for a given ontology $S$ and a set of OFDs $\Sigma$, we take a similar approach to Beskales et. al.~\cite{BIGG13}, where we build a conflict graph that models the errors among the tuples within an equivalence class. Each conflict graph must be generated w.r.t. a given sense (more on this in Section~\ref{sec:ontrep}).  The minimum number of required data changes to achieve consistency can be approximated by computing the minimum vertex cover of the conflict graph.  In the \lit{Find Repair} sub-module, we compute the specific repair value for a cell, either from the current attribute domain or as a V-instance repair. 
% Computing the minimum number of changes to $I$ to obtain $I'$ such that $I' \models \Sigma$ w.r.t. $S'$ (denoted as  $\delta_{opt}(S', I')$) is NP-hard.  Computing the exact number of data repairs beyond a single FD is known to be NP-hard \cite{MinCost1}.  Since OFDs subsume FDs, our problem remains NP-hard. In the same spirit of \cite{BIGG13}, we use an approximation solution to compute the minimum number of data repairs to satisfy $\Sigma$.  Since we assume there is no overlap between LHS and RHS attributes of any pair of OFDs, and we only repair the RHS attribute values to resolve the violations. Thus, we modify the existing data repair algorithm in \cite{BIGG13} by only selecting the LHS attributes to the \lit{Fixed\_Attr} set instead of randomly selecting an attribute. Based on the modification, there exists a $P$-approximate upper bound on $\delta_{opt}(S', I')$, denoted $\delta_{P}(S', I')$, where the approximation ratio $P = 2 \times min\{|Z|, |\Sigma|\}$. Here, $|\Sigma|$ denotes the number of OFDs, and $|Z|$ denotes the number of (unique) RHS attributes in $\Sigma$.}




%\fei{You need to be very clear here about how your solution addresses the limitations stated earlier (right before 5.2.1). These points will be the novel parts of your solution. Currently, the text below reads as if it's the same as the existing algorithm by Lukasz et. al.  What are the unique contributions that are new?}

\eat{
\begin{algorithm}[t]
  \begin{small}
    \caption{Repair$\_$Data$\_$Ontology($I, \Sigma, S$)} \label{pc:repdataont}
    \begin{algorithmic}[1]
        \STATE obtain $S'$ from $\mathcal{P}(S)$ such that $\delta_{opt}(S', I) \leq \tau$ and no other $S'' \in \mathcal{P}(S)$ with $\delta_{opt}(S'', I) \leq \tau$ has $dist(S, S'') < dist(S, S')$. ( (ties are broken using $\delta_{opt}(S', I)$)
        \IF{$S' \neq \emptyset$}
            \STATE obtain $I'$ such that $I' \models \Sigma$ while performing at most $\delta_{opt}(S', I)$ cell changes.
            \RETURN $(S', I')$
        \ELSE
            \RETURN $(\emptyset, \emptyset)$
        \ENDIF
    \end{algorithmic}
  \end{small}
\end{algorithm}
}
% \eat{That is, $\delta_{opt}(S', I)$ $\leq$ $\delta_{P}(S', I)$ $\leq$ $P \times \delta_{opt}(S', I)$, for some constant $P$.}

% \blue{
% \definition[$P$-approximate $\tau$-constrained repair] Given an instance $I$, a set of OFDs $\Sigma$, an ontology $S$, and a threshold $\tau$, a $P$-approximate $\tau$-constrained repair $(S', I')$ is a repair such that $dist(I, I') \leq \tau$, and no other repair $(\mathcal{S''}, I'')$ has
% $(dist(S, \mathcal{S''}), P \times dist(I, I'')) ≺ (dist(S, S'), \tau)$.
% }

% \eat{We first present the architecture of our system, followed by the description of two modules: the ontology repair module and data repair module.}

% \blue{Figure~\ref{fig:framework} shows the OFDClean system architecture. Given a relation instance $I$, an ontology $S$, and a set of OFDs $\Sigma$, OFDClean returns a set of fixes to $I$ and $S$ such that $I \models \Sigma$.}

% \begin{figure}[ht!]
% \centering
%       \includegraphics[width=3.6in]{figures/Framework.pdf}
%      \vspace{-0.5cm}
%     \caption{OFDClean System Architecture. \fei{this needs updating.} \label{fig:framework}}
% \end{figure}

\eat{Based on the inputs, the {\em ontology repair} module contains two sub modules. For each OFD: $X \rightarrow_{syn} A$ or $X \rightarrow_{\theta} A$ w.r.t. the ontology $S$ (from $S$), the {\em potential candidates} module detects a set of values that exist in $A$ but not in $S$ as the potential candidates. For each value $q$ in the set, we use a word embedding technique (like \textit{word2vec}) to find the most relevant node $s$ in $S$. If the correlation between $q$ and $s$ is higher than a threshold and adding $q$ as the child of $s$ is a {\em safe} ontology repair, then the module keeps $q$ in $\textit{Cand}(S)$ as an ontology repair candidate.}


% \eat{In the {\em outer loop}, for each $k$ from $0$ to $|\textit{Cand}(S)|$, we select all $k$-combinations from $\textit{Cand}(S)$. Then for each $k$-combination, we repair $S$ with the $k$ selected values to create a new set of ontologies $S_k$, and the module in the {\em inner loop} returns a set of minimal data repairs $I_k$ \textit{w.r.t.} $S_k$. 
% Finally, for each $k$, we traverse all the repair pairs ($I_k, S_k$) and only keep the minimal repair as one solution.}

% \eat{In the {\em inner loop}, for each new set of ontologies $S_k$, our goal is to consider violations from all OFDs together and find the minimal data repairs. To achieve this goal, we extend an equivalence class based algorithm~\cite{BFFR05} to find the minimal data repairs based on OFDs.}

% \eat{An \textit{equivalence class} consists of a set E of cells. In an instance $I$, each cell $c$ has an associated equivalence class, denoted by $eq(c)$. For an equivalence class $x$, there exist a unique target value, denoted by $targ(e)$. Given a set of OFDs and ontologies $S$ with different senses, we build equivalence classes and find fixes as follows:}

\eat{
\begin{enumerate}
\item[(1)] \blue{Initialization. We create a set of unresolved tuples for each OFD, and put each cell $c$ involved in the OFD to the corresponding unresolved set. We also create a global equivalence set $\varepsilon$ to keep all the equivalence classes for all OFDs. Here, $\varepsilon$ is initialized with all the cells at the beginning.}
\item[(2)] \blue{Merge equivalence classes. For each OFD $X\rightarrow_{syn} A$ or $X\rightarrow_\theta A$ and an ontology S (with different senses), we find all set of tuples that have the same value in the LHS and try to find the one with minimum $mergcost$ to merge w.r.t. a target value.}
\item[(3)] \blue{Assign a target value. After finding the set of candidate tuples to merge (with minimum $mergcost$), we merge the cells of the attribute $A$ and update the $A$ values to the target value. For each cell that we have changed it's value, if there exists another OFD in which $A$ is associated with it's LHS, we add that cell to the correspondent unresolved set.}
\end{enumerate} 
\blue{We repeat the whole process until there is no remained cell in all the unresolved sets.}
}

% fei: redundant, already in paper text.
%For a given ontology $S$, We define two types of ontology functional dependency (OFD) over a relation instance $I$, which are synonym OFD and inheritance OFD. A synonym OFD $\phi_1$ is represented as $X \rightarrow_{syn} A$, where $X$ is a set of attributes and $A$ is a single attribute. Similarly, An inheritance OFD $\phi_2$ is represented as $X \rightarrow_{\theta} A$, where $\theta$ is a threshold representing the allowed path length between two nodes in $S$. By definition, a synonym OFD is a special case of an inheritance OFDs by setting $\theta = 0$, and we consider all the synonym values as one node in an ontology. 



\noindent\begin{minipage}{.5\textwidth}
  \centering
  \rule{0.3\textwidth}{0pt}
    \includegraphics[width=6.5cm]{figures/repairframework.pdf}
  \captionof{figure}{OFDClean framework.} \label{fig:repairframework}
\end{minipage}%
\begin{minipage}[ht]{.5\textwidth}
  \centering
  \rule{0.3\textwidth}{0pt}
    \includegraphics[width=6.5cm]{figures/ECG.pdf}
  \captionof{figure}{Sense assignment.} \label{fig:ecg}
\end{minipage}

==> discovery.tex <==
\section{Verifying OFDs}
 \label{sec:discovery}

In this section, we describe how we generate candidate OFDs, and present our algorithms to verify whether a candidate is a synonym or inheritance FD.  For clarity, we will refer to OFDs based on the synonym relationship as \emph{synonym FDs}, and OFDs based on the inheritance relationship as \emph{inheritance FDs}.  

\subsection{Generating Candidates}
Let an OFD candidate be of the form $O: X \rightarrow A$.  To find a complete, minimal set of OFDs, we test whether a candidate is either a synonym FD or an inheritance FD.  Based on our axiomatization for OFDs (Section~\ref{sec:foundations}), we normalize all OFDs to a single attribute consequent, i.e., $X$ $\rightarrow$ $A$ for any attribute $A$.   A candidate $O$ is non-redundant if its attribute sets $X, A$ are not supersets of already discovered dependencies.  The set of possible antecedent and consequent values is the collection of all attribute sets, which can be modeled as a set containment lattice.  Each node in the lattice represents an attribute set and an edge exists between sets $X$ and $Y$ if $X$ $\subset$ $Y$ and $Y$ has exactly one more attribute than $X$.  For a node $X$, we consider candidate OFDs of the form $(X \setminus A) \rightarrow A$, where $A \in X$.
We define $k$ to represent the number of levels in the lattice.  A relation with $n$ attributes will generate a $k = n$ level lattice, with $k = 0$ representing the top (root node) level.  For brevity, Figure \ref{fig:lattice} shows the search lattice for 4 of the 5 attributes in Table \ref{tab:example}.

\begin{figure}[t]
\centering
       \includegraphics[width=2.6in]{figures/lattice.pdf}
         \vspace{-0.3cm}
    \caption{Search lattice. \label{fig:lattice}}
    	\vspace{-0.3cm}
\end{figure}

After computing the partitions $\Pi_{A}, \Pi_{B} \dots$ for single attributes at level $k = 1$, we efficiently compute the partitions for subsequent levels in linear time by taking the product, i.e., $\Pi_{AB}$ = $\Pi_{A} \cdot \Pi_{B}$.  Each candidate is evaluated by traversing the lattice in a breadth-first search manner.  We consider all $X$ consisting of single attribute sets, followed by all 2-attribute sets, and continue level by level to multi-attribute sets until (potentially) level $k$ = $n$ similarly as for other useful use cases of Apriori~\cite{AMW96} such as TANE.  The algorithm efficiency is based on leveraging the work done in previous levels to prune descendant nodes that are supersets of discovered OFDs.   \eatTR{We reduce the search space by avoiding the evaluation of these descendant nodes, thereby saving considerable computation time.}

%We describe the necessary criteria for a candidate to qualify as a synonym or inheritance FD next.
%*******************************************************

\subsection{Synonym FDs}
\label{sec:synFD}
Given an ontology $S$, two concepts $c_{1}$ and $c_{2}$ in $S$ are synonyms if they are semantically equivalent.  Given an input relational instance $I$, ontology $S$, candidate $O:$ $X \rightarrow_{syn} A$, we present an algorithm that verifies whether each value in $X$ corresponds to either equal or synonymous values in $A$ under some common class (sense).  If this is true, then $O$ holds over $I$.  We assume that the partitions for each attribute set $X$, $\Pi_{X}$, and the \emph{names($C$)} are given.  

In Algorithm \ref{alg:syn}, \emph{CheckSynonymFD}, for each equivalence class in $\Pi_{X}$, and all tuples within the equivalence class (representing value $x$), we check whether each corresponding value in $A$ maps to a common class (sense).  If this is true, for all tuples in all equivalence classes, then $O$ holds over $I$.  Otherwise, if there exists a tuple with a value not synonymous (semantically equivalent) to other tuples within the same class, then we have found a non-synonymous value.  The candidate $O$ is then considered in the next $k+1$ level of the search lattice by  expanding $X$ with an additional attribute, $((X \cup B) \rightarrow_{syn} A$).  

\begin{algorithm}[t]
\begin{small}
\begin{algorithmic}
%\begin{footnotesize}
\STATE  \textbf{INPUT} $I$, $S$, $\Pi_{X}$, \emph{names()} \\
%, synFDs = \{\} 
%\end{footnotesize}
\end{algorithmic}
%\begin{algorithmic}[1]
%\begin{small}
%\FOR {each $k$}
%       \FOR {each $\Pi_{X}$}
%        \FOR {each $C_{A}$}
%        \STATE bFoundOFD = computeOverlap($\Pi_{X}, C_{A}$)
%%        \STATE processNext(bFoundOFD, synFDs);
%        \IF {bFoundOFD}
%          \STATE synFDs += \{$X \rightarrow_{syn} A$\} where $A \in (R \setminus X)$
%          \STATE prune candidates $XY \rightarrow_{syn} A, \forall Y \subseteq (R \setminus X)$    \footnotemark{}
%          \ENDIF
%        \ENDFOR
%     \ENDFOR
%%   \ENDFOR
%   \STATE \textbf{return} synFDs

%\end{small}
%\end{algorithmic}
%\medskip

%\begin{algorithmic}
%\STATE { \textbf{computeOverlap}$(\Pi_{X},C_{A})$}
%\end{algorithmic}
\begin{algorithmic}[1]
\STATE $g_{x}[X]$ = \{ $t$ $|$ $t$ $\in$ $I$ and $t[X]$ $=$ $x$ \}
\FOR {each $x \in \Pi_{X}(I)$}
%\STATE $v = \Pi_{A}(g_{x}[X])$
\STATE {$t =  \Pi_{A}(g_{x}[X])$, so $t = (t_{1}, t_{2}, \ldots , t_{m}$)}
%\IF {names($C_{t_{1}} \cap C_{t_{2}} \ldots \cap C_{t_{m}} = \emptyset$) }
\IF {names(${t_{1}}$) $\cap$ $\ldots$ $\cap$ names(${t_{m}}$) = $\emptyset$}       \label{line:synchk}
%\STATE \COMMENT{the values in the equivalence class are not synonyms nor equal}
   \STATE \textbf{return} false
\ENDIF
\ENDFOR
   \STATE \textbf{return} true
\end{algorithmic}
\caption{CheckSynonymFD \label{alg:syn}}
\end{small}
\end{algorithm}
\begin{table} \vskip -0.6cm \end{table}
%\footnotetext{\small We apply further optimizations as described later.}



%*********************************************************

% 3 figures spread across horizontally
%\begin{figure*}[!htb]
%\minipage{0.22\textwidth}
%    \vskip -0.25cm
%    \includegraphics[width=1.8in]{figures/lattice.pdf}
%    \caption{Search lattice. \label{fig:lattice}}
%    \vspace{-0.4cm}
%\endminipage\hfill
%\minipage{0.22\textwidth}
%  \includegraphics[width=1.8in]{figures/clinical.pdf}
%  \vskip -0.2cm
%  \caption{Scalability in N.}\label{fig:clinical}
%\endminipage\hfill
%\minipage{0.22\textwidth}%
% \includegraphics[width=1.8in]{figures/levelsbar.pdf}  
% \vskip 0.4cm
%\caption{Runtime per level. \label{fig:level}}
%\endminipage\hfill
%\end{figure*}


% 3 figures in a minipage



%*************************************************************

% This needs further explanation, what does "not good" mean?  Removed for now.
%\textbf{\textit{Definition 3.2.1.}} \\*
%\noindent\rule[0.5ex]{\linewidth}{1pt}
%The composition of RHS does not hold for OFDs like FDs. For example, if $A$ $\rightarrow$ $B$ and $A$ $\rightarrow$ $C$, then $A$ $\rightarrow$ $BC$ for FDs, but does not hold good for OFDs. \\*
%\noindent\rule[0.5ex]{\linewidth}{1pt} \\*


%The following definition formalizes this intuition.
%\begin{definition}
%A synonym FD $X \rightarrow_{syn} A$  holds over a relational instance $I$ if for each $x$ $\in$ $\Pi_{X}(I)$, there exists a class C, such that $\Pi_{A}(g_{x}[X])$ $\subseteq$ synonym$(C)$, where $g_{x}[X]$ = \{$t| t \in I$ and $t[X] = x$\}.
%\end{definition}



\begin{example}\label{example:syn}
Consider candidate $O$:  [CC]  $\rightarrow_{syn}$  [CTRY]  from Table \ref{tab:example}.  We have $\Pi_{CTRY}$ = \{\{$t_1$\}\{$t_2,t_7$\}\{$t_3$\}\{$t_4$\}\{$t_5$\}\{$t_6\}$\} and $\Pi_{CC}$ = \{\{$t_1,t_5,t_6$\}\{$t_2,t_4,t_7$\}\{$t_3$\}\}.  We consider each equivalence class in $\Pi_{CC}$.  The first class, \{$t_1,t_5,t_6$\}, representing the value `US' corresponds to three distinct values in CTRY.   We check the names(`United States') $\cap$ names(`America') $\cap$ names(`USA').  According to a given ontology $S$, the values resolve to a non-empty value indicating the three references are to the same country.  Similarly, the second class \{$t_2,t_4,t_7$\} corresponds to names(`India') $\cap$ names(`Bharat') = `India'.  The last equivalence class \{$t_3$\} contains a single tuple, thus, there is no conflict.  Since we have resolved all references in CTRY to either equal or synonymous values, $O$ holds over Table \ref{tab:example}.
%A variation that considers two senses, where the value 'India' applies under sense $s_{1}$ and 'Bharat' applies under sense $s_{2}$ would cause $F$ to not be satisfied, since the values in the equivalence class $x_{2}$ = \{2,4,7\} would not share a common sense.
\end{example}

In Section \ref{sec:foundations}, we present details of our overall algorithm to discover OFDs, called \emph{FASTOFD}, that invokes \emph{checkSynonymFD} and \emph{checkInheritanceFD} (details in Section \ref{sec:inhFD}).



%*************************************************************
\subsection{Inheritance FDs}
\label{sec:inhFD}
Given an ontology $S$, two concepts $c_{1}$ and $c_{2}$ participate in an inheritance relationship if $c_{1}$ and $c_{2}$ have common ancestor. \eatTR{, or equivalently, $c_{1}$ is a superclass of $c_{2}$}.   Given an instance $I$, ontology $S$, and candidate $O: X \rightarrow_{\theta} A$, Algorithm \ref{alg:inherit}, \emph{CheckInheritanceFD}, determines whether $O$ is an inheritance OFD over $I$ if for every equivalence class, the corresponding values in $A$ all share a common ancestor.  Clearly, if we search high enough in $S$, we can always find a common ancestor.  However, we would like to find values in $S$ that are closely related to the values in $A$.  Hence, we define a topological constraint over $S$ that considers a restricted version of inheritance that computes the \emph{least common ancestor (LCA)} between all values in $\Pi_{A}(g_{x}(X))$, and requires the distance between each of the values, and the LCA, to be within a distance of $\theta$.


%\begin{definition}
%An inheritance FD $\emph{X}$ $\rightarrow_{\theta}$ $\emph{A}$ holds over $I$ if for each $x$ $\in$ $\Pi_{x}(I)$, there exists a class $C$, such that $\Pi_{A}(g_{x}[X])$ $\subseteq$ $ancestors(C)$, where $g_{x}[X]$ = \{$t$ $|$ $t$ $\in$ $I$ and $t[X]$ $=$ $x$\}.  In addition, for each $v \in \Pi_{A}(g_{x}[X])$, distance($v$, LCA) $\leq \theta$ in $S$.
%\end{definition}

%*************************************************************

Verifying whether a candidate inheritance FD holds over $I$ proceeds in a similar manner as Algorithm \ref{alg:syn}.  The difference is we identify values that participate in an inheritance relationship within a distance of $\theta$ in $S$.  In Algorithm \ref{alg:inherit}, for each equivalence class in $\Pi_{X}$, we identify the corresponding values in $\Pi_{A}$.  For each of these equivalence classes in $\Pi_{A}$, we compute the least common ancestor among all its tuples $t$.  If the distance between each $t$ and the LCA is within the threshold $\theta$, then the candidate $X \rightarrow_{\theta} A$ holds.

\begin{example}\label{example:isa}
Consider candidate $O: X \rightarrow_{\theta} A$: [SYMP, DIAG] $\rightarrow_{\theta}$ [MED], and the ontology in Figure \ref{fig:ontology}.
For each $x \in  \Pi_{X}$ = \{\{$t_1,t_2,t_3$\}\{$t_4,t_5,t_6$\}\{$t_7$\}\}, we identify the corresponding values in $\Pi_{A}(g_{x}(X))$.  For $x_{1}$ = \{$t_1,t_2,t_3$\} and $x_{4}$ = \{$t_4,t_5,t_6$\}, the LCA is `analgesic'.  Suppose $\theta = 2$, all values in $\Pi_{A}(g_{x}(X))$ are within a distance of $\theta$, e.g., distance(`ibuprofen', `analgesic') = distance(`tylenol', `analgesic') = 2.  Hence, for $\theta = 2$, $O$ holds.
\end{example}

\begin{algorithm}[t]
\begin{small}
\begin{algorithmic}
%\begin{footnotesize}
\STATE  \textbf{INPUT} $I$, $S$, $\Pi_{X}$, $\theta$, \emph{descendants()} \\
%\end{footnotesize}
\end{algorithmic}
\begin{algorithmic}
\STATE { \textbf{computeLCA}$(\Pi_{X},C_{A})$}
\end{algorithmic}
\begin{algorithmic}[1]
\STATE $g_{x}[X]$ = \{ $t$ $|$ $t$ $\in$ $I$ and $t[X]$ $=$ $x$ \}
\FOR {each $x \in \Pi_{X}(I)$}
%\STATE $v = \Pi_{A}(g_{x}[X])$
\STATE {$t =  \Pi_{A}(g_{x}[X])$, so $t = (t_{1}, t_{2}, \ldots , t_{m}$)}
\STATE \%function LCA returns distance number to least common ancestor
\IF {LCA(descendants(names(${t_{1}}$)) \ldots descendants(names(${t_{m}})) > \theta$) }
%\STATE \COMMENT{the data values are not within a distance of $\theta$ in $S$}
   \STATE \textbf{return} false
\ENDIF
%\ENDFOR
\ENDFOR
   \STATE \textbf{return} true
\end{algorithmic}
\caption{CheckInheritanceFD \label{alg:inherit}}
\end{small}
\end{algorithm}
\begin{table}\vspace{-0.8cm}\end{table}




==> document.tex <==
\section{Introduction}\label{sec:introduction}
In the previous work, we address the problem of discovering a complete, minimal (non-redundant) set of synonym and inheritance OFDs for the given relational instance and ontology. However, the data (and/or the ontology) may change over time which makes the OFDs are not held anymore, and it is often unclear whether the data is incorrect or whether the ontology is incorrect (or both).

\blue{For example, the Food and Drug Administration (FDA) of the USA approves novel drugs every month while the drug ontology is updated with delay~\cite{Dron}. Therefore, to ensure the data consistency w.r.t. the set of discovered OFDs, there is a need for a data cleaning framework to repair data and ontology that can respond to this change.}  \fei{What change?  How is it caused?  What consistency?}  For the ontology repair, we only consider insertions (i.e., add new nodes/senses to the ontology). 

\blue{This is because the existing ontology is often generated by the experts in a specific domain, and the ontology is already verified by the historical data for a long time.}  \fei{You are assuming that once data is in the ontology it is correct (bc is human verified), so all the more reason to be clear on what kind of changes we are assuming and then what kind of updates we allow to the ontology.  Also be clear about the changes to the data.}


\subsection{Contributions}
In this work, for a given set of OFDs, we address a data cleaning problem in which a dataset that violates the specified OFDs \textit{w.r.t.} a set of ontologies, and we return multiple non-redundant suggestions for how to modify the data and/or ontologies in order to achieve consistency \textit{w.r.t.} the OFDs. \fei{is it always multiple?  What does non-redundant mean?} \morteza{We tried to use the sentence from the relative trust paper. because we are suggesting some Pareto-optimal solutions. non-redundant refers to Pareto-optimality.} We make the following contributions:

\begin{enumerate}
\item We define the OFD-repair problem w.r.t. an ontology $O$, and define a space of minimal data and ontology repairs based on dominance \textit{w.r.t.} the number of updates to the data and to $O$.
Our solution returns multiple non-redundant suggestions for how to modify the data and/or ontologies to achieve consistency \textit{w.r.t.} the OFDs.

\item \blue{We propose a framework for finding minimal data repair such that no more than $\tau$ ontology modifications will be required to make the data satisfy the given OFDs \textit{w.r.t.} the modified ontology.} 
% \item We propose an algorithm for finding minimal changes to a set of ontologies such that no more than $\tau$ data changes will be required to satisfy the given OFDs \textit{w.r.t.} the modified ontologies.
\end{enumerate}






%\section{Related Work}
% \noindent\textbf{Dependency Discovery.} There are many works to mine all kind of dependencies over a relation. These works including discovery of functional dependencies (FDs) \cite{huhtala1999tane,lopes2000efficient,wyss2001fastfds,wang2009functional,abedjan2014dfd}, conditional functional dependencies (CFDs) \cite{chiang2008discovering,golab2008generating,fan2011discovering}, differential dependencies (DDs) \cite{song2011differential}, matching dependencies (MDs) \cite{song2013efficient}, conditional inclusion dependencies (CINDs) \cite{bravo2007extending}, denial constraints (DCs)\cite{chu2013discovering} and ontology functional dependencies (OFDs) \cite{baskaran2017efficient}. Our current work is not about discovering dependencies in a relation, but we are going to repair the data and ontology with OFDs.\\



==> experiments_old.tex <==
\section{Experiments}
\label{sec:eval}

We now turn to the evaluation of our techniques using real datasets.  Our evaluation focuses on four objectives:

\begin{enumerate}
\item An evaluation of scalability and performance as compared to existing FD discovery algorithms.  We compare our algorithm against seven existing techniques as we scale the number of tuples and the number of attributes. 
\item An evaluation of the performance benefits of our proposed optimization techniques to prune redundant OFD candidates.
\item An evaluation of the efficiency of our algorithm to identify interesting dependencies early on during the lattice-based traversal.  We measure efficiency in terms of running time and the size of the OFDs discovered at each level of the lattice.
\item A qualitative evaluation of the utility of the discovered OFDs.
\item \fei{evaluation of our new contribution...}
%measuring the accuracy of the discovered OFDs.  We quantify accuracy in terms of precision and recall against a ground truth data set with known synonyms and inheritance relationships.
\end{enumerate}

Our experiments were performed using four Intel Xeon processors at 2.1GHz each with 32 GB of memory.  All algorithms were implemented in Java.  The reported runtimes are averaged over six executions.  For  the comparative experiments, we use the Metanome implementations of existing FD discovery algorithms %provided by the Metanome profiling platform 
\cite{PBF+15}. 


% Data Characteristics
\subsection{Data Characteristics}
We use two real datasets.  The first dataset is obtained from the Linked Clinical Trials (LinkedCT.org) database.  
%The LinkedCT.org project provides an open interface for international clinical trials data 
We use 1M records (15 attributes) including data about the study, country, medical diagnosis, prescribed drugs, illnesses, symptoms, treatment, and outcomes.  The second dataset contains US census data (collected from http://census.gov/) with population properties such as work class, marital status, race, relationship, occupation, and salary.  We use a portion of this dataset that contains 150K records with 11 attributes.  In all our experiments, we refer to the U.S. National Library of Medicine Research \cite{medOntology}, and WordNet ontologies.  


%\begin{figure}[!h]
%\centering
%\minipage[t]{0.5\linewidth}
%   \centering
%         \includegraphics[width=1\textwidth]{figures/clinical.pdf}
%%  \vskip -0.2cm
%  \caption{Scalability in N.}\label{fig:clinical}
%  %  \vspace{-0.4cm}
%\endminipage\hfill
%\minipage[t]{0.5\linewidth}
%  \centering
%  \includegraphics[width=1.8in]{figures/levelsbar.pdf}
%\caption{Runtime per level. \label{fig:level}}
%\endminipage\hfill
%\end{figure}


%*********************************************
%performance
\subsection{Scalability}
\textbf{Experiment-1: Comparative Scalability in Number of Tuples.}  We evaluate the scalability of our algorithm with respect to the number of tuples ($N$) against seven existing FD discovery algorithms: TANE \cite{HKPT98}, FUN \cite{NC01}, FDMine \cite{YH08}, DFD \cite{ASN14}, DepMiner \cite{LPL00}, FastFDs \cite{WGR01}, and FDep \cite{FS99}.  Figure \ref{fig:clinical} and Figure \ref{fig:census} show the running times using the clinical trials (with 15 columns) and census (11 columns) datasets, respectively, using $\theta = 5$ for each attribute.  In Figure \ref{fig:clinical}, we report partial results for FDMine and FDep as both techniques exceeded the main memory limits.  Similar to previous studies, we found that FDMine returns a much larger number of non-minimal dependencies, about 24x (for clinical) and 118x (for census) leading to increased memory requirements \cite{ASN14}.   We ran DepMiner and FastFDs using 100K records and report running times of 4hrs and 2.3 hrs, respectively. However, for larger data sizes (200K+ records), we terminated runs for these two techniques after 12 hours; hence they do not appear in Figure \ref{fig:clinical}.  
For the smaller census data, Figure \ref{fig:census} shows that our techniques outperform  FastFDs, DepMiner, and FDep, since these three techniques scale quadratically with respect to the number of tuples.

The running times of FASTOFD scale linearly with the number of tuples, similar to other lattice based approaches (TANE, FUN, and DFD).  We achieve this linear runtime since we index the values in the ontology (recall Section \ref{sec:complexity}).  
%The runtime is dominated by data verification of OFDs. 
%For our chosen datasets, we found there was a large number of smaller equivalence classes, which lead to the decreased verification time that dominated the overall running time. 
As expected, discovering OFDs incurs an increased runtime.  We found that discovering synonym and inheritance OFDs incur an average overhead of 1.8x and 2.4x, respectively, over existing lattice-traversal FD discovery algorithms.  This can be explained by the inherent complexity of OFDs (which subsume FDs), and the increased number of discovered OFDs. For example, in the clinical data, many illnesses and medications are referenced by multiple names but refer to the same entity; e.g., a drug can be referred to by its generic name or its brand name.  
%Given the increased number and increased complexity of OFDs, FASTOFD discovers these dependencies within reasonable time bounds from existing solutions.

\eatTR{
Similar to previous studies, we found that FD
Our techniques show a linear scale-up w.r.t. the number of tuples, with the majority of time dominated by verification of OFDs.  For our chosen datasets, we found there was a large number of smaller equivalence classes, which lead to the decreased verification time that dominated the overall running time.  Our techniques outperform TANE by an average of 19.5\%, and we observed that our clinical trials dataset contained 3x more satisfying OFDs versus FDs, since many illnesses and medications are referenced by multiple names but refer to the same entity, e.g., a drug can be referred to by its generic name or its brand name.   We observe that discovering inheritance FDs incurs an average of 7.1\% overhead than discovering synonym FDs.  For inheritance FDs, we need to traverse the ontology to find the least common ancestor within a path length of $\theta$.  In contrast, the verification of a synonym FDs requires checking for a non-empty intersection among a set of values, which can be done in constant time.
}

\textbf{Experiment-2: Comparative Scalability in the Number of Attributes.}   We evaluate FASTOFD's scalability with the number of attributes ($n$), using $N$ = 100k tuples, and $\theta = 5$.  Figures \ref{fig:numattrs} and \ref{fig:numattrs2} show  the running times using the clinical trials and census datasets, respectively.  All algorithms scale exponentially w.r.t. the number of attributes since the space of candidates grows with the number of attribute set combinations.  FASTOFD scales comparatively with other lattice based approaches.  Our solution discovers 3.1x more dependencies on average (this includes synonym OFDs, inheritance OFDs, and traditional FDs since they are subsumed by OFDs), compared to existing approaches, validating the overhead we incur.  In Figures \ref{fig:numattrs} and  \ref{fig:numattrs2}, we report partial results for DepMiner, FastFDs, and FDep (before memory limits were exceeded), where we achieve almost two orders of magnitude improvement due to our optimizations.  Similar to existing lattice-based approaches, our techniques perform well on a smaller number of attributes due to effective pruning strategies that reduce the search space.  

\eatTR{
As expected, we saw an exponential scale-up in running time w.r.t. the number of attributes.  This is not surprising given that the number of minimal OFDs over the attribute lattice is exponential in the worst case. 
A larger number of inheritance versus synonym FDs are found, leading to the increased running time.  We observe that the execution time more than triples from $n = 7$ to $n = 15$ for clinical data, and more than 5x from $n = 7$ to $n = 11$ for census data, due to the increased number of attribute combinations, and consequently, the larger search space of candidates that must be evaluated.   
}




\begin{figure*}
\begin{minipage}[t]{0.25\textwidth}
\centering
\includegraphics[width=4.3cm]{./figures/NClinical2.pdf}
\vspace{-2mm}
\caption{Scalability in N (clinical).}
\label{fig:clinical}
\end{minipage}%
\hspace{-0.1in}
\begin{minipage}[t]{0.25\textwidth}
\centering
\includegraphics[width=4.3cm]{./figures/NCensus2.pdf}
\vspace{-2mm}
\caption{Scalability in N (census).}
\label{fig:census}
\end{minipage}
\hspace{-0.15in}
\begin{minipage}[t]{0.25\textwidth}
\centering
\includegraphics[width=4.3cm]{./figures/numAttrsClinical2.pdf}
\vspace{-2mm}
\caption{Scalability in $n$ (clinical).}
\label{fig:numattrs}
\end{minipage}%
\hspace{-0.1in}
\begin{minipage}[t]{0.25\textwidth}
\centering
\includegraphics[width=4.3cm]{./figures/numAttrsCensus2.pdf}
\vspace{-2mm}
\caption{Scalability in $n$ (census).}
\label{fig:numattrs2}
\end{minipage}
\vspace{-2mm}
\end{figure*}

\begin{figure}
\begin{minipage}[t]{0.24\textwidth}
\centering
\includegraphics[width=4.4cm]{./figures/opt2.pdf}
\vspace{-5mm}
\caption{Impact of Opt-2.}
\label{fig:opt2}
\end{minipage}%
\hspace{0in}
\begin{minipage}[t]{0.24\textwidth}
\centering
\includegraphics[width=4.4cm]{./figures/opt2.pdf}
\vspace{-5mm}
\caption{Impact of Opt-3,4.}
\label{fig:opt34}
\end{minipage}
\end{figure}




% \begin{figure*}[ht]
% \centering
% %**************************
% %\minipage[b]{0.3\linewidth}
% %  \centering
% %  \includegraphics[width=1.8in]{figures/NClinical.pdf}
% %    \vspace{-0.3cm}
% %  \caption{Scalability in N (clinical data).}\label{fig:clinical}
% %\endminipage\hfill
% %\minipage[b]{0.3\linewidth}
% %  \centering
% %  \includegraphics[width=1.8in]{figures/NClinical.pdf}
% %    \vspace{-0.3cm}
% %  \caption{Scalability in N (clinical data).}\label{fig:clinical}
% %\endminipage\hfill
% %\minipage[b]{0.3\linewidth}
% %  \centering
% %  \includegraphics[width=1.8in]{figures/NClinical.pdf}
% %    \vspace{-0.3cm}
% %  \caption{Scalability in N (clinical data).}\label{fig:clinical}
% %\endminipage\hfill

% %**************************

 
% %*******************************
% \minipage[b]{0.3\linewidth}
%   \centering
%   \includegraphics[width=1.8in]{figures/NClinical2.pdf}
%   \vspace{-0.3cm}
%   \caption{Scalability in N (clinical).}\label{fig:clinical}
% \endminipage
% \minipage[b]{0.3\linewidth}
%   \centering
%   \includegraphics[width=1.8in]{figures/NCensus2.pdf}
%   \vspace{-0.3cm}
% \caption{Scalability in N (census). \label{fig:census}}
% \endminipage
% \minipage[b]{0.3\linewidth}
%   \centering
%  \includegraphics[width=1.8in]{figures/numAttrsClinical2.pdf}
%  \vspace{-0.3cm}
%   \caption{Scalability in $n$ (clinical).}\label{fig:numattrs}
%   \endminipage\hfill
%   %%
%   \minipage[b]{0.3\linewidth}
%   \centering
%  \includegraphics[width=1.8in]{figures/numAttrsCensus2.pdf}
%  \vspace{-0.3cm}
%   \caption{Scalability in $n$ (census).}\label{fig:numattrs2}
%  \vspace{-0.3cm}
% \endminipage
% \minipage[b]{0.3\linewidth}
%   \centering
%   \includegraphics[width=1.8in]{figures/opt_augment2.pdf}
%  \vspace{-0.3cm}
%   \caption{Impact of Opt-2.}\label{fig:opt2}
%   \vspace{-0.3cm}
% \endminipage
% \minipage[b]{0.3\linewidth}
%   \centering
%  \includegraphics[width=1.8in]{figures/opt_keys.pdf}
%  \vspace{-0.3cm}
%   \caption{Impact of Opt-3.}\label{fig:opt3}
%   \vspace{-0.3cm}
%   \endminipage\hfill
% %%
% %   \minipage[b]{0.3\linewidth}
% %   \centering
% % \includegraphics[width=1.9in]{figures/opt_disc.pdf}
% % \vspace{-0.3cm}
% %  \caption{Impact of Opt-4.}\label{fig:opt4}
% %   \endminipage
% %   \minipage[b]{0.3\linewidth}
% %   \centering
% %  \includegraphics[width=1.5in]{figures/recall.pdf}
% % \vspace{-0.3cm}
% %  \caption{Recall.}\label{fig:recall}
% %   \endminipage
% %   \minipage[b]{0.3\linewidth}
% %   \centering
% %  \includegraphics[width=2.0in]{figures/ofdclean1.pdf}
% % \vspace{-0.3cm}
% %  \caption{Synonym and inheritance values found per level.}\label{fig:ofdclean1}
% %   \endminipage\hfill
   
% \end{figure*}

%**********************************************
\begin{figure*}[ht!]
\centering
  \minipage[b]{0.3\linewidth}
  \centering
  \includegraphics[width=6cm]{./figures/levelsbar.pdf}
\caption{Runtime per level. \label{fig:level}}
  \endminipage
  \hspace{0.5cm}
      \minipage[b]{0.3\linewidth}
  \centering
  \includegraphics[width=6cm]{figures/ofdclean1.pdf}
  \caption{Synonym and inheritance values found per level.}\label{fig:ofdclean1}
  \endminipage
  \hspace{0.5cm}
  \minipage[b]{0.3\linewidth}
  \centering
  \includegraphics[width=6cm]{figures/ofdclean2.pdf}
  \caption{Number of approximate OFDs vs. support.}\label{fig:ofdclean2}
  \endminipage\hfill
\vspace{-3mm}
   
\end{figure*}

%*********************************************

\subsection{Optimization Benefits}
\label{sec:opt}
We now evaluate the efficiency of our optimizations using the clinical trials dataset.  We focus our evaluation on \emph{Optimizations 2, 3} and \emph{4 (Opt-2, Opt-3, Opt-4)}. Recall that for $O: X \rightarrow A$, \emph{Optimization 1} prunes trivial dependencies where $A \in X$.   Our lattice based search does not consider candidates where $A \in X$, so we do not generate trivial dependencies.   \emph{Opt-2} prunes candidates containing a superset of $X$ if $O$ already holds over $I$.  \emph{Opt-3} and \emph{Opt-4} avoid checking whether $O$ is an OFD if $X$ is a key or $O$ is found to be a traditional FD, respectively.  We use 500K tuples from the clinical trials dataset.  Our optimizations achieve significant performance improvements.  For instance, at 100K tuples, Opt-4 reduces running times by 59\%.

\textbf{Experiment-3: Pruning Non-Minimal OFDs (Opt-2).}  Figure \ref{fig:opt2} shows the running times of our discovery algorithm with and without Opt-2 implemented, labeled as `FASTOFD\_optimized' and `FASTOFD', respectively.  Opt-2 achieves an average 31\% improvement in running time due to the aggressive pruning of redundant candidates at  lower lattice levels.
%, saving considerable computation time.  

\textbf{Experiment-4: Exploiting Keys (Opt-3).} Figure \ref{fig:opt34} shows the running times to evaluate Opt-3.  As expected, we see a smaller performance improvement (compared to Opt-2) since we reduce the verification time due to existence of keys, rather than pruning candidates.  We found two key attributes in the clinical data: (1) \texttt{NCTID} representing the clinical trials.gov unique identifier for a clinical study; and (2) \texttt{OrgStudyID}, an identifier for a group of related studies.  Opt-3 achieves an average 14\% improvement in running time.  Given the existence of more keys, we would expect to see a greater improvement in running time.  

\textbf{Experiment-5: Exploiting FDs (Opt-4).} Similarly, Figure \ref{fig:opt34} shows the evaluation for Opt-4.  Since the original dataset did not have any FDs that were satisfied over the entire relation,  we modified the data to include five FDs: 
%\begin{itemize}
	F1: overall\_status $\rightarrow$ number\_of\_groups, 
	F2: study\_design $\rightarrow$ study\_type,
    F3: [condition, time\_frame] $\rightarrow$ measure,
  F4: [safety\_issue, study\_type] $\rightarrow$ eligibility\_minimum\_age, 		
F5: [condition, country] $\rightarrow$ drug\_name.
%\end{itemize}
%\begin{enumerate}[noitemsep]
%\item[F1:] overall\_status $\rightarrow$ number\_of\_groups
%\item[F2:] study\_design $\rightarrow$ study\_type
%\item[F3:] [condition, time\_frame] $\rightarrow$ measure
%\item[F4:] [safety\_issue, study\_type] $\rightarrow$ eligibility\_minimum\_age
%\item[F5:] [condition, country] $\rightarrow$ drug\_name
%\end{enumerate}
%
Given this set of FDs, the running times decrease by an average of 27\%.  We expect that the performance gains are proportional to the number of satisfying FDs in the data; more satisfying FDs leads to less time spent verifying candidate OFDs.  Overall, our optimizations achieve an average of 24\% improvement in running time, and our canonical representations are effective in avoiding redundancy.

%*********************************************
% Efficiency
\subsection{Efficiency}
%\textbf{Exp-2: Efficiency.}
\textbf{Experiment-6: Effectiveness over lattice levels.} 
We argue that compact OFDs (involving few attributes) are the most interesting.  OFDs with more attributes contain more unique equivalence classes.  Thus, a less compact dependency may hold but may not be very meaningful due to overfitting.  We evaluate the efficiency of our techniques to discover these compact dependencies.  To do this, we measure the number of OFDs, and the time spent, at each level of the lattice using the clinical trials data.  OFDs discovered at the upper levels (involving fewer attributes) are more desirable.
%than those discovered at the lower levels.  
Figure \ref{fig:level} shows the running time at each level of the lattice, and the total number of synonym and inheritance OFDs found at each level (labeled on top of the bars).  Table \ref{tab:countlvl} shows the breakdown for each type of OFD per level (missing levels indicate no OFDs found).

For synonym OFDs, approximately 61\% are found in the first 6 levels taking about 25\% of the total time.  For inheritance OFDs, 
%the results are a bit better, where 
63\% of the dependencies are found in the first 6 levels taking 16\% of the total time.  The remaining 35-40\% of dependencies (found in the lower levels) are not as compact, and the time to discover them would take well over 70\% of the total time.   Since most of the interesting OFDs are found at the top levels, we can prune the lower levels (beyond a threshold) to improve overall running times.  




%\hspace{2pt}
\begin{table}
  \centering
    \begin{tabular}{|c||c|c|}
       \hline
        level & synonym OFDs & inheritance OFDs \\
       \hline \hline
       1 & 5   & 5   \\
       2 & 4  & 6  \\
       4 & 3  & - \\
       6 & 4 & 7 \\
       8 & - & 1 \\
       9 & 5 & 5 \\
       11 & 3 & 4 \\
       14 & 2 & 2 \\
       \hline
   \end{tabular}
    \captionof{table}{Number of OFDs found per level.}
    \vskip -0.9cm
 \label{tab:countlvl}
 \end{table}

 
%*********************************************
%quality
\subsection{Qualitative Evaluation}
%As expected, our algorithms discover a larger number of dependencies than FD discovery algorithms as the space of values satisfying synonym and inheritance relationships subsumes values satisfying only equality.   In our comparative evaluation with TANE, our algorithms found 3x more dependencies than TANE.
\textbf{Experiment-7: Finding Interesting OFDs.} 
%To measure the accuracy of the discovered OFDs, we used clean versions of the data containing a known number of satisfying synonym and inheritance OFDs as the ground truth.  We then randomly injected 2\% error, and measured the precision and recall.  We found the discovered dependencies to be correct, and the recall values ranged between 70\%-80\%.  Figure \ref{fig:recall} shows the recall results for the clinical trials and census datasets. 
We now show that the OFDs we discovered are intuitive and relevant.
%We found the discovered OFDs to be intuitive and relevant.  
For example, in the census data, synonym OFD $O_{1}$: OCCUP $\rightarrow_{syn}$ SAL states that equivalent jobs earn a similar salary (with SAL being a categorical attribute representing salary levels).   In the clinical data, two examples are the inheritance OFD $O_{2}$: [SYMP, DIAG] $\rightarrow_{inh}$ DRUG, and the synonym OFD $O_{3}$: CONDITION $\rightarrow_{syn}$ DRUG.  In $O_{2}$, a set of symptoms and diagnosis leads to a prescribed treatment from the same drug family; e.g., a headache diagnosed as a migraine is prescribed ibuprofen (which is-a non-steroid anti-inflammatory drug) for pain relief.  In $O_{3}$, we found that specific medical conditions are treated with similar drugs, but the drug names vary across countries.  For example, \emph{fever} is treated with \emph{acetaminophen} in Canada, and with \emph{Paracetamol} in India.  The discovered dependencies re-affirm that many applications contain domain specific synonym and inheritance attribute relationships that go beyond equality, which are not currently captured by existing techniques.  In future work, we intend to explore the influence  of the parameter $\theta$ on the quality of discovered OFDs. 

% \begin{figure}[!h]
%\centering
%  \includegraphics[width=2.2in]{figures/recall.pdf}
% \vspace{-0.3cm}
%  \caption{Recall.}\label{fig:recall}
%\end{figure}

%\begin{table}[htbp]
%\centering
%\begin{tabular}{|c| c| c |}
%\hline
% & Clinical trials & Census \\
% \hline
%Synonym FD & 11 & 7 \\
%Inheritance FD & 14 & 10 \\
%TANE & 4 & 3 \\
%\hline
%\end{tabular}
%\caption {Number of discovered dependencies.}
%\label{tab:compare}
%\end{table}

%*********************************************
%OFD Data Cleaning
\subsection{Data Cleaning with OFDs}
\label{sec:ofdclean}
We now evaluate the utility of OFDs for data cleaning using the clinical data.  OFDs provide rich contextual information that is used to distinguish synonymous and inheritance values that are not syntactically equivalent but refer to the same entity.  In addition, approximate OFDs can identify potentially dirty data values, and provide recommendations of possible correct values for repair. 

\textbf{Experiment-8: Eliminating False-Positive Data Quality Errors.}
To quantify the benefits of OFDs versus traditional FDs, which are commonly used in data cleaning techniques, we aim to capture the value that OFDs provide, namely, the number of syntactically `non-equal' values referring to the same entity.   For example, under traditional FDs, a dependency \texttt{CTRY} $\rightarrow$ \texttt{CC}, with CTRY value `Canada' mapping to CC values `CA', `CAN', and `CAD', would all be considered as errors.  However, under a synonym OFD, these tuples are considered clean, since `CA', `CAN', and `CAD' are acceptable representations of `Canada'.   

Table \ref{tab:countlvl} shows the number of synonym and inheritance FDs found at each level in the clinical data.   For each discovered OFD, we sample and compute the percentage of tuples containing syntactically non-equal values in the consequent.  These values represent either synonyms or values participating in an inheritance relationship.  Under FD based data cleaning, these tuples would be considered errors.  However, by using OFDs, these false positive errors are saved since they are not true errors.  Figure \ref{fig:ofdclean1} shows the percentage of synonym and inheritance values at each lattice level where an OFD was found.  Overall, we observe that a significantly large percentage of tuples are falsely considered as errors under a traditional FD based data cleaning model.  For example, at level 1, 75\% and 84\% of the values in synonym and inheritance OFDs, respectively, contain non-equal values.  Only after level 6, we see that the number of tuples containing equal values in the consequent comprise over half of the satisfying tuples in the OFD.  This is somewhat expected, since the dependency becomes more constrained with an increasing number of antecedent attributes.  By correctly recognizing these `erroneous' tuples as clean, we reduce the computational effort of existing data cleaning techniques, and the manual burden for users to decipher through these falsely categorized errors.  

\textbf{Experiment-9: Evaluation of Approximate OFDs.}
 Approximate OFDs can be used in data cleaning to identify potentially dirty data values, and recommend values (from the clean set of tuples) for data repair.  Similar to past work, we assume that the data is mostly clean and consistent.  Figure \ref{fig:ofdclean2} shows the number of discovered synonym and inheritance OFDs for values of $\kappa \geq 0.5$ over the clinical data.  As expected, we observe a moderate increase in the number of discovered dependencies as the support level decreases.  
 
 We examined a sample of the approximate OFDs at each $\kappa$ level, and make two observations.  First, data repairs for the `dirty' tuples, comprising at most 20\% and 10\% of the total number of tuples, respectively, at $\kappa = 0.8$ and $\kappa = 0.9$, were more easily determined than at lower $\kappa$ levels due to the increased support of satisfying tuples, since patterns of values occurred with higher frequency (using a frequency based repair model).  For example, in approximate synonym OFD [CC, DIAG] $\rightarrow_{syn}$ DRUG, we found that references to drug names fluctuated greatly depending on the country, the diagnosis, and whether the drug is referred to as a brand name or in its natural (biological) form.  For example, a medication commonly used to treat anemia is also used to treat cancer and kidney failure, and is referred to by at least four different names: in its natural form as `Erythropoietin', and synthetically as `Epoetin', `Epogen', `Procrit', and `Darbepoetin Alfa'.   Secondly, approximate OFDs at $\kappa = 0.5$ and $\kappa = 0.6$ appeared to suffer from the expected overfitting problem.  At these levels, due to many lower frequency tuple pattern values, it is not as clear as to how the dirty tuples should be repaired.  
 
 In summary, approximate OFDs serve as a new data quality rule to capture domain relationships that were not considered by existing data quality dependencies.  Our observations indicate that approximate OFDs with higher support contain more reliable values for repairing inconsistent, and potentially dirty values.  As next steps, we intend to explore how approximate OFDs can be incorporated into automated data cleaning techniques to provide richer semantics during the data cleaning process.
 
   
 %*********************************************
%OFD Data Cleaning
\textbf{\blue{Experiment-10: Effectiveness of Ontology and Data Repairs.}}\label{sec:repaireval}
\blue{Use two datasets to measure the repair accuracy (precision and recall) and runtime by varying the error rate of the datasets, and incompleteness rate of the ontology. Compare with HoloClean in data repair.}

\begin{figure}
\begin{minipage}[t]{0.24\textwidth}
\centering
\includegraphics[width=4.4cm]{./figures/acc-kiva-er.eps}
\vspace{-5mm}
\caption{data error rate vs. accuracy(Kiva).}
\label{fig:erkiva}
\end{minipage}%
\hspace{0in}
\begin{minipage}[t]{0.24\textwidth}
\centering
\includegraphics[width=4.4cm]{./figures/rt-kiva-er.eps}
\vspace{-5mm}
\caption{data error rate vs. run time(Kiva).}
\label{fig:ermed}
\end{minipage}
\end{figure}

\begin{figure}
\begin{minipage}[t]{0.24\textwidth}
\centering
\includegraphics[width=4.4cm]{./figures/acc-kiva-ont.eps}
\vspace{-5mm}
\caption{Impact of ontology incompleteness (Kiva).}
\label{fig:oikiva}
\end{minipage}%
\hspace{0in}
\begin{minipage}[t]{0.24\textwidth}
\centering
\includegraphics[width=4.4cm]{./figures/a.eps}
\vspace{-5mm}
\caption{Impact of ontology incompleteness (Med).}
\label{fig:oimed}
\end{minipage}
\end{figure}

\textbf{\blue{Experiment-11: Effectiveness of selecting sense.}}
\blue{Use two datasets to measure the accuracy of selecting senses and the runtime.}

\textbf{\blue{Experiment-12: Effectiveness of the beam size $b$ for ontology repair.}}
\blue{Use two datasets to measure the runtime and the repair accuracy by varying the value of $b$.}

\begin{figure}
\begin{minipage}[t]{0.24\textwidth}
\centering
\includegraphics[width=4.4cm]{./figures/acc-kiva-beam.eps}
\vspace{-5mm}
\caption{beam size vs. repair accuracy (Kiva).}
\label{fig:bsacckiva}
\end{minipage}%
\hspace{0in}
\begin{minipage}[t]{0.24\textwidth}
\centering
\includegraphics[width=4.4cm]{./figures/rt-kiva-beam.eps}
\vspace{-5mm}
\caption{beam size vs. run time (Kiva).}
\label{fig:bsrtkiva}
\end{minipage}
\end{figure}

\textbf{\blue{Experiment-13: Scalability of OFDClean.}}
\blue{Use two datasets to measure the OFDClean's runtime and accuracy by varying the number of tuples, and the number of OFDs.}

\blue{\subsection{Case Study}}
\blue{Case study over clinical data: what violations that our approach identify, and what type of repairs we can apply.}






==> response.tex <==
\twocolumn
\pagenumbering{gobble}

\begin{center}\textbf{Response Letter} \\
\vspace{1em}
\textbf{Contextual Data Cleaning with Ontology Functional Dependencies}
\end{center}
\label{sec-response}
%\vspace{1.8ex}

We thank the reviewers for their constructive comments and clarifications to further improve this work.  We have revised the paper to address all comments.  %We  highlight changes in \reviseOne{magenta for Reviewer 1}.

%We coded the major comments with [M], and minor comments with [m].  \fei{Convention is usually weak points (major) as W and C for comments (less significant).  Alternatively M and m for major and minor.}
 \vspace{0.8ex}


%\lukasz{Macro for Lukasz to comment}
%\jarek{Macro for Jarek to comment}


%\noindent {\bf Associate-Editor} \\
%We include all authors from the original CIKM conference paper.  We have new student authors to reflect their work, and new contributions of this manuscript beyond the conference paper. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{1.8ex} \hrule \vspace{0.6ex} 

%\fei{Please insert line breaks to create spacing for improved readability.}

\noindent {\bf Reviewer 1} \\
Thank you for your detailed comments.  Please find our responses below, and changes in the revision in \reviseOne{blue}.  \\

\noindent{\bf W1:}  The semantics you pick for the attribute sets on the right hand side is fine, but when you define it, you should write $I\models\phi$ and $I\models X\rightarrow A$ instead of writing $\phi\models I$ and $X\rightarrow A\models I$. A minor point. 


\reviseOne{We corrected these typos in Section~\ref{sec:prelim}.  
} \\

%\fei{Jarek: I wrote the above, but upon reading the proof for Decomposition, it seems like you intended for the latter defn, i.e., all attributes in $Y$ share the same sense.  Can you please clarify?} 
%\jarek{We mean in our definition that X -> A for all A in Y, when considering right-hand-side as a set.}

\noindent{\bf W2:}  I've pointed out earlier on that synonyms also have an impact on the left-hand side of an OFD. Your reply is that consideration of that would lead to a larger search space. I don't understand this argument. Isn't it true that synonyms on the left-hand side simply give rise to larger equivalence classes? The search space is still the same. A restriction to your special case is perhaps fine, but certainly reduces the value of the contribution. 

%\fei{Jarek: I think we had a good reason for this, but don't recall, do you?}

\reviseOne{ 
\begin{table}[h!]
\scriptsize
\caption{Example table \label{tbl:responseTable}}
\vspace{-0.3cm}
\begin{tabular}{ | l | l | l | l | l |}
  \hline
  \textbf{tid} & \textbf{SYMP} & \textbf{MED} & \textbf{DISEASE} \\
  \hline
  $t_1$  & Headache & Cartia & Hyperpiesis \\
   \hline
  $t_2$   & Headache & Tiazac & Hypertension \\
  \hline
  $t_3$   & Headache & Bevyxxa  & Hypertension  \\
  \hline
  $t_4$  & Headache & Bevyxxa  & Hypertension \\
  \hline
   $t_5$  & Headache & Berixaban  & HHD  \\
  \hline
    $t_6$   & Headache & Tiazac & HHD \\
    \hline
    $t_7$ & Headache &  Aspirin \textcolor{blue}{(Tiazac)} & Hyperiesia  \\
  \hline
\end{tabular}
\end{table}
}

\reviseOne{
Consider an OFD $\phi_1:$ \kw{[SYMP]} $\rightarrow$ \kw{[MED]}, which indicates that for a given symptom, a unique medication is prescribed.  Table~\ref{tbl:responseTable} shows sample records, where MED values are interpreted under two senses according to the country and its regulatory agency for medications:  (1) US FDA: \\ $\{Cartia, Tiazac, Cardizem\}$; and (2) Israel Ministry of Health (MoH):  $\{Cartia, Aspirin, ASA\}$.  Validating $\phi_1$ over a relation requires evaluating each equivalence class, and checking for differing values in MED.}

\reviseOne{We now consider synonyms on the left-hand-side of an OFD $\phi_2:$ \kw{[MED]} $\rightarrow$ \kw{[DISEASE]}, where  DISEASE has synonyms $\{HHD, Hypertension\}$ under a given sense (we note that \emph{HHD} refers to \emph{Hypertensive Heart Disease}).  Validating $\phi_2$ under any sense, the equivalence classes do indeed become larger, i.e., instead of having five equivalence classes (no synonyms under any sense), we now have four classes (under the FDA sense, for example), namely $\{t_1, t_2, t_6\}, \{t_3, t_4\}$, $\{t_5\}$, $\{t_7\}$.  However, we must consider \emph{all} senses during validation, which requires \emph{evaluating a larger total number of equivalence classes.}
}

\reviseOne{The impact of multiple senses becomes more evident when repairing data values to satisfy OFDs.  Updating an attribute value to resolve an inconsistency under one sense can introduce errors w.r.t. another sense.  For example, updating $t_7$[MED] in Table~\ref{tbl:responseTable} from \emph{Aspirin} to \emph{Tiazac} corrects an error w.r.t. the US FDA sense (shown in blue), but introduces a new error under the MoH sense (\emph{Tiazac} does not exist under the MoH).  Furthermore, this leads to a new error in $t_7$[DISEASE] w.r.t. $\phi_2$ and tuples $\{t_2, t_6\}$, since $\{Hypertension$, $HHD\}$ and \emph{Hyperiesia} are not synonyms. 
}

\reviseOne{This example shows that updates to synonym values in the left-hand-side of an OFD induce new equivalence classes for each sense, that must each be evaluated during OFD validation. Interactions between OFDs (when attributes overlap between two or more OFDs) lead to an increased space of equivalence classes that must be evaluated, particularly when trying to minimize/maximize an objective function, e.g., minimizing the number of updates to achieve consistency.  Thus, in our work, we initially focus on synonyms in the right-hand-side of an OFD.
} \\


%\begin{enumerate}
%    \item Clearly explain difference between NFDs and OFDs and semantics, focusing on interpretations/senses; 
 %   \item Provide example (Jaguar has 3 possible senses); [Jarek]: Reviewers may say that the example with jaguar is artificial. I attached in Overleaf: see slides.pptx from our meeting were have different interpretations based on countries (with some nice diagrams). I feel like incorporating this might be more beneficial, so reviewers can better understand OFDs.
%    \item Discuss verification between the two; 
%    \item Acknowledge indeed larger equivalence classes.  However, for values with multiple senses, verifying multiple interpretations and interactions with other classes leads to a larger space of tuples to be considered.  Consequently, a larger space of repair values. 
%\end{enumerate}


\noindent{\bf W3:}  You are stating that "The axioms for strong and weak FDs [33], and the axioms for FDs with nulls as proposed by Lien [34], are not equivalent to those for OFDs, since the latter does not cover augmentation. I have appended a proof that shows that your axiom system for OFDs is equivalent to Lien's axiom system for NFDs. That means, in particular, that the implication problem of OFDs reduces to the implication problem of NFDs, or we can simply view OFDs as NFDs. This is further confirmed by Algorithm 1, which is the same as the algorithm for NFDs. 

\reviseOne{We agree with the reviewer that the axiom systems are equivalent for NFDs and OFDs. We revised the submission to include our own proof of equivalency of axioms in Section~\ref{sec:axioms}. As a consequence, after proving completness of axioms for OFDs, and showing the equivalency with NFDs,  we state that existing algorithms for NFDs can be used to determine whether an OFD holds and cite Theorem~\ref{thm:inference} for the  Algorithm~\cite{Lien82}.}

\reviseOne{We note that the definitions of OFDs and NFDs are not semantically equivalent, i.e., verifying that a single OFD holds does not imply a corresponding NFD holds (and vice versa); e.g, in Table~\ref{tab:cleanexample} an OFD [CC]  $\rightarrow$  [CTRY] holds, however, a corresponding NFD [CC]  $\rightarrow$  [CTRY] does \emph{not} hold. Also, while data verification for FDs and NFDs can be done on pairs of tuples, for OFDs it has to be performed on an entire equivalence class over the  left-hand-side attributes. Following Table~\ref{tab:mVio}, although all pairs of $t[Y]$ values share a common class, (i.e., \{\emph{v,w}\}: \E{D}, \{\emph{v,z}\}: \E{C}, \{\emph{w,z}\}: \E{F}), the intersection of these three classes is empty. Hence, $ \{ t_{1}, t_{2} \} \models  \set{X} \rightarrow \set{Y}$, $ \{ t_{2}, t_{3} \} \models  \set{X} \rightarrow \set{Y}$ and $ \{ t_{1}, t_{3} \} \models \set{X} \rightarrow \set{Y}$, but $ \{ t_{1}, t_{2}, t_{3} \} \not \models \set{X} \rightarrow \set{Y}$.}

\reviseOne{Similar conclusions were reached for other classes of dependencies, such as FDs and \emph{pointwise order functional dependencies} (POFDs). While definitions of FDs and POFDs are semantically different, the introduced PODs axioms are equivalent to FD axioms, leading to the same inference~\cite{Wi2001}.  We added the above discussion to Section~\ref{sec:axioms}.}

The equivalence will require you to carefully revisit the comparison of your work against that of the research literature, and explain the novelty. This will also need to include a revised consideration of the discovery and repair problem. Ultimately, the equivalence says that the problems that are being studied appear to be simpler than how they are currently being presented. 

\reviseOne{Given the different semantics between OFDs and NFDs, our novel contributions are as follows: \\
\uline{(1) Discovery:}   While OFD and NFD discovery can be modeled via a set-containment lattice, OFD discovery must check, for each equivalence class, whether there exists a non-empty intersection of the corresponding senses.  This incurs increased complexity during verification based on the number of synonyms and senses available in the ontology.  \\
\uline{(2) Data Repair:}  Computing data repairs to achieve consistency w.r.t. OFDs requires finding a sense that minimizes a cost function, e.g., the number of updates to achieve consistency, where interactions between OFDs and finding the best sense both incur additional challenges beyond NFDs.  Our greedy-based repair algorithm selects a sense that minimizes the number of data updates for a single OFD,  given $k$ ontology repairs.  This requires finding a sense, among all candidate senses, for each equivalence class.  In contrast, NFD verification is done over pairwise tuples, and NFDs do not consider multiple interpretations of their right-side values.  We further refine this initial sense selection (for each equivalence class) to consider interactions (overlapping attributes) among multiple OFDs.  Given that data updates w.r.t. one OFD can cause errors w.r.t. another OFD, our repair algorithm prioritizes updates to values that resolve  the largest number of errors to achieve consistency, and to avoid exhaustively enumerating all sense to equivalence class assignments.  We update the related work accordingly (Section~\ref{sec:rw}).
%[Fei, Jarek, Lukasz] Expend on the discussion above to answer second part of the question. Build around data verification being different leading to different discovery / repair, and make an argument about lattice (suggested by Lukasz)
} \\



%\fei{Jarek/Lukasz: can you please confirm (above) and verify the axioms equivalency question?}

\noindent{\bf W4:} The proof of the soundness and completeness of your axiomatization for OFDs needs to be part of the article, and it needs to be carefully examined. Your argument of justifying the use of a three-tuple relation does not seem to be valid to me. You would need to show (in mathematical terms) that general implication is equivalent to three-tuple implication.  

\reviseOne{We provide the proof of axioms completeness in the revised version (Section~\ref{sec:axioms}).  We incorporated the reviewer's suggestion and simplified the proof to include tableaux with two tuples. While the proof of completeness with three tuples was correct, the third tuple was redundant, thus, the core of the proof remains the same. Counter to data verification, which can be invalidated via three tuples for OFDs as described in [W3], logical inference for OFDs can be done via two tuples.} 

\vspace{1.8ex} \hrule \vspace{0.6ex} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\fei{Discuss results for: (a) reducing false positives with OFD discovery + approximate OFDs + error detection; (b) KIVA accuracy against HoloClean, and incompleteness rates?  }




==> sense_v0.tex <==

%**********************************************
\section{Sense Assignment}\label{sec:sense}

%As shown in Example~\ref{ex:motivating}, selecting different senses to interpret a given equivalence class leads to different ontology repairs and data repairs. In the global view, selecting an unsuitable sense for each equivalence class may impact the number of data repairs and the number of ontology repairs. In this case, the repair solution that we report may not be the $\tau$-constrained repair. 
%OFDs provide greater expressiveness over traditional dependencies via assignment of senses to equivalence classes.  
Given a set of senses for an ontology $S$, we want to compute $\lambda_x$ for each $x$ and $\phi \in \Sigma$ such that the repairs are Pareto-optimal, and each repair $(I',S')$ is minimal and $\tau$-constrained.  A naive approach  evaluates all candidate senses against all $x \in \Pi_X$, and would consider an exponential number of solutions, which is not feasible in practice.  

In this section, we introduce a greedy heuristic that will be shown to be experimentally effective.  We propose a two step approach.  First, we build an initial solution by greedily selecting the senses that minimize the number of repairs for each $x \in \Pi_X$ and for each $\phi: X \rightarrow_{syn} A$, leading to a local minimum.  Second, we consider the interactions among pairs of equivalence classes $x, x'$, where $x \in \Pi_X, x' \in \Pi_{X'}$ for $\phi, \phi' \in \Sigma$, respectively, by performing a local search to improve the initial solution w.r.t. minimizing the number of repairs, and is $\tau$-constrained.  We model the interactions among all $\phi, \phi' \in \Sigma$ that share a common consequent attribute by constructing a \emph{dependency graph}, where nodes represent equivalence classes and edges represent a shared consequent attribute. We traverse this dependency graph to refine the initial solution.  We evaluate the tradeoff between updating the initial sense assignment and a new assignment to $x$ by estimating the number of necessary data and ontology repairs to achieve alignment between $x, x'$.  We visit nodes $x'$ within a neighbourhood of the current node $x$ as defined via a distance function.  In this work, we use the \emph{Earth Mover's Distance (EMD)} to quantify the amount of work needed to transform the data distributions modeled in $x$ to the distribution represented in $x'$~\cite{Rubner00}.  We visit nodes $x'$ where the EMD values between $x, x'$ are largest, indicating regions with the greatest amount of conflict, while avoiding exhaustive enumeration of all candidate assignments.  We first describe our greedy  algorithm to generate an initial solution, followed by local neighbourhood refinement.


\eat{Question - We adopt a philosophy that if $\phi_1, \phi_2$ share a common consequent attribute, and share similar data distributions in their respective equivalence classes according to a threshold $\theta$, then we visit the node and check whether a refinement improves the utility  score.}  

\eat{
\begin{enumerate}
    \item neighbourhood relation: We consider visiting $x'$ in $sim(x,x') < \theta$ where sim is KL OR random order; and
    \item utility functions consider (i) minimizing the average (O,D) repairs among all classes or (ii) minimizing the maximum (O,D) + $\epsilon$ for each $x$.
\end{enumerate}
}

%Instead, we propose a two-step approach that first determines the senses that minimize the number of repairs for each single  $\phi: X \rightarrow_{syn} Y$, i.e., leading to a local minimum.   We then model the interactions among all $\phi_1, \phi_2 \in \Sigma$ that share a common consequent attribute $A$, by constructing a \emph{dependency graph}.  We traverse this graph to assign senses to each equivalence class $x$ (from the locally optimal set) for each $\phi$.  We adopt a philosophy that if $\phi_1, \phi_2$ share a common consequent attribute, and share similar data distributions in their respective equivalence classes, then they are assigned the same sense.  
%\fei{I have read and revised up to here, and will continue in Sec. 6.  I modified some of the section titles.}

\eat{Revise this section accordingly to the new algorithm: greedy initialization based on best sense assignment for a class (Sec. 5.1), followed by local search for a pair of classes that refines the sense assignment for the class pair if there are higher \textbf{utility scores} (Sec.5.2 + 5.3).  Need to ensure that there is a benefit towards local modification of already chosen senses.  Is this an opportunity to combine Sec. 5.2 and 5.3?}



\eat{As mentioned in Section~\ref{sec:framework}, our goal is to find a set of senses for all equivalence classes such that the repairs w.r.t. the selected senses is the \lit{minimal repair} (defined in Section~\ref{def:minimal}). However, traversing all the possible senses combinations for all the equivalence classes to find suitable senses is expensive.      To reach the goal, we first\eat{model the interactions between equivalence classes by using an undirected graph, and} select senses for each equivalence class locally by computing the required minimum number of data repair and ontology repair.  \fei{Does this not depend on a sense in the first place?  How do you choose the senses to consider initially?}     After that, since selecting a sense $\lambda$ for an equivalence class $x$ may impact the sense selection for other equivalence classes that interact with $x$, we propose a heuristic approach with a variant to select the senses by computing the similarity of the value distributions between each pairwise equivalence classes that overlap. The intuition is that the two equivalence classes with similar value distributions are likely to have the same sense.}

% We propose a heuristic approach to select senses for each equivalence class $x$ and the idea is to globally evaluate the number of tuples and distinct values are not covered by a given sense, in $x$ and the equivalence classes that intersect with $x$.  \fei{I didn't understand the last sentence.} The intuition behind this is that the minimal number of tuples and distinct values are not covered by a given sense leads to the minimal number of cell and ontology changes, respectively.

% \blue{Selecting a sense $\lambda$ for an equivalence class $x$ may impact the sense selection for other equivalence classes that interact with $x$. To find the best senses for all equivalence classes, \fei{We need to be more specific what "best" means for us.}  we first model the interactions between equivalence classes by using an undirected graph. In each iteration, we start with an equivalence class to select a sense, and then use the Breadth-first First Search (BFS) approach to traverses the graph and select sense for the other equivalence classes.  \fei{This is a good place to briefly justify why you are doing BFS, etc.} We consider all the unduplicated sense assignments in all the iterations as the final results.  \fei{I don't understand last sentence.}  In the following subsections, we first show the steps of how to select senses in each iteration, and then propose an optimization to our approach.}

% We propose a heuristic approach to select sense for each equivalence class $x$ and the idea is to globally evaluate the coverage of tuples and distinct values, in $x$ and the equivalence classes that intersect with $x$, by assuming the equation of the pairwise values that exist in $x$. Then we expand the selected equations (that have higher coverage) with one new value (exists in $x$) at a time to guide us narrow the senses search space. The intuition behind this is that the maximal coverage of $x$ leads to the minimal number of cell changes. Our approach consists of the following steps.

% Ideally for each equivalence class, the selected sense would lead to the minimal number of data and ontology repairs.   However, it is infeasible in practice if equivalence classes have overlap.

% Given an instance $I$, an ontology $S$ and a set of synonym OFDs $\Sigma$, we model the interactions between equivalence classes by using an undirected graph where the vertices represent the set of equivalence classes in $I$, an edge indicates that two connected vertices (equivalence classes) intersect with each other.



\subsection{Computing an Initial Assignment} \label{sec:greedy}
For $\phi: X \rightarrow_{syn} A$,  $x \in \Pi_X$, we want to compute $\lambda_x$, an initial sense assignment for each $x$.  To compute a minimal repair, we seek senses $\lambda_x$ \blue{containing as many values as possible (maximal overlap) with values in $x$}.  Let $t_u, v_u$ represent the number of distinct tuples and values, respectively, that are not covered by $\lambda_x$.   Let $\vec{r}_{\lambda_{x}} =  (t_u, v_u)$ be a vector representing the number of necessary tuples and values that must be updated in $x$ under sense $\lambda$ to satisfy $\phi$.  We seek a sense $\lambda'$ such that $\vec{r}_{\lambda_{x}'} \prec  \vec{r}_{\lambda_{x}}, \forall \lambda_x$. 
\eat{i.e., the repair $\vec{r}_{\lambda_{x}'}$ dominates $\vec{r}_{\lambda_{x}}$, for all senses. }

%to find senses that lead to a minimal number of data and ontology repairs.   We define a vector our goal is to find the initial sense $\lambda_x$ for $x$, where there is no other sense $\lambda' \in \Lambda_{\phi}$ such that $\lambda' \prec \lambda_x$.  $(\lambda'(\#tup), \lambda'(\#dist)) \prec (\lambda_x(\#tup), \lambda_x(\#dist))$.

% \fei{Note in Defn. 4, you are using symbols $X,Y, x$ again that refer to equiv. classes and attributes in the OFD, this can be confusing.}

The enumeration of all candidate senses to $x$ is practically inefficient.  We take a greedy approach that finds a $\lambda_x$ with maximal overlap with values in $x$.  We first construct an index of all senses containing each value $v \in x$, denoted by $sset(v)$.  For example, Figure~\ref{fig:ecg}(c) shows $sset(c_3) = \{\lambda_1, \lambda_4\}$.  To maximize the coverage of values, we naturally seek values with maximal frequency.  However, given that values in $x$ may contain errors, we seek an ordering of the values in $x$ that is robust to outliers.  The \emph{Median Absolute Deviation (MAD)} measure quantifies the variability of a sample, being more resilient to outliers than the standard deviation~\cite{rc1993}.  \eat{Since we assume that errors are normally small in number, the deviations from a small number of outliers are less relevant.}  Let $f(v)$ denote the frequency of value $v$. For a univariate dataset $\{f(v_1), f(v_2), \ldots f(v_n)\}$, MAD is defined as the median of the absolute deviations from the median, i.e., MAD($x$) = median$(|f(v_i) - f(\bar{(v)})|)$, where $f(\bar{(v)})$ is the median of all values in $x$.   We sort the values in $x$ according to their decreasing MAD scores.  \blue{We iteratively search for a sense $\lambda_x$ containing as many values as possible from $x$ with the highest MAD scores. \eat{, i.e., starting with $k = |MAD($x$)|$.}  For each value $v_i$, we compute the intersection of their respective $sset(v_i)$.  If there exists a non-empty intersection, the algorithm ends, and returns the senses in the intersection as an assignment for $x$, denoted as $potential\_set(x)$. We select the sense $\lambda_x$ containing the largest number of values in $x$.   Algorithm~\ref{pc:greedyassignment} provides the details.  }


%We iteratively search for a sense $\lambda_x$ that covers $k$ values, where $k = \{|MAD(x)|, \ldots , 1\}$, considering the top-$k$ values with the highest MAD scores.  For each value $v_i$ in the top-$k$, we compute the intersection of their respective $sset(v_i)$ set of senses.  If there exists a non-empty intersection, the algorithm ends, and returns the senses in the intersection as an assignment for $x$, denoted as $potential\_set(x)$. We select the sense $\lambda_x$ that covers the largest number of tuples. Algorithm~\ref{pc:greedyassignment} provides the details.  


%Algorithm~\ref{pc:greedyassignment} gives the details.  First, we index each value $v_{idx}$ exists in the ontology with the set of senses that contain $v_{idx}$, denoted by $sset(z)$ (Lines~\ref{line:indexstart}-\ref{line:indexend}). For example, as shown in Figure~\ref{fig:ecg}(c), $sset(c_3) = \{\lambda_1, \lambda_4\}$.    Secondly, we use a heuristic approach to find the sense $\lambda$ that occurs the most frequently across all the sense sets $sset(v'_{idx})$, where $v'_{idx}$ is the distinct value in $x$.   

%We first derive a ranking of the values in $x$, and compute the median absolute deviation (MAD)~\cite{rc1993} for each value in $x$ based on their occurrence frequency.  We sort the values in descending order, denoted by $MAD(x)$ (Lines~\ref{line:mad}-~\ref{line:candidate}).  We select the sense containing as many of the top values in $MAD(x)$.  Next, we iterate through $MAD(x)$ by considering a size $m$, $m = \{|MAD(x)|, |MAD(x) - 1|, ..., 1\}$. A naive approach is to traverse each $m$ combinations of the values in $MAD(x)$ and compute the sense set intersection of these values, to find the sense that has the maximal coverage of tuples in the data.  \fei{This seems to counter the top values statement?  Are you looking for max coverage or senses containing top values?  Hard to do both.}  However, it is infeasible in practice as the performance increases exponentially w.r.t. $|MAD(x)|$. Thus, instead of traversing each $m$ combinations of the values in $MAD(x)$, we only traverse each top-$m$ combinations. \fei{What does top-$m$ combinations mean?}  The algorithm stops when the set intersection result is not empty, and considers the result senses as the potential senses, denoted by $potential\_set(x)$ (Lines~\ref{line:m}-\ref{line:endwhile}). Lines~\ref{line:ppset} to \ref{line:lambdax} show that if there more than one sense in the set intersection result, we select sense $\lambda_x$ that has the maximum coverage over $x$ in terms of the number of tuples.  The algorithm returns $\lambda_x$ as the initial sense for $x$ in Line~\ref{line:initialresult}.

% MAD is a common tool to find outliers in one-dimensional data, while in our case, we use MAD to identify the values in $x$ that have high frequency based on the measurement in~\cite{LLKBL13} 

% \blue{To efficiently compute $\lambda_x$ for an equivalence class $x$ when there exists a large number of senses, we narrow the search space based on index techniques with the following steps: (1) index each value $v$ exists in the ontology with the set of senses that contain $v$, denoted by $sense\_set(v)$;  \fei{As shown in Figure ..}(2) we traverse the sense set $sense\_set(u)$ of each value $u \in x$, to find the sense $\lambda$ that has the highest frequency. \fei{What are we counting here for frequency?  For a given value $v \in x$, you get a list of all the senses containing $v$, then what are we counting as frequency?}  Then, $\lambda$ is a potential $\lambda_x$ for $x$ since the number of distinct values that are excluded by $\lambda$ is minimum \fei{I didn't understand the last statement, but I think you need to say something about why minimum matters towards reducing the number of repairs.  The current description is not clear enough to make that inference.}; (3) \fei{Given X, what are we trying to do now? Why is MAD useful?} we compute the median absolute deviation (MAD) for each value $u \in x$ based on its occurrence frequency in $x$. MAD is a common tool to find outliers in one-dimensional data, while in our case, we use MAD to identify the values in $x$ that have high frequency based on the measurement in~\cite{LLKBL13}; \fei{This last sentence is ambiguous. HOw is this related to finding outliers and our case? What are you trying to do with MAD?  Identify values in $x$ with high frequency to do what?  What is [27]?  You need to formally define MAD, and say why this choice is a good one for your objective.} (4) we compute the number of tuples are not captured by each sense that belongs to the sense sets of aforesaid values with high frequency in (3), \fei{I did not understand the last sentence. What do these tuples represent?  Why do we care about frequency again?  You use frequency a lot and is it the same count frequency in each case?  Try to explain what you are doing and justify it with reason.  You mention frequency a lot but need to explain why you are doing these steps. Why is finding the minimal best? } and consider the sense with the minimal number as a potential $\lambda_x$; (5) randomly select a sense from the set of potential senses for $x$.}\fei{Why is random good and not some other choice?}


%\begin{figure}[t]
%\centering
%      \includegraphics[width=7.5cm]{figures/ECG.pdf}
%     \vspace{-0.2cm}
%    \caption{Sense assignment}\label{fig:ecg}
%    \vspace{-0.5cm}
%\end{figure}


%***********************
\noindent\begin{minipage}[t]{.5\textwidth}
\begin{algorithm}[H]
\centering
\caption{Initial$\_$Assignment($x$, $S$, $\Lambda$)}\label{pc:greedyassignment}
  \footnotesize
%    \caption{Initial$\_$Assignment($x$, $S$, $\Lambda$)}\label{pc:greedyassignment}
    \begin{algorithmic}[1]
 %       \STATE $\Lambda$ be the set of all the senses of $S$ 
%        \STATE let $\lambda_x \in \Lambda$ be the initial sense is selected for $x$
        \STATE let $sset(v) \leftarrow \emptyset$ %be the sense set s.t. each sense $\lambda \in sset(v)$ contains $v$
        \FOR{each $\lambda \in \Lambda$} \label{line:indexstart}
            \FOR{each value $v \in \lambda$}
                \STATE $sset(v) \leftarrow sset(v) \bigcup \lambda$
            \ENDFOR
        \ENDFOR \label{line:indexend}
        % \STATE let $f(u)$ be the occurrence frequency of each value $u \in x$
%        \STATE compute MAD for values in $x$ w.r.t. their occurrence frequencies \label{line:mad}
%        \STATE let $MAD(x)$ be the set saves the values in $x$ w.r.t. their MAD in descending order \label{line:candidate}
        \STATE $k \leftarrow |MAD(x)|$ \label{line:m}
        \STATE $potential\_set(x) \leftarrow \emptyset$ %be the set saves all the potential selected senses
        \WHILE{$potential\_set(x)$ is $\emptyset$}
            \FOR{each top-$k$ $\{f(v_1), ..., f(v_n)\} \in MAD(x)$}
                \STATE $\Lambda' \leftarrow sset(v_1) \bigcap ... \bigcap sset(v_n) $
                \IF{$\Lambda' \neq \emptyset$}
                    \STATE $potential\_set(x) \leftarrow potential\_set(x) \bigcup \Lambda'$
                \ENDIF
            \ENDFOR
            \STATE $k \leftarrow k-1$ \label{line:endwhile}
        \ENDWHILE
        \FOR{each sense $\lambda \in potential\_set(x)$} \label{line:ppset}
            \STATE $cover(\lambda) \leftarrow$ the tuple coverage of $\lambda$ over $x$
        \ENDFOR 
        \STATE $\lambda_x \leftarrow \lambda \in cover(\lambda)$ with maximal tuple coverage \label{line:lambdax}
        \RETURN $\lambda_x$ \label{line:initialresult}
    \end{algorithmic}
%  \end{small}
\end{algorithm}
\end{minipage}%
\hfill
\begin{minipage}[t]{0.46\textwidth}
\begin{algorithm}[H]
    \centering
     \caption{Local$\_$Refinement($G$, $x$, $\Lambda$)}\label{pc:refine}
    \footnotesize
   \begin{algorithmic}[1]
%        \STATE let $G$ be the dependency graph
%        \STATE let $\{(x_1, x_2), w(x_1,x_2)\} \in EMD$, where $e_{w(x_1,x_2)}$ be EMD value between interacted equivalence classes $x_1$ and $x_2$
%        \STATE let $\{x, \sum e_{w(x)}\} \in \sum e_{w}$, where $\sum e_{w(x)}$ be the sum of EMD value between $x$ and its neighbors \fei{I don't understand the point of summing EMD values per node, and I think much of these two lines 3, 4 can be simplified using our notation in text, it is currently very hard to read and understand.  This is supposed to be pseudocode.}
%        \STATE let $\{x, \lambda_x\} \in \Lambda(I)$
        \STATE $u_1 \leftarrow $ BFS($G$) %be the start equivalence class to use BFS manner search graph $G$
        \FOR{each vertex $u_2$ connected to $u_1$}
            \IF{$w(u_1,u_2) > \theta$} \label{line:theta}
                \STATE compute $min\{$\cost $\}$ repair \label{line:mincost}
                \IF{sense reassignment for $u_2$ to $\lambda'$} 
                    \IF{$w'(u_1,u_2) < w(u_1,u_2)$}  %and $\sum e'_{w(v)} \leq \sum e_{w(v)}$}
                        \STATE $\Lambda \leftarrow \Lambda(I) \setminus \{u_2, \lambda\}$
                        \STATE $\Lambda \leftarrow \Lambda(I) \bigcup \{u_2, \lambda'\}$ \label{line:reassign}
                    \ENDIF
                \ENDIF
            \ENDIF
        \ENDFOR
        \STATE continue until all all $u_1$ visited \label{line:stop}  %\fei{Can this not be defined with a forall nodes in G?}
        \RETURN $\Lambda$ \label{line:refineresult}
    \end{algorithmic}
\end{algorithm}
\end{minipage}


\begin{example}\label{ex:ecg}
Figure~\ref{fig:ecg}(a) shows a data instance $I$ for two synonym OFDs $\phi_1: A \rightarrow C$ and $\phi_2: B \rightarrow C$.  Figure~\ref{fig:ecg}(b) shows seven senses and the corresponding synonym values for each sense.  Let $\lambda_{x_3}$ represent equivalence class $x_3 = \Pi_{B=b_2}$. Figure~\ref{fig:ecg}(c)) shows the index of senses for each value for all $x$.  We compute the MAD for values in $x_3$, i.e.,  $c_1 - c_4$, and determine that the ranked ordering is $\{c_4, c_2, c_1, c_3\}$.  We intersect the senses in $sset(c_2)$ and $sset(c_4)$, resulting in $\lambda_2$ as the initial sense for $x_3$. 
%(1) we index each distinct value exists in the data of attribute $C$ with a set of senses that contain the value (as shown in ; (2) based on the computation of MAD w.r.t. the occurrence frequency of each value in $x_3$ (i.e., $c_1 - c_4$), the frequencies of $c_2$ and $c_4$ are higher than the median.  \fei{You need to show this computation, what values are considered, and the final ranking of the values. } We apply set intersection between $sset(c_2)$ and $sset(c_4)$, and the result is $\lambda_2$. Then we consider $\lambda_2$ as initial sense for $x_3$. 
\end{example}

\begin{comment}
\begin{algorithm}[t]
  \begin{small}
    \caption{Initial$\_$Assignment($x$, $S$, $\Lambda$)}\label{pc:greedyassignment}
    \begin{algorithmic}[1]
 %       \STATE $\Lambda$ be the set of all the senses of $S$ 
%        \STATE let $\lambda_x \in \Lambda$ be the initial sense is selected for $x$
        \STATE let $sset(v) \leftarrow \emptyset$ %be the sense set s.t. each sense $\lambda \in sset(v)$ contains $v$
        \FOR{each $\lambda \in \Lambda$} \label{line:indexstart}
            \FOR{each value $v \in \lambda$}
                \STATE $sset(v) \leftarrow sset(v) \bigcup \lambda$
            \ENDFOR
        \ENDFOR \label{line:indexend}
        % \STATE let $f(u)$ be the occurrence frequency of each value $u \in x$
%        \STATE compute MAD for values in $x$ w.r.t. their occurrence frequencies \label{line:mad}
%        \STATE let $MAD(x)$ be the set saves the values in $x$ w.r.t. their MAD in descending order \label{line:candidate}
        \STATE $k \leftarrow |MAD(x)|$ \label{line:m}
        \STATE $potential\_set(x) \leftarrow \emptyset$ %be the set saves all the potential selected senses
        \WHILE{$potential\_set(x)$ is $\emptyset$}
            \FOR{each top-$k$ $\{f(v_1), ..., f(v_n)\} \in MAD(x)$}
                \STATE $\Lambda' \leftarrow sset(v_1) \bigcap ... \bigcap sset(v_n) $
                \IF{$\Lambda' \neq \emptyset$}
                    \STATE $potential\_set(x) \leftarrow potential\_set(x) \bigcup \Lambda'$
                \ENDIF
            \ENDFOR
            \STATE $k \leftarrow k-1$ \label{line:endwhile}
        \ENDWHILE
        \FOR{each sense $\lambda \in potential\_set(x)$} \label{line:ppset}
            \STATE $cover(\lambda) \leftarrow$ the tuple coverage of $\lambda$ over $x$
        \ENDFOR 
        \STATE $\lambda_x \leftarrow \lambda \in cover(\lambda)$ with maximal tuple coverage \label{line:lambdax}
        \RETURN $\lambda_x$ \label{line:initialresult}
    \end{algorithmic}
  \end{small}
\end{algorithm}
\end{comment}
%-------------------------------------------------



% \blue{\begin{example}\label{ex:ecg}
% \fei{Please consolidate all the examples to the same running example theme. I will review all examples at the end.} 
% \eat{Consider two synonym OFDs $\phi_1: A \rightarrow C$ and $\phi_2: B \rightarrow C$ over table Figure~\ref{fig:ecg}(a).  Figure~\ref{fig:ecg}(b) shows the ontology with seven senses over attribute $C$, the values in each sense are synonyms. Based on the definition in Section~\ref{sec:prelim}, there are four equivalence classes: $x_2 = \{t_1 - t_4\}$, $x_4 = \{t_5 - t_{10}\}$, $x_1 = \{t_1 - t_7\}$, $x_3 = \{t_8 - t_{10}\}$.} Continue with Example~\ref{ex:dominate}, Table~\ref{tab:uncover} shows the number of tuples and distinct values are not covered by each sense for each equivalence class.  The best senses (with the corresponding numbers of data and ontology repairs are marked as orange) for equivalence class $x_1$ are $\lambda_1$ and $\lambda_2$, since they dominate other senses based on the vector dominate definition. Similarly, the best senses for  $x_4$, $x_2$ and $x_3$ are $\lambda_4$, $\lambda_1$ and $\lambda_4$, respectively. 
% \end{example}}



% \begin{table}
% \scriptsize
% 	\centering
%     \begin{tabular}{ | c | c | c | c | c | c | c | c | c |}
%     \hline
%     \small
%      \multirow{2}{*}{Senses}& \multicolumn{2}{c|}{$x_1$}& \multicolumn{2}{c|}{$x_4$} & \multicolumn{2}{c|}{$x_2$}  & \multicolumn{2}{c|}{$x_3$}  \\
%     \cline{2-9}
%       & \#tup & \#dist & \#tup & \#dist & \#tup & \#dist & \#tup & \#dist   \\
%     \hline \hline
%     $\lambda_1$ & \orange{\textbf{3}} & \orange{\textbf{1}} & 3 & 2  & \orange{\textbf{1}} & \orange{\textbf{1}} & 1  & 1 \\
%     \hline
% 	$\lambda_2$ & \orange{\textbf{2}} & \orange{\textbf{2}} & 3 & 2  & 2 & 2 & 3  & 2 \\
% 	\hline
% 	$\lambda_3$ & 3 & 2 & 3 & 2  & 2 & 2 & 2  & 1 \\
% 	\hline
% 	$\lambda_4$ & 4 & 2 & \orange{\textbf{2}} & \orange{\textbf{1}}  & 2 & 2 & \orange{\textbf{0}}  & \orange{\textbf{0}} \\
% 	\hline
% 	$...$ & $...$ & $...$ & $...$ & $...$  & $...$ & $...$ & $...$  & $...$ \\
%     \hline
%     \end{tabular}
%     \vskip 0.1cm
% 	\caption{The number of tuples and distinct values are not covered by senses.}
% 	\label{tab:uncover}
% \end{table}



%-------------------------------------------------

% \blue{\subsection{Compute the Tuple Coverage} For each equivalence class $x$ of a synonym OFD $X \rightarrow_{syn} A$, we first assume the equation of each pairwise values that exist in the domain($A$) (the value domain of attribute $A$) of $x$, and compute the coverage of tuples in $x$. The tuples that in the coverage consist of two parts: (1) the tuples belong to the same intersection between $x$ and another equivalence class, and the values of attribute $A$ cover both values in the equation. We use Intersect($x$) to denote the number of tuples in this type of coverage; (2) the tuples belong to the same intersection between $x$ and another equivalence class, and the values of attribute $A$ cover one of the values in the equation. We use Non-Intersect($x$) to denote the number of tuples in this type of coverage. To be simple, we consider the coverage for a given equation of $x$ as the sum of Intersect($x$) and Non-Intersect($x$). In practice, however, we can emphasize either part by assigning a higher weight.} 

% \blue{\begin{example}\label{ex:coverage}
% Consider equivalence class $x_4 = \{t_3 - t_9\}$ of OFD $\phi_1: A \rightarrow C$, where domain($C$) = $\{c_2, c_3, c_4, c_5\}$. Equivalence class $x_4$ intersects with equivalence class $x_1$ and $x_3$. There are 6 equations of pairwise values, which are $c_2 = c_3$, $c_2 = c_4$, $c_2 = c_5$, $c_3 = c_4$, $c_3 = c_5$, $c_4 = c_5$. Consider the equation $c_2 = c_4$, which covers 4 tuples $t_3 - t_5, t_7$. We have Intersect($x$) $= 3$ since $c_2 = c_4$ covers 3 tuples ($t_3 - t_5$) in the intersection between $x_4$ and $x_1$, and both $c_2$ and $c_4$ belong to the intersection; Non-Intersect($x$) $= 1$ since $c_2 = c_4$ covers 1 tuple ($t_7$) in the intersection between $x_4$ and $x_3$, and only $c_2$ belongs to the intersection. Thus, the coverage of equation $c_2 = c_4$ in $x_4$ is $3+1=4$.
% \end{example} }

%\subsection{Utility Measures}

\subsection{Local Refinement} \label{sec:refinement}
%We have an initial assignment of senses to interpret the OFDs, i.e.,  $\lambda_x, \forall x \in \Pi_X, \forall \phi \in \Sigma$, where $\phi: X \rightarrow_{syn} A$. 
We discuss how we model interactions between $x, x'$, and address conflicting sense assignments that can lead to an increased number of repairs.
%The initial sense assignment, however, assumes $x$ occurs independently of any other $x' \in \Pi_{X'}$ for $\phi': X' \rightarrow_{syn} A'$.  We model the interactions between $x, x'$, and address conflicting sense assignments that may lead to an increased number of repairs.

\subsubsection{Modeling Interactions} \label{sec:interactions}
%\fei{Zheng: Pls. revise as per the red comments below, as I make my pass over 5.2 and 5.3.  I will not have time to review your changes again, so please double check your work, and this will be the version sent.}

Let $\Omega_{x,x'}(\lambda) = \{t | t \in (x \cap x')\}$ represent the set of overlapping tuples between two equivalence classes $x, x'$ from $\phi, \phi'$, respectively, interpreted w.r.t. sense $\lambda$.   To quantify conflict among $\phi, \phi'$, we need to interpret tuple values in the intersection of $x$ and $x'$ under the lens of the assigned sense. That is, conflicts may arise when there is a difference in the interpretation of the tuple values.  Specifically, let $x_{\lambda}$ represent the set of values in $x$ when interpreted under sense $\lambda$.  Given synonym relations, we assume that for each sense $\lambda$, there exists a canonical value representing  all  equivalent values in $\lambda$.  Let $D(x_{\lambda})$ represent the distribution of values in $x_{\lambda}$, where values in $x$ that are in $\lambda$ are represented by the canonical value.   If $x, x'$ are assigned the same sense $\lambda$, then for tuples in their intersection ($\Omega_{x,x'}(\lambda)$), they share the same distribution $D(\Omega_{x,x'}(\lambda))$.   When it is clear from the context, we use \Omegalambda to denote overlapping tuples in $x, x'$. 
%In general, this is not the case for $\lambda \neq \lambda'$.  

% \begin{figure}
% % \begin{minipage}[t]{0.24\textwidth}
% \centering
% \includegraphics[width=4.4cm]{./figures/DistOmega.pdf}
% \vspace{-5mm}
% \caption{Value distributions for $\Omega$ of $x_2$ and $x_3$ w.r.t. $\lambda_1$ and $\lambda_2$.}
% \label{fig:distomega}
% % \end{minipage}%
% % \hspace{0.1in}
% % \begin{minipage}[t]{0.24\textwidth}
% % \centering
% % \includegraphics[width=4.4cm]{./figures/.pdf}
% % \vspace{-5mm}
% % \caption{}
% % \label{fig:distomega2}
% % \end{minipage}
% \end{figure}

\begin{example}
Let $x_2 = \Pi_{A=a_1}$ and $x_3  =\Pi_{B=b_2}$, highlighted in blue and red, respectively, in Figure~\ref{fig:ecg}(a).  If we assign sense $\lambda_1$ to both classes, then the tuples in $\Omega_{x_2,x_3}(\lambda_1) = \{t_3, t_4, t_5, t_6\}$  share the same distribution, as shown via light grey bars in Figure~\ref{fig:ecg}(d), assuming that $c_2$ is the canonical value for $\lambda_1$. \eat{Assume $c_2$ is the canonical value for $\lambda_1$, then $\Omega$ of $x_2$ and $x_3$ shares the same distributions.  If we assign $\lambda_2$ to $x_2$ and $\lambda_1$ to $x_3$,  Figure~\ref{fig:ecg}(d) shows the two different distributions of values in $\Omega$.}
% Figure~\ref{fig:distomega1} shows that if $x_2$ and $x_3$ are assigned the same sense $\lambda_1$ or $\lambda_2$, the tuples in the interaction (i.e., $t_3 - t_6$) share the same distribution. While if we assign different senses for $x_2$ and $x_3$, the distributions of the tuples in the interaction are different.
% \fei{I'm a bit confused by your figure references, are they supposed to be Fig 4 and 5? See my revision in purple.}
\end{example}


The above example demonstrates that when two distributions $D$(\Omegalambda), $D(\Omega(\lambda'))$ are equivalent for $\lambda = \lambda'$, the \emph{outliers}, i.e., values not captured by $\lambda$, translate into necessary repairs to achieve consistency w.r.t. tuples in $\Omega$. In the above example, $c_4$ is the outlier, and we can resolve the inconsistency by updating $c_4$ to $c_2$ or by adding $c_4$ to $\lambda_1$.
\eat{In this case, the two interacted equivalence classes share the same outliers in $\Omega$. For example, as shown in Figure~\ref{fig:ecg}(d), consider assigning $\lambda_1$ to both $x_2$ and $x_3$. Assume $c_2$ is the canonical value for $\lambda_1$, fei: already said previously, redundant with the example.} In contrast, when $\lambda \neq \lambda'$, tuples in \Omegalambda and $\Omega(\lambda')$ will share different outliers.  For example, consider assigning $\lambda_1$ to $x_2$, and $\lambda_2$ to $x_3$.  The distributions for $\Omega_{x_2,x_3}(\lambda_1)$ and $\Omega_{x_2,x_3}(\lambda_2)$ are shown via the light grey bars and dark grey bars, respectively, in Figure~\ref{fig:ecg}(d).  Assuming $c_2$ is the canonical value for each sense, the outliers are $c_1$ and $c_3$ for $\lambda_2$, and $c_4$ for $\lambda_1$.  Let \rhoomega \ represent the set of outliers w.r.t. sense $\lambda$, i.e., the unique values in \Omegalambda \ not covered by  $\lambda$, \rhoomega = $\{v | v \in \Omega_{x,x'}(\lambda), v \not \in \lambda\}$.   We can resolve these outliers by: (1) updating the sense of $x$ from $\lambda$ to a new $\lambda'$; (2) adding outlier values \rhoomega \ to $S$; or (3) performing data repairs to update the values in \rhoomega \  to values $v \in \lambda$. 

For a class $x$, we seek a new sense assignment $\lambda'' \neq \lambda$ that includes one or more  values in \rhoomega.  This will cause an increase in the number of data or ontology repairs, as this will require sacrificing at least one value $t[A]$ for attribute $A$ that was covered under $\lambda$, $t \in \{x \setminus \Omega_{x,x'}(\lambda) \}$.  This penalty occurs since if there existed a better sense $\lambda''$ that covered all values in $\rho_{\lambda,x}$  then $\lambda''$ would have been assigned to $x$ during the initialization step (Section~\ref{sec:greedy}).  Hence, we can have $x$ keep $\lambda$ or be re-assigned to $\lambda''$.  However, we must consider the tradeoff of this re-assignment, by incurring a possible penalty (an increased number of repairs) according to the  non-overlapping tuples in $x$.  Alternatively, if $x$ keeps $\lambda$, then we must update the outlier values via data and/or ontology repairs.  

\textbf{Achieving Alignment.} 
To evaluate the tradeoff of a sense re-assignment, we define a cost function \cost \ that sums the number of data and ontology repairs to align  $D$(\Omegalambda), $D(\Omega(\lambda'))$.  For ontology repairs, to re-align $D$(\Omegalambda), $D(\Omega(\lambda'))$, we must add each outlier value in 
\rhoomega $\cup \rho_{\Omega, \lambda'}$ to ontology $S$, via senses $\lambda$ and $\lambda'$, i.e.,  \cost = |\rhoomega| + |$\rho_{\Omega, \lambda'}|$.  Since ontology repairs do not lead to further conflicts, they do incur a cost proportional to the number of values added to $\lambda$ and $S$.  For data repairs, we resolve differences by updating tuples $\{t| t \in$ \Omegalambda, $t[A] \in$ \rhoomega $\cup \rho_{\Omega, \lambda'}\}$ to a value from the 
candidate set $(\lambda \cap \lambda')$, which guarantees that the repaired value is covered by both senses.  We set \cost $=  |\mathcal{R}$(\Omegalambda)$| + |\mathcal{R}(\Omega(\lambda'))|$, where $\mathcal{R}$(\Omegalambda) = $\{t |t \in $\Omegalambda, $t[A] \in$ \rhoomega  $\}$, i.e., the number of tuples containing an outlier value.  We select the repair value from the candidate set that minimizes \cost.\   Lastly, we consider sense re-assignment that updates $\lambda$ to $\lambda'$ for $x$.  For $t \in x$, the delta cost, i.e., the number of data repairs to replace $\lambda$ with $\lambda'$ is \cost $=  |\mathcal{R}(x_{\lambda'})| - |\mathcal{R}(x_{\lambda})|$, where $\mathcal{R}(x_{\lambda}) = \{t |t \in x, t[A] \in \rho_{x, \lambda}\}$.  For a pair of classes $x, x'$, we consider all three repair options, and select the option that locally minimizes \cost. 

\begin{figure}[t]
\begin{minipage}[b]{0.3\linewidth}
\centering
\includegraphics[width=3.5cm]{./figures/DistLambda1.pdf}
\caption{$x_{2\lambda_1}$, $x_{3\lambda_1}$ distributions.}
\label{fig:distlambda1}
\end{minipage}
\hspace{-0.2cm}
\begin{minipage}[b]{0.3\linewidth}
\centering
\includegraphics[width=3.5cm]{./figures/DistLambda2.pdf}
\caption{$x_{2\lambda_2}$, $x_{3\lambda_2}$ distributions.}
\label{fig:distlambda2}
\end{minipage}
\hspace{-0.2cm}
\begin{minipage}[b]{0.3\linewidth}
\centering
\includegraphics[width=5.5cm]{./figures/DG.pdf}
\caption{Dependency graph.}
\label{fig:dg}
\end{minipage}
\end{figure}

%\begin{figure}
%\centering
%\includegraphics[width=9cm]{./figures/DG.pdf}
%\caption{Dependency graph. \eat{Update the weights and nodes to $w(u_1, u_2)$ and $u_i$. That is, do not use $x$ notation.}}
%\label{fig:dg}
%\end{figure}

\begin{example} \label{ex:alignment}
Figure~\ref{fig:distlambda1} and Figure~\ref{fig:distlambda2} shows the distribution of values in $x_2$ and $x_3$ with initial senses $\lambda_1$ and $\lambda_2$, respectively. 
%Consider equivalence classes $x_2$ and $x_3$ with initial senses $\lambda_1$ and $\lambda_2$, respectively. The value distribution for both equivalence classes w.r.t. $\lambda_1$ and $\lambda_2$ are shown in Figure~\ref{fig:distlambda1} and Figure~\ref{fig:distlambda2}, respectively. 
Let $c_2$ be the canonical value for $\lambda_1$ and $\lambda_2$. We then have: $\rho_{x_2, \lambda_1} = \{c_4, c_6\}$, $\rho_{x_3, \lambda_1} = \{c_4\}$, and  $\rho_{x_2, \lambda_2} = \{c_1, c_3, c_6\}$, $\rho_{x_3, \lambda_2} = \{c_1, c_3\}$. 
We evaluate ontology and data repair, and two sense assignment options: (i) we can add $c_4$ to $\lambda_1$, and add $c_1$ and $c_3$ to $\lambda_2$ to eliminate the conflict, leading to \cost = 3; (ii) we can update three tuples with values \{$c_4$, $c_1$ $c_3$\} to $c_2$; giving \cost = 3; (iii) we can assign $\lambda_1$ to $x_3$ (from $\lambda_2$), leading to $|\mathcal{R}(x_{3, {\lambda_1}})| - |\mathcal{R}(x_{3, \lambda_2})| = 3- 2 = 1$
%The new value distribution for $x_3$ w.r.t. $\lambda_1$ is shown as the dark bars in Figure~\ref{fig:distlambda1}. Since $|\mathcal{R}(x_3, \lambda_1)| = 3$, $|\mathcal{R}(x_3, \lambda_2)| = 2$ (i.e., update $c_1$ and $c_3$ to $c_2$), $\mathcal{C}ost() = 3 - 2 = 1$;
(iv) we can assign  $\lambda_2$ to $x_2$ where we update $\{c_1, c_3, c_6\}$ to $c_2$ giving \cost  = $|\mathcal{R}(x_{2, \lambda_2)}| - |\mathcal{R}(x_{2, \lambda_1)}| = 4-2 = 2$  Hence,  since \cost \ is minimal with option (iii), we re-assign $\lambda_1$ to class $x_3$. 

%The new value distribution for $x_2$ w.r.t. $\lambda_2$ is shown in light grey bars in Figure~\ref{fig:distlambda2}. Since $|\mathcal{R}(x_2, \lambda_2)| = 4$ (i.e., update $c_1, c_3, c_6$ to $c_2$), $|\mathcal{R}(x_2, \lambda_1)| = 2$ (i.e., update $c_4$ and $c_6$ to $c_2$), $\mathcal{C}ost() = 4 - 2 = 2$. Based on the above strategies, we will consider (iii) which re-assign sense $\lambda_1$ to $x_3$ since its cost $\mathcal{C}ost()$ is minimal.  
\end{example}

\begin{minipage}[t]{0.46\textwidth}
\begin{algorithm}[H]
    \centering
    \caption{Sense$\_$Assignment($I$, $\Sigma$, $S$, $\theta$)}\label{pc:algorithm}
    \footnotesize
    \begin{algorithmic}[1]
       \STATE  $\Lambda \leftarrow \{\emptyset, \emptyset\}$ 
 %       \STATE let $\{x, \lambda_x\} \in \Lambda(I)$, where $\lambda_x$ be the initial sense is selected for the equivalence class $x$ \fei{I don't think you need these two lines if they have already been defined in the text.  You just need to populate $\Lambda(I)$. What is $I$? }
        \FOR{each $\phi \in \Sigma$} \label{line:initialstart}
            \FOR{each $x \in \Pi_X(I)$}
                \FOR{each  $\lambda \in \Lambda$}
                    \STATE $\lambda_x \leftarrow$ Initial$\_$Assignment($x$, $S$, $\Lambda$)
                    \STATE $\Lambda \leftarrow \Lambda \bigcup \{x, \lambda_x\}$ \label{line:initialend}
                \ENDFOR
            \ENDFOR
        \ENDFOR
        \STATE  $G$ = CreateDepGraph($I, \Sigma, S, \Lambda$)  %($x$, $\Lambda(I)$, EMD), minimize words} Model the dependency graph $G$ \label{line:graph}
        % \STATE Let $EMD$ be the map that saves each pairwise equivalence classes and its EMD values
 %       \STATE Let $\{(x_1, x_2), e_{w(x_1,x_2)}\} \in EMD$ and $e_{w(x_1,x_2)}$ is maximal \label{line:maximal} \fei{Should we not sort the edges in DSC and just pop them off a stack? A while loop that pops as long as EMD > $\theta$?}
        % \STATE let $\{x, \sum e_{w(x)}\} \in \sum e_{w}$ be the total EMD between $x$ and its neighbors
        \STATE \textbf{sort}($G$, DSC)  Sort vertices in DSC order EMD edge weights
        
       \WHILE{($u_1$ = BFS($G$) and EMD($u_1$) > $\theta$)}
   %     \IF{$\sum e_{w(x_1)} > \sum e_{w(x_2)}$}  \fei{I don't understand this condition.}
    %        \STATE $x \leftarrow x_1$
    %    \ELSE
     %       \STATE $x \leftarrow x_2$ \label{line:startnode}
    %    \ENDIF
        \STATE $\Lambda \leftarrow$  Local$\_$Refinement($G$, $x$, $\Lambda$) \label{line:refine}
        \ENDWHILE
        \RETURN $\Lambda$ \label{line:finalresult}
    \end{algorithmic}
\end{algorithm}
\end{minipage}
\hfill
\noindent\begin{minipage}[t]{.5\textwidth}
\begin{algorithm}[H]
\centering
   \caption{Ontology$\_$Repair ($I$, $\Sigma$, $S$, $b$) }\label{pc:repont}
  \footnotesize
%    \caption{Initial$\_$Assignment($x$, $S$, $\Lambda$)}\label{pc:greedyassignment}
    \begin{algorithmic}[1]
        \STATE $Cand(S) \leftarrow \emptyset$ %be the set that contains all the candidate ontology repairs w.r.t. $\Sigma$
        \STATE $\mathcal{P(S)} \leftarrow \{\emptyset, ..., \emptyset \}$ %be the set that saves all Pareto-optimal ontology repair solutions
        \FOR{each $\phi \in \Sigma$}
            \FOR{each $x \in \Pi_X(I)$}
                \IF{$t_{e} \in x$ and $t_{e}[A] \not \in S$}
                    \STATE $Cand(S) \leftarrow Cand(S) \bigcup t_{e}[A]$
                \ENDIF
            \ENDFOR
        \ENDFOR
        % \FOR{each $c \in Cand(S)$}
        %     \STATE $S^{*} \leftarrow$ add $c$ to $S$
        % \ENDFOR
        % \STATE sort all $c \in Cand(S)$ w.r.t increasing $\delta_{opt}(S^{*}, I')$, where $\delta_{opt}(S^{*}, I') \leq \tau$
        % \STATE top-$b_1(S) \leftarrow \{\emptyset, ..., \emptyset \}$
        % \STATE top-$b_1(S) \leftarrow$ select top-$b$ of sorted $c$
        % \STATE insert top one element of top-$b_1(S)$ into $\mathcal{S}$
        \STATE $k \leftarrow 1$
        \STATE Generate $\mathcal{V}_k$ as clusters of size $k$, with values $v \in Cand(S)$
        \STATE $L_k \leftarrow \{v_k | v_k \in {\mathcal{V}_k} \}$
        \WHILE{$L_k \neq \emptyset$}
%            \FOR{each $v_k \in L_k$}  \fei{The below has to be reviewed.}
%                \STATE $S^{*} \leftarrow$ add $v_k$ to $S$ 
 %           \ENDFOR
 %           \STATE sort all $v_k \in Cand(S)$ w.r.t increasing $\delta_{opt}(S^{*}, I')$, where $\delta_{opt}(S^{*}, I') \leq \tau$
            \STATE $\delta(v_k)$ = compute data repairs for $v_k$ 
            \STATE $L_k \leftarrow$ top-$b$ nodes with smallest $\delta(v_k)$ to expand
            \STATE $v_k* = \{v_k |$ min $\delta(v_k)\}$
            \STATE $\mathcal{P(S)} \leftarrow (S', I')$ using $v_k*$ %insert top one element of top-$b_l(S)$ into $\mathcal{S}$
%            \FOR{each $v \in$ top-$b_l(s)$}
%                \FOR{each $c \in L_1 \setminus v$}
%                    \STATE $v \leftarrow v \bigcup c$
%                \ENDFOR
 %               \STATE $L_{l+1} \leftarrow L_{l+1} \bigcup v$
%            \ENDFOR
            \STATE $k \leftarrow k+1$
        \ENDWHILE
        \RETURN $\mathcal{P(S)}$
    \end{algorithmic}
%  \end{small}
\end{algorithm}
\end{minipage}%


% COMMENTED and side-by-side above
\eat{
\begin{algorithm}[t]
  \begin{small}
    \caption{Local$\_$Refinement($G$, $x$, $\Lambda$)}\label{pc:refine}
    \begin{algorithmic}[1]
%        \STATE let $G$ be the dependency graph
%        \STATE let $\{(x_1, x_2), w(x_1,x_2)\} \in EMD$, where $e_{w(x_1,x_2)}$ be EMD value between interacted equivalence classes $x_1$ and $x_2$
%        \STATE let $\{x, \sum e_{w(x)}\} \in \sum e_{w}$, where $\sum e_{w(x)}$ be the sum of EMD value between $x$ and its neighbors \fei{I don't understand the point of summing EMD values per node, and I think much of these two lines 3, 4 can be simplified using our notation in text, it is currently very hard to read and understand.  This is supposed to be pseudocode.}
%        \STATE let $\{x, \lambda_x\} \in \Lambda(I)$
        \STATE $u_1 \leftarrow $ BFS($G$) %be the start equivalence class to use BFS manner search graph $G$
        \FOR{each vertex $u_2$ connected to $u_1$}
            \IF{$w(u_1,u_2) > \theta$} \label{line:theta}
                \STATE compute $min\{$\cost $\}$ repair \label{line:mincost}
                \IF{sense reassignment for $u_2$ to $\lambda'$} 
                    \IF{$w'(u_1,u_2) < w(u_1,u_2)$}  %and $\sum e'_{w(v)} \leq \sum e_{w(v)}$}
                        \STATE $\Lambda \leftarrow \Lambda(I) \setminus \{u_2, \lambda\}$
                        \STATE $\Lambda \leftarrow \Lambda(I) \bigcup \{u_2, \lambda'\}$ \label{line:reassign}
                    \ENDIF
                \ENDIF
            \ENDIF
        \ENDFOR
        \STATE continue until all all $u_1$ visited \label{line:stop}  %\fei{Can this not be defined with a forall nodes in G?}
        \RETURN $\Lambda$ \label{line:refineresult}
    \end{algorithmic}
  \end{small}
\end{algorithm}
}


\subsubsection{Identifying Candidate Classes}
%Given $x, x'$, to minimize the difference between their value distributions, we must either: (1) update the sense for $x$; or (2) we perform leading to the minimal number of incurred data/ontology repairs.  
In this section, we discuss how to select pairs of classes $x, x'$ for refinement.  Visiting all pairs is not feasible, involving an exponential number of combinations.   For classes $x_{\lambda}, x'_{\lambda'}$, we quantify the deviation between their respective distributions, by measuring the amount of work needed to transform $D($\Omegalambda$)$ to $D(\Omega(\lambda'))$ (or vice-versa).  We quantify this work using the Earth Mover's Distance measure.  

\noindent \textbf{Earth Mover's Distance.} 
The Earth Mover's Distance, $EMD(P,Q)$ between two distributions $P, Q$ measures the minimal amount of work (cost) that must be performed to transform $P$ to another distribution $Q$ over a region $\mathcal{D}$~\cite{rtg2000}.  In our case, $\mathcal{D}$ refers to the attribute domain.

%cost that must be paid to transform one distribution into the other~\cite{rtg2000}. While in statistics, EMD is a widely measure of the distance between two probability distributions over a region $D$. Here, $D$ refers to the value domain of a given attribute. Intuitively, given two distributions $P$ and $Q$, we consider $P$ is differ from $Q$ if EMD between $P$ and $Q$ is greater than a threshold.

Let distributions $P, Q$ contain $m, n$ clusters, respectively, with $P=\{p_i,w_{p_i}\}_{i=1}^{m}, Q=\{q_j,w_{q_j}\}_{j=1}^{n}$
where $p_i, q_j$ are the cluster representatives, and $w_{p_i}, w_{q_j} > 0$ are the cluster weights.   Let $D = [d_{i,j}]$ be the ground distance between clusters $p_i$ and $q_j$. The goal is to find a flow $F=[f_{i,j}]$, with $f_{i,j}$ the flow between $p_i$ and $q_j$, that minimizes the overall cost. By solving the linear optimization problem, EMD is defined as the work normalized by the total flow: $EMD(P, Q) = \frac{\sum_{i=1}^{m}\sum_{j=1}^{n} f_{i,j} d_{i,j}}{\sum_{i=1}^{m}\sum_{j=1}^{n} f_{i,j}}$.
%Similarly, signature $Q=\{(q_1,w_{q_1}),(q_2,w_{q_2}),...,(q_n,w_{q_n})\}$ has $n$ clusters. 

The EMD can be computed by solving an instance of a transportation problem, using an algorithm to compute the minimum cost flow, e.g., the network simplex algorithm~\cite{james1997}. As a special case, if $\mathcal{D}$ is a one-dimensional array of bins, the EMD can be efficiently computed by scanning the array and keeping track of how much mass needs to be transported between consecutive bins, i.e., EMD $=\sum |EMD_i|$ where $EMD_{i+1} = p_i + EMD_i - q_i$ and $EMD_0 = 0$.

Let $P, Q$ represent distributions $D(\Omega_{x_1, x_2}(\lambda_1)), D(\Omega_{x_1, x_2}(\lambda_2))$, respectively.  We compute $EMD(P,Q)$ and check whether $EMD(P,Q) > \theta$, for a user-given threshold $\theta$.  Intuitively, if $P,Q$ are sufficiently different (according to $\theta$), then classes $x_1, x_2$ are candidates to consider sense re-assignment to re-align $P$ and $Q$.  Towards finding the sense with minimal repair, if the cost \cost \ of sense re-assignment and the EMD values are lower with the new sense, we proceed with sense re-assignment for $x_1, x_2$.  Otherwise, we keep the initial senses for $x_1$ and $x_2$.

\eat{For any pairwise equivalence classes $x_1$ and $x_2$ that interacted, we compute the value distributions $P$ and $Q$ for $x_1$ and $x_2$, respectively. Intuitively, if $x_1$ and $x_2$ have the similar value distributions, we can resolve the violations by applying fewer changes for both $x_1$ and $x_2$. Otherwise, if $P$ and $Q$ are different, i.e., $EMD(P,Q)$ is greater than a user defined threshold $\theta$, then it leads to more repairs. Based on the above intuition, we propose an algorithm to refine the sense assignment and the idea is that if $EMD(P,Q) > \theta$ and $x_1$ and $x_2$ are assigned different initial senses. We evaluate the cost $\mathcal{C}ost()$ of reassigning the sense of $x_1$ to $x_2$ (or vice verse). If $\mathcal{C}ost()$ of reassigning sense is minimal compare to that of applying data and ontology repairs, and the EMD decreases for $x_1$ and $x_2$ with new senses, we reassign the sense. Otherwise, we keep the initial senses for both $x_1$ and $x_2$.}


\textbf{Dependency Graph.} 
%We construct a dependency graph $G$ that models the interactions between equivalence classes $x, x'$. 
Let $G = (V,E)$ denote a \emph{dependency graph}, where each vertex $u \in V$ represents an equivalence class $x$, and an edge $e = (u_1, u_2) \in E$ exists when the corresponding classes $(x_1 \cap x_2) \neq \emptyset$.  We use the terms $u_1, u_2$ to represent classes when it is clear from the context.  Let $w(u_1,u_2)$ denote the weight of edge $e$, representing the EMD value between $u_1$ and $u_2$.  We visit nodes  in a breadth-first search manner, and select nodes $u_1$ with the largest EMD value by summing over all edges containing $u_1$.  This strategy prioritizes classes that require the largest amount of work.  For each visited edge, we check whether $w(u_1, u_2) > \theta$, and if so, check whether a sense re-assignment will reduce the weight, i.e., reduce the EMD value under the new sense.  If so, then the new sense re-aligns the two class distributions and incurs a minimal cost \cost.  The algorithm ends when all vertices have been visited.  Algorithm~\ref{pc:refine} provides  details. 


%\blue{Let $w(x, \sum x_i)$ be the sum of EMD value for each $x_i$ that is neighbor to $x$. \fei{Why do I need to compute this sum?  State its purpose.}  
%Algorithm~\ref{pc:refine} gives the algorithm pseudocode for sense refinement. For a given node $u$, we use breath first search (BFS) manner to traverse $G$ by visiting each neighbour $v$ such that $w(u,v) > \theta$.   We apply each alignment strategy mentioned in Section~\ref{sec:interactions} for $u$ and $v$ to compute $\mathcal{C}ost()$.  If the strategy whose cost $\mathcal{C}ost()$ is minimal, and it requires the sense reassignment (e.g., reassign the sense of $u$ to $v$), we compute $w'(u,v)$ and $w(v,\sum v_i)$ with the reassigned sense. We assign new sense to $v$ if $w'(u,v) < w(u,v)$ and $w'(v,\sum v_i) \leq w(v, \sum v_i)$ (Lines~\ref{line:mincost}-\ref{line:reassign}).  \fei{this is new, so state why you expect this condition to hold after reassignment, at least most of the time.}
%Otherwise, we do not refine the sense for $v$, i.e., keep $\lambda_{v}$ for $v$.  This is because if $e'_{w(v)} > e_{w(v)}$, even though reassigning the sense for $v$ reduces the number of repairs for $x$ and $v$ locally (i.e., $w'(x,v) < w(x,v)$), it causes more repairs globally for $v$ and its neighbors. \fei{I did not understand the last sentence.}  The algorithm stops until all the nodes are visited, and return the results (Lines~\ref{line:stop}-\ref{line:refineresult}).}




\eat{ %original code
\begin{algorithm}[t]
  \begin{small}
    \caption{Local$\_$Refinement($G$, $x$, $EMD$, $\sum e_w$ $\Lambda(I)$)}\label{pc:refine}
    \begin{algorithmic}[1]
        \STATE let $G$ be the dependency graph
        \STATE let $\{(x_1, x_2), w(x_1,x_2)\} \in EMD$, where $e_{w(x_1,x_2)}$ be EMD value between interacted equivalence classes $x_1$ and $x_2$
        \STATE let $\{x, \sum e_{w(x)}\} \in \sum e_{w}$, where $\sum e_{w(x)}$ be the sum of EMD value between $x$ and its neighbors \fei{I don't understand the point of summing EMD values per node, and I think much of these two lines 3, 4 can be simplified using our notation in text, it is currently very hard to read and understand.  This is supposed to be pseudocode.}
        \STATE let $\{x, \lambda_x\} \in \Lambda(I)$
        \STATE let $u$ be the start equivalence class to use BFS manner search graph $G$
        \FOR{each vertex $v$ connects to $u$}
            \IF{$e_{w(u,v)} > \theta$} \label{line:theta}
                \STATE compute $min\{\mathcal{C}ost()\}$ for three options \label{line:mincost}
                \IF{achieving $min\{\mathcal{C}ost()\}$ requires sense reassignment $\lambda_v'$ for $v$} 
                    \IF{$w'(u,v) < w(u,v)$ and $\sum e'_{w(v)} \leq \sum e_{w(v)}$}
                        \STATE $\Lambda(I) \leftarrow \Lambda(I) \setminus \{v, \lambda_v\}$
                        \STATE $\Lambda(I) \leftarrow \Lambda(I) \bigcup \{v, \lambda_v'\}$ \label{line:reassign}
                    \ENDIF
                \ENDIF
            \ENDIF
        \ENDFOR
        \STATE continue until all the nodes are visited \label{line:stop}  \fei{Can this not be defined with a forall nodes in G?}
        \RETURN $\Lambda(I)$ \label{line:refineresult}
    \end{algorithmic}
  \end{small}
\end{algorithm}

\begin{figure}
\centering
\includegraphics[width=9cm]{./figures/DG.pdf}
\vspace{-5mm}
\caption{Dependency graph. \fei{Update the weights and nodes to $w(u_1, u_2)$ and $u_i$. That is, do not use $x$ notation.}}
\label{fig:dg}
\end{figure}
}

\begin{example}
Figure~\ref{fig:dg}(a) shows the dependency graph corresponding to the equivalence classes in Figure~\ref{fig:ecg}(a), with EMD values as edge weights.  \eat{and the EMD values are shown on the edges.} Suppose $\theta = 10$, and we visit nodes in BFS order of $\{u_2, u_1, u_3, u_4, u_5\}$.  Starting at node $u_2$ (the blue node), we evaluate edge $(u_2, u_3)$ with weight 22. From Example~\ref{ex:alignment}, we update the sense for $u_3$ from $\lambda_2$ to $\lambda_1$ since the new weight $w'(u_3,u_2) < w(u_3,u_2) = 3 < 22$. \eat{ and $\sum e'_{w(x_3)} = 3 + 1 = 4 < e_{w(x_3)} = 22 + 7 = 29$.}  We next consider edge $(u_2, u_1)$ with $w(u_2,u_1) = 11$, with costs to update $u_1$ for data repair, ontology repair and sense reassignment as 1, 1 and 0, respectively.  However, after updating $u_1$ sense $\lambda_6$ to $\lambda_1$, $w'(u_2,u_1)$ does not decrease.  Thus, we do not refine the sense for $u_1$, and keep $\lambda_6$ as is.  \eat{You need to explain this second condition more in your text as I mentioned earlier because it creates questions about why you leave the senses as is, and why this is OK to do.  It also raises questions about EMD and the relationship to our operations to align the distributions.}   The algorithm then visits node $u_3$ and evaluates edge ($u_3$, $u_4$), where after sense reassignment to $\lambda_1$ for $u_3$, we have $w(u_3, u_4) = 1 < \theta$, and there is no further evaluation needed.  Lastly, we visit nodes $u_4, u_5$, where $w(u_4,u_5) = 4 < \theta$, and the algorithm terminates.    Figure~\ref{fig:dg}(b) shows the final sense assignments.
\end{example}


\subsection{Algorithm}
\label{sec:sensealg}
Algorithm~\ref{pc:algorithm} presents the details of our sense assignment algorithm.  We first compute an initial assignment for every equivalence class $x$.  We construct the dependency graph $G$, and compute the $EMD$ between overlapping classes ($u_1, u_2$) as edge weights.  We visit nodes in decreasing order of their $EMD$ values by summing over all corresponding edges.  For example, Figure~\ref{fig:ecg}(d) shows that we visit $u_2$ first since the EMD value of $u_2$ = 22 + 11 = 33, and of $u_3$ = 22 + 7 = 29.  Furthermore, we visit edge $(u_2, u_3)$ first since $w(u_2,u_3) = 22$ is the largest edge weight of $u_2$. We refine the sense for each equivalence class based on Algorithm~\ref{pc:refine}. Lastly, the algorithm returns the final sense assignment. 

\noindent \textbf{Complexity.} Computing an initial assignment takes time O($|\Pi_{X}| \cdot m$) to evaluate all $|\Pi_{X}|$ equivalence classes, and in the worst case, the total $m$ senses.  Traversing the dependency graph is in the same order as BFS, taking time $O((|V|+|E|) \cdot m)$, and to evaluate the candidate senses for each visited node.     


%first select the pairwise equivalence classes $x_1$ and $x_2$ such that $e_{w(x_1,x_2)}$ is maximal. We compute $\sum e_{x_1}$ and $\sum e_{x_2}$, and consider the one with higher value as the starting node (Lines~\ref{line:maximal}-\ref{line:startnode}). For example, as shown in Figure~\ref{fig:ecg}(d), we first select pairwise equivalence classes $x_2$ and $x_3$ since $e_{w(x_2,x_3)} = 22$ is maximal. Since $\sum e_{x_2}=22+11 = 33$ and $\sum e_{x_3}=22+7 = 29$, we select $x_2$ as the start node.   We refine the sense for each equivalence class based on Algorithm~\ref{pc:refine} (Line~\ref{line:refine}). Finally, algorithm returns the results in Line~\ref{line:finalresult}. 


% \begin{algorithm}[t]
%   \begin{small}
%     \caption{Local$\_$Assignment ($I$, $\Sigma$, $S$) }\label{pc:singular}
%     \begin{algorithmic}[1]
%         \STATE let $\Lambda_l(I) \leftarrow \{\emptyset, \emptyset\}$ be the map that saves the initial sense selection for each equivalence class $x \in \Pi_X(I)$
%         % \STATE let set($\Lambda$) be the set of $\Lambda(I)$
%         \STATE let $\{x, \lambda(x)\} \in \Lambda(I)$, where $\lambda_x$ be the initial sense is selected for the equivalence class $x$
%         \FOR{each OFD: $X \rightarrow A \in \Sigma$}
%             \FOR{each equivalence class $x \in \Pi_X(I)$}
%                 \FOR{each sense $\lambda \in \Lambda$}
%                     \STATE compute the initial sense $\lambda_x$ for $x$
%                     \STATE $\Lambda_l(I) \leftarrow \Lambda_l(I) \bigcup \{x, \lambda_x\}$
%                 \ENDFOR
%             \ENDFOR
%         \ENDFOR
%         \RETURN $\Lambda_l(I)$
%     \end{algorithmic}
%   \end{small}
% \end{algorithm}

\eat{
\begin{algorithm}[t]
  \begin{small}
    \caption{Sense$\_$Assignment($I$, $\Sigma$, $S$, $\theta$)}\label{pc:algorithm}
    \begin{algorithmic}[1]
       \STATE  $\Lambda \leftarrow \{\emptyset, \emptyset\}$ 
 %       \STATE let $\{x, \lambda_x\} \in \Lambda(I)$, where $\lambda_x$ be the initial sense is selected for the equivalence class $x$ \fei{I don't think you need these two lines if they have already been defined in the text.  You just need to populate $\Lambda(I)$. What is $I$? }
        \FOR{each $\phi \in \Sigma$} \label{line:initialstart}
            \FOR{each $x \in \Pi_X(I)$}
                \FOR{each  $\lambda \in \Lambda$}
                    \STATE $\lambda_x \leftarrow$ Initial$\_$Assignment($x$, $S$, $\Lambda$)
                    \STATE $\Lambda \leftarrow \Lambda \bigcup \{x, \lambda_x\}$ \label{line:initialend}
                \ENDFOR
            \ENDFOR
        \ENDFOR
        \STATE  $G$ = CreateDepGraph($I, \Sigma, S, \Lambda$)  %($x$, $\Lambda(I)$, EMD), minimize words} Model the dependency graph $G$ \label{line:graph}
        % \STATE Let $EMD$ be the map that saves each pairwise equivalence classes and its EMD values
 %       \STATE Let $\{(x_1, x_2), e_{w(x_1,x_2)}\} \in EMD$ and $e_{w(x_1,x_2)}$ is maximal \label{line:maximal} \fei{Should we not sort the edges in DSC and just pop them off a stack? A while loop that pops as long as EMD > $\theta$?}
        % \STATE let $\{x, \sum e_{w(x)}\} \in \sum e_{w}$ be the total EMD between $x$ and its neighbors
        \STATE \textbf{sort}($G$, DSC)  Sort vertices in DSC order EMD edge weights
        
       \WHILE{($u_1$ = BFS($G$) and EMD($u_1$) > $\theta$)}
   %     \IF{$\sum e_{w(x_1)} > \sum e_{w(x_2)}$}  \fei{I don't understand this condition.}
    %        \STATE $x \leftarrow x_1$
    %    \ELSE
     %       \STATE $x \leftarrow x_2$ \label{line:startnode}
    %    \ENDIF
        \STATE $\Lambda \leftarrow$  Local$\_$Refinement($G$, $x$, $\Lambda$) \label{line:refine}
        \ENDWHILE
        \RETURN $\Lambda$ \label{line:finalresult}
    \end{algorithmic}
  \end{small}
\end{algorithm}
}
\eat{
\begin{algorithm}[t]
  \begin{small}
    \caption{Sense$\_$Assignment($I$, $\Sigma$, $S$, $\theta$)}\label{pc:algorithm}
    \begin{algorithmic}[1]
        \STATE let $\Lambda(I) \leftarrow \{\emptyset, \emptyset\}$ be the map that saves the sense selection for each equivalence class $x$. \fei{I think you need to reduce the text in the alg. block, simplify reading.}
        \STATE let $\{x, \lambda_x\} \in \Lambda(I)$, where $\lambda_x$ be the initial sense is selected for the equivalence class $x$ \fei{I don't think you need these two lines if they have already been defined in the text.  You just need to populate $\Lambda(I)$. What is $I$? }
        \FOR{each OFD: $X \rightarrow A \in \Sigma$} \label{line:initialstart}
            \FOR{each equivalence class $x \in \Pi_X(I)$}
                \FOR{each sense $\lambda \in \Lambda$}
                    \STATE $\lambda_x \leftarrow$ Greedy$\_$Assignment($x$, $S$, $\Lambda$)
                    \STATE $\Lambda(I) \leftarrow \Lambda(I) \bigcup \{x, \lambda_x\}$ \label{line:initialend}
                \ENDFOR
            \ENDFOR
        \ENDFOR
        \STATE \fei{$G$ = CreateDepGraph($x$, $\Lambda(I)$, EMD), minimize words} Model the dependency graph $G$ \label{line:graph}
        % \STATE Let $EMD$ be the map that saves each pairwise equivalence classes and its EMD values
        \STATE Let $\{(x_1, x_2), e_{w(x_1,x_2)}\} \in EMD$ and $e_{w(x_1,x_2)}$ is maximal \label{line:maximal} \fei{Should we not sort the edges in DSC and just pop them off a stack? A while loop that pops as long as EMD > $\theta$?}
        % \STATE let $\{x, \sum e_{w(x)}\} \in \sum e_{w}$ be the total EMD between $x$ and its neighbors
        \IF{$\sum e_{w(x_1)} > \sum e_{w(x_2)}$}  \fei{I don't understand this condition.}
            \STATE $x \leftarrow x_1$
        \ELSE
            \STATE $x \leftarrow x_2$ \label{line:startnode}
        \ENDIF
        \STATE $\Lambda(I) \leftarrow$  Local$\_$Refinement($G$, $x$, $EMD$, $\sum e_{w}$, $\Lambda(I)$) \label{line:refine}
        \RETURN $\Lambda(I)$ \label{line:finalresult}
    \end{algorithmic}
  \end{small}
\end{algorithm}
}

% \begin{algorithm}[t]
%   \begin{small}
%     \caption{Local$\_$Assignment ($I$, $\Sigma$, $S$, $EMD$, $\Lambda_l(I)$) }\label{pc:singular}
%     \begin{algorithmic}[1]
%         \STATE let $\Lambda_l(I) \leftarrow \{\emptyset, \emptyset\}$ be the map that saves the initial sense selection for each equivalence class $x \in \Pi_X(I)$
%         % \STATE let set($\Lambda$) be the set of $\Lambda(I)$
%         \STATE let $\{x, \lambda(x)\} \in \Lambda(I)$, where $\lambda_x$ be the initial sense is selected for the equivalence class $x$
%         \FOR{each OFD: $X \rightarrow A \in \Sigma$}
%             \FOR{each equivalence class $x \in \Pi_X(I)$}
%                 \FOR{each sense $\lambda \in \Lambda$}
%                     \STATE compute the initial sense $\lambda_x$ for $x$
%                     \STATE $\Lambda_l(I) \leftarrow \Lambda_l(I) \bigcup \{x, \lambda_x\}$
%                 \ENDFOR
%             \ENDFOR
%         \ENDFOR
%         \RETURN $\Lambda_l(I)$
%     \end{algorithmic}
%   \end{small}
% \end{algorithm}

% \blue{\subsection{OFD interactions}
% For each equivalence class $x$, selecting the best sense locally is often infeasible since it may impact the sense selection for other equivalence classes that interact with $x$. Thus, we propose an approach to compute the similarity of the value distributions between each pairwise equivalence classes that overlap, and heuristically select the same sense for them if their value distributions are similar. We use Kullback-Leibler divergence (KL divergence)~\cite{kl51} to compute the distribution similarity since it is a commonly used asymmetric measurement (i.e., $D_{KL}(P||Q) \neq D_{KL}(Q||P)$), which helps us order the equivalence classes to select the sense. }

% \blue{Algorithm~\ref{pc:efficient} outlines the steps of our approach. Let $D_{KL}$ denotes the map saves each pairwise equivalence classes that overlap, and the corresponding KL divergence which is not infinite. From lines 2 to 6, for the minimal KL divergence $D_{KL}(P(x_1)||P(x_2))$ in $D_{KL}$ (the corresponding equivalence classes for $P(x_1)$ and $P(x_2)$ are $x_1$ and $x_2$, respectively), if there is no sense selected for both $x_1$ and $x_2$, we select sense $\lambda_l(x_2)$ for both of them, and remove $D_{KL}(P(x_1)||P(x_2))$ from $D_{KL}$. The process is repeated until $D_{KL}$ is empty. Finally, we select the best local sense for each equivalence class that are not assigned a sense (lines 7 to 10), and return the final results in line 11.}


% \begin{algorithm}[t]
%   \begin{small}
%     \caption{Efficient$\_$Assignment($I$, $\Sigma$, $S$, $EMD$, $\Lambda_l(I)$)}\label{pc:efficient}
%     \begin{algorithmic}[1]
%         % \STATE let $\Lambda(I) \leftarrow \{\emptyset, \emptyset\}$ be the map that saves the sense selection for each equivalence class $x \in \Pi_X(I)$
%         \STATE Let $\Lambda(I) \leftarrow \{\emptyset, \emptyset\}$ be the map that saves the sense selection for each equivalence class $x$.
%         \WHILE{$D_{KL} \neq \emptyset$}
%             \STATE let $\{(x_1, x_2), D_{KL}(P(x_1)||P(x_2)\}$ $\in$ $D_{KL}$, where $D_{KL}(P(x_1)||P(x_2))$ is minimal
%             \IF{$\lambda(x_1) = \emptyset$ and $\lambda(x_2) = \emptyset$}
%                 \STATE $\Lambda(I) \leftarrow \Lambda(I) \bigcup \{x_1, \lambda_l(x_2)\} \bigcup \{x_2, \lambda_l(x_2)\}$
%             \ENDIF
%             \STATE $D_{KL} \leftarrow D_{KL} \setminus D_{KL}(P'||Q')$
%         \ENDWHILE
%         \FOR{each OFD: $X \rightarrow A \in \Sigma$}
%             \FOR{each equivalence class $x \in \Pi_X(I)$}
%                 \IF{$\lambda(x) = \emptyset$}
%                     \STATE $\Lambda(I) \leftarrow \Lambda(I) \bigcup \{x, \lambda_l(x)\}$
%                 \ENDIF
%             \ENDFOR
%         \ENDFOR
%         \RETURN $\Lambda(I)$
%     \end{algorithmic}
%   \end{small}
% \end{algorithm}





% \blue{\subsection{OFD Interactions}
% For each equivalence class $x$, selecting the best sense locally is often infeasible since it may impact the sense selection for other equivalence classes that interact with $x$. Thus, we propose a heuristic approach to select the senses by computing the similarity of the value distributions between each pairwise equivalence classes that overlap.  \fei{specifically, for overlapping OFDs} The idea is to heuristically select the same sense first if two overlapped equivalence classes have similar value distributions.  For each pairwise connected vertices, we measure the similarity of their probability distribution based on Kullback-Leibler divergence (KL divergence)~\cite{kl51}, which is saved in a set $D_{KL}$ if the divergence value is not infinite}

% \blue{Algorithm~\ref{pc:selectsense} outlines the steps of our approach. Given an instance $I$, a set of synonym OFDs $\Sigma$, an ontology $S$ and a set of senses $\Lambda$, we firstly compute the best sense locally for each equivalence class $x$, denoted by $\lambda_l(x)$, based on the approach introduced in Section~\ref{sec:local} (lines 4 to 7). Secondly, we model the interactions between equivalence classes by using an undirected graph, denoted by G, where the vertices represent the set of equivalence classes in $I$, an edge indicates that two connected vertices (equivalence classes) intersect with each other (lines 8).
% For each pairwise connected vertices, we measure the similarity of their probability distribution based on Kullback-Leibler divergence (KL divergence)~\cite{kl51}, which is saved in a set $D_{KL}$ if the divergence value is not infinite (lines 9 to 16). For any two probability distributions $P$ and $Q$, KL divergence (written as $D_{KL}(P||Q)$) measures how $P$ is different from $Q$. We use KL divergence because it is a commonly used asymmetric measurement (i.e., $D_{KL}(P||Q) \neq D_{KL}(Q||P)$), which helps us order the equivalence classes to select the sense. Lines 17 and 18 describe two strategies to assign the sense, which refer to Algorithm~\ref{pc:singular} and Algorithm~\ref{pc:multi}, respectively.}

% \blue{Algorithm~\ref{pc:singular} shows an efficient approach to assign the sense. In each iteration, for the minimal KL divergence $D_{KL}(P'||Q')$ in set $D_{KL}$ (the corresponding equivalence classes for $P'$ and $Q'$ are $x_1$ and $x_2$, respectively), if there is no sense selected for both $x_1$ and $x_2$, we select sense $\lambda_l(x_2)$ for both of them (lines 1 to 5).
% Finally, we select the best sense locally for each equivalence class that are not assigned a sense (lines 6 to 9), and return the final results in line 10.}  \fei{Is this my variation of the algorithm?  you assign 2 at a time without consideration of neighbours.}



%\blue{\begin{example} \label{ex:efficient}
%\fei{Zheng: update to show ...}
%Continue with Example~\ref{ex:ecg} and Figure~\ref{fig:ecg}(d) shows the interactions between equivalence classes. We compute the KL divergence of all pairwise connected equivalence classes if it is not infinite: $D_{KL}(x_1||x_2) = 0.109$, $D_{KL}(x_2||x_1) = 0.112$, $D_{KL}(x_3||x_4) = 0.462$. Firstly, we start with equivalence class $x_2$ since $D_{KL}(x_1||x_2)$ is the minimal one. We select the best sense $\lambda_1$ locally for $x_2$, and assign the same sense $\lambda_1$ to $x_1$. In the second iteration, for $D_{KL}(x_2||x_1) = 0.112$, since both $x_2$ and $x_1$ are already assigned senses, we skip the step and continue.  For $D_{KL}(x_3||x_4) = 0.462$, we select sense $\lambda_4$ locally for $x_4$ and assign the same sense $\lambda_4$ to $x_3$ as well.  \fei{Consolidate to the same running example theme. }
%\end{example}}

% \begin{algorithm}[t]
%   \begin{small}
%     \caption{Sense$\_$Assignment ($I$, $\Sigma$, $S$, $\Lambda(I)$) }\label{pc:singular}
%     \begin{algorithmic}[1]
%         \STATE let $\Lambda(I) \leftarrow \{\emptyset, \emptyset\}$ be the map that saves the sense selection for each equivalence class $x \in \Pi_X(I)$
%         \STATE let set($\Lambda$) be the set of $\Lambda(I)$
%         \STATE let $\{x, \lambda(x)\} \in \Lambda(I)$, where $\lambda(x)$ be the sense is selected for the equivalence class $x$
%         \FOR{each OFD: $X \rightarrow A \in \Sigma$}
%             \FOR{each equivalence class $x \in \Pi_X(I)$}
%                 \FOR{each sense $\lambda \in \Lambda$}
%                     \STATE compute the best sense $\lambda_l(x)$ locally for $x$
%                 \ENDFOR
%             \ENDFOR
%         \ENDFOR
%         \STATE let G be the undirected graph that models the interactions between equivalence classes
%         \STATE let $D_{KL} \leftarrow \emptyset$ be the set saves all the KL divergences
%         \FOR{each pairwise connected vertices $u, v \in G$}
%             \STATE let $P$ be the probability distribution for $u$
%             \STATE let $Q$ be the probability distribution for $v$
%             \IF{$D_{KL}(P||Q) \nrightarrow \infty$}
%                     \STATE $D_{KL} \leftarrow$ $D_{KL} \bigcup D_{KL}(P||Q)$
%             \ENDIF
%             \IF{$D_{KL}(Q||P) \nrightarrow \infty$}
%                     \STATE $D_{KL} \leftarrow$ $D_{KL} \bigcup D_{KL}(Q||P)$
%             \ENDIF
%         \ENDFOR
%         \STATE $\Lambda(I) \leftarrow$ Singular$\_$Assignment($D_{KL}$, $\Lambda(I)$, $G$) \textbf{or}
%         \STATE set($\Lambda$) $\leftarrow$ Multiple$\_$Assignment($D_{KL}$, $\Lambda(I)$, $G$)
%         % \FOR{the minimal element $D_{KL}(P'||Q') \in D_{KL}$}
%         %     \STATE let $x_1$ and $x_2$ be the corresponding equivalence classes whose probability distribution are $P'$ and $Q'$, respectively.
%         %     \IF{$\lambda(x_1) = \emptyset$ and $\lambda(x_2) = \emptyset$}
%         %         \STATE $\Lambda(I) \leftarrow \Lambda(I) \bigcup \{x_1, \lambda_l(x_2)\} \bigcup \{x_2, \lambda_l(x_2)\}$
%         %     \ENDIF
%         %     \STATE $D_{KL} \leftarrow D_{KL} \setminus D_{KL}(P'||Q')$
%         % \ENDFOR
%         % \FOR{each OFD: $X \rightarrow A \in \Sigma$}
%         %     \FOR{each equivalence class $x \in \Pi_X(I)$}
%         %         \IF{$\lambda(x) = \emptyset$}
%         %             \STATE $\Lambda(I) \leftarrow \Lambda(I) \bigcup \{x, \lambda_l(x)\}$
%         %         \ENDIF
%         %     \ENDFOR
%         % \ENDFOR
%         \RETURN $\Lambda(I)$ or set($\Lambda$)
%     \end{algorithmic}
%   \end{small}
% \end{algorithm}

% \begin{algorithm}[t]
%   \begin{small}
%     \caption{Singular$\_$Assignment($D_{KL}$, $\Lambda(I)$)}\label{pc:efficient}
%     \begin{algorithmic}[1]
%         \STATE let $\Lambda(I) \leftarrow \{\emptyset, \emptyset\}$ be the map that saves the sense selection for each equivalence class $x \in \Pi_X(I)$
%         \FOR{the minimal element $D_{KL}(P'||Q') \in D_{KL}$}
%             \STATE let $x_1$ and $x_2$ be the corresponding equivalence classes whose probability distribution are $P'$ and $Q'$, respectively
%             \IF{$\lambda(x_1) = \emptyset$ and $\lambda(x_2) = \emptyset$}
%                 \STATE $\Lambda(I) \leftarrow \Lambda(I) \bigcup \{x_1, \lambda_l(x_2)\} \bigcup \{x_2, \lambda_l(x_2)\}$
%             \ENDIF
%             \STATE $D_{KL} \leftarrow D_{KL} \setminus D_{KL}(P'||Q')$
%         \ENDFOR
%         \FOR{each OFD: $X \rightarrow A \in \Sigma$}
%             \FOR{each equivalence class $x \in \Pi_X(I)$}
%                 \IF{$\lambda(x) = \emptyset$}
%                     \STATE $\Lambda(I) \leftarrow \Lambda(I) \bigcup \{x, \lambda_l(x)\}$
%                 \ENDIF
%             \ENDFOR
%         \ENDFOR
%         \RETURN $\Lambda(I)$
%     \end{algorithmic}
%   \end{small}
% \end{algorithm}



% \blue{\subsection{A Variant Approach}
% Algorithm~\ref{pc:efficient} is efficient since each equivalence class is visited exactly once when selecting the sense, and the algorithm returns one solution. However, it may ignore the potential sense selections which lead to minimal repair. For example, in Example~\ref{ex:efficient}, we select $\lambda_1$ for $x_1$ since $\lambda_1$ is the best sense for $x_2$ in local. While $\lambda_2$ is another best sense for $x_1$ in local, which is ignored. Besides that, Algorithm~\ref{pc:efficient} does not consider the interactions between equivalence classes.}

% \blue{To address the above issues, after computing KL divergence $D_{KL}(P||Q)$ for all pairwise connected equivalence classes, we propose a variant approach to consider each equivalence class $x$ whose corresponding probability distribution is $Q$ as the start to report a set of solutions. we model the interactions between equivalence classes by using an undirected graph, denoted by G, where the vertices represent the set of equivalence classes in $I$, an edge indicates that two connected vertices (equivalence classes) intersect with each other}

% \blue{To address the above issues, as shown in Algorithm~\ref{pc:multi}, after computing KL divergence $D_{KL}(P||Q)$ for all pairwise connected equivalence classes, we propose a variant approach to consider each equivalence class $x$ whose corresponding probability distribution is $Q$ as the start (lines 3 to 4) to report a set of solutions. From lines 5 to 16, the algorithm uses breath-first search (BFS) manner to select senses for the other equivalence classes start from $x$, which addresses the interaction issue between equivalence classes. To be more specific, given an equivalence class (vertex) $w$ with a selected sense $\lambda(w)$, the steps of assigning the sense to the vertex $v$ that connects to $w$ (lines 8 to 15) are as follows: (1) compute the sense candidates $Cand(v|w)$ for $v$ based on the constraint from $w$, which states that the values are not captured by $\lambda(w)$ should be excluded in $\lambda(v)$. Otherwise, there exists conflict when repair $v$ and $w$; (2) if the best local sense $\lambda_l(v)$ for $v$ is one of the sense candidates or the KL divergence from $w$ to $v$ is infinite, then we assign sense $\lambda_l(v)$ to $v$. Otherwise, assign sense $\lambda_l(w)$. Finally, the algorithm returns a set of solutions in line 17.} 
% The singular assignment algorithm is efficient since each equivalence class is visited exactly once when selecting the sense, and the algorithm returns one solution. However, it may ignore the potential sense selections which lead to minimal repair.  \fei{Can you give an example?} Thus, after computing and sorting (acceding order) KL divergence $D_{KL}(P||Q)$ for all pairwise connected equivalence classes, we propose a variant approach that considers each equivalence class $x$ whose corresponding probability distribution is $Q$ as the start to select sense first, \fei{I don't understand this last stmt.} and then use breath-first search (BFS) manner to select sense for the equivalence classes that connect with $x$. \fei{Why do you do this?} In each iteration, the steps are as follows: (1) select sense $\lambda_l(x)$ locally for $x$; (2) for each equivalence class $x'$ (connected with $x$) whose corresponding probability distribution $P'$, if $D_{KL}(P'||Q)$ is not infinite, we select the same sense $\lambda_l(x)$ for $x'$ as well. \fei{was this not done in the KL version?} Otherwise, we select sense $\lambda_l(x')$ locally for $x'$; (3) repeat the process according to the BFS manner until all the equivalence classes are visited.}  
% \cyan{tips: (1) consider more nodes as the starting node, which covers more solutions; (2) BFS manner helps address the interactions between equivalence classes.}


% \begin{algorithm}[t]
%   \begin{small}
%     \caption{Multiple$\_$Assignment($D_{KL}$, $\Lambda(I)$, $G$)\fei{Zheng to update}}\label{pc:multi}
%     \begin{algorithmic}[1]
%         %\STATE let G be the undirected graph that models the interactions between equivalence classes
%         \STATE let set($\Lambda$) be a set of sense assignments, i.e., $\Lambda(I) \in$ set($\Lambda$)
%         \STATE let set(root) be the set of equivalence classes (vertexes) to start searching
%         \FOR{each $\{(x_1,x_2), D_{KL}(P(x_1)||P(x_2))\} \in D_{KL}$}
%             % \STATE let $x$ be the corresponding equivalence class whose probability distribution is $Q$
%             \STATE set(root).add($x_2$)
%         \ENDFOR
%         \FOR{each equivalence class $x \in$ Set(root)}
%             \STATE start with $x$ to use BFS manner search graph $G$
%             \STATE let $w$ be a vertex with the selected sense $\lambda(w)$
%             \FOR{each vertex $v$ connects to $w$}
%                 \IF{$\lambda(v) = \emptyset$}
%                     \STATE compute $Cand(v|w)$ based on the constraints of $w$
%                     \STATE let $P(v)$ and $P(w)$ be the probability distributions for $v$ and $w$, respectively
%                     \IF{$\{(v, w), D_{KL}(P(v)||P(w))\} \notin D_{KL}$ or $\lambda_l(v) \in Cand(v|w)$}
%                         \STATE $\Lambda(I) \leftarrow \Lambda(I) \bigcup \{v, \lambda_l(v)\}$
%                     \ELSE
%                         \STATE $\Lambda(I) \leftarrow \Lambda(I) \bigcup \{v, \lambda(w)\}$
%                     \ENDIF
%                 \ENDIF
%             \ENDFOR
%             \STATE set($\Lambda$).add($\Lambda(I)$)
%         \ENDFOR
%         \RETURN set($\Lambda$)
%     \end{algorithmic}
%   \end{small}
% \end{algorithm}

% \begin{algorithm}[t]
%   \begin{small}
%     \caption{Multiple$\_$Assignment($D_{KL}$, $\Lambda(I)$, $G$)}\label{pc:multi}
%     \begin{algorithmic}[1]
%         \STATE let set(root) be the set of equivalence classes (vertexes) to start searching
%         \FOR{each element $D_{KL}(P||Q) \in D_{KL}$}
%             \STATE let $x$ be the corresponding equivalence class whose probability distribution is $Q$
%             \STATE set(root).add($x$)
%         \ENDFOR
%         \FOR{each equivalence class $x \ in$ Set(root)}
%             \FOR{each vertex $u$ in $G$}
%                 \STATE visited[$u$] $\leftarrow$ FALSE
%             \ENDFOR
%             \STATE visited[$x$] $\leftarrow$ TRUE
%             \STATE $\Lambda(I) \leftarrow \Lambda(I) \bigcup \{x, \lambda_l(x)\}$
%             \STATE let $q$ be queue saves the neighbors of the vertex is being visited
%             \STATE $q$.push($x$)
%             \WHILE{$q \neq \emptyset$}
%                 \STATE $w$ = $q$.pop()
%                 \FOR{each vertex $v$ connects to $w$}
%                     \IF{visited[$v$] is FALSE}
%                         \STATE compute $Cand(v, \Lambda(I))$ based on the constraints of $w$
%                         \STATE let $P(v)$ and $P(w)$ be the probability distributions for $v$ and $w$, respectively
%                         \IF{$\lambda_l(v) \in Cand(v, \Lambda(I))$ or $D_{KL}(P(v)||P(w)) \notin D_{KL}$}
%                             \STATE $\Lambda(I) \leftarrow \Lambda(I) \bigcup \{v, \lambda_l(v)\}$
%                         \ELSE
%                             \STATE $\Lambda(I) \leftarrow \Lambda(I) \bigcup \{v, \lambda_l(w)\}$
%                         \ENDIF
%                         \STATE $q$.push($v$)
%                     \ENDIF
%                 \ENDFOR
%                 \STATE visited[$w$] $\leftarrow$ TRUE
%             \ENDWHILE
%             \STATE set($\Lambda$).add($\Lambda(I)$)
%         \ENDFOR
%         \RETURN set($\Lambda$)
%     \end{algorithmic}
%   \end{small}
% \end{algorithm}

%\blue{\begin{example} \label{ex:multi}
%Based on the KL divergence results of all pairwise connected equivalence classes in Example~\ref{ex:efficient}, we consider $x_2$, $x_1$ and $x_4$ as the start, and apply BFS manner to select the senses for the other equivalence classes in each iteration. Consider the first iteration takes $x_2$ as the start, and we select sense $\lambda_1$ locally for it. Then based on BFS manner, we assign the sense for $x_1$ next. Since $c_4$ is not captured by $\lambda_1$ for $x_2$, the sense candidates for $x_1$ are $\{\lambda_1, \lambda_4, \lambda_5\}$. We select $lambda_1$ for $x_1$, because $\lambda_l(x_1) = lambda_1$. Similarly, we assign $\lambda_4$ to $x_2$ and $x_3$.       In the second iteration, we consider $x_1$ as the start, and our approach computes another set solution which assigns $\lambda_2$, $\lambda_2$, $\lambda_4$ and $\lambda_4$ for $x_1$, $x_2$, $x_4$ and $x_3$, respectively.      Similarly in the final iteration, we start selecting sense for $x_4$ and the results are the same with the previous iterations. Thus, we have two sets of sense assignment for $(x_2, x_1, x_4, x_1$, which are $(\lambda_1, \lambda_1, \lambda_4, \lambda_4)$ and $(\lambda_2, \lambda_2, \lambda_4, \lambda_4)$.
%\end{example}}

% \blue{In each iteration, we randomly start with an equivalence class to select a sense, and the equivalence class is not selected as the start before. Then, we use the BFS approach to traverses the graph and select sense for the other equivalence classes. }


% \blue{Based on the vector dominate definition mentioned in Section~\ref{sec:reptype1}, for a given equivalence class $x$, our goal is to select the sense that dominates \fei{I don't think a sense dominates} the others for the vector ($\#$tup, $\#$dist), which leads to the minimal number of data repair and ontology repair.
% However, selecting sense for an equivalence class $x$ may impact the sense selection for the other equivalence classes that interact with $x$. Thus, given an OFD $X \rightarrow_{syn} A$, for any two equivalence classes $x_1$ and $x_2$ that have interaction (i.e., there exists an edge between two nodes in the undirected graph), if our approach selected sense $\lambda_1$ for $x_1$, then the sense $\lambda_2$ for $x_2$ has to satisfy the following condition: for any value $v$ exists in both domain($\lambda_1$) and domain($A$) of $x_1 \cap x_2$, the value $v$ should exist in domain($\lambda_2$). }

% \fei{This requirement needs to be more precise.  Does the given OFD apply to $x_1$ or $x_2$?  What does it mean for $A$ to be in $x_1 \cap x_2$?  If a value exists in the intersection, does it not by default exist in the domain of each equivalence class?  I think you are trying to say that if a value overlaps between the two equivalence classes, then those values need to be covered by the sense?  If so, please explain why this is needed in your algorithm.}

% Thus, after selecting a sense $\lambda \in \Lambda$ of OFD $X \rightarrow_{syn} A$ for $x$, the values in the domain($A$) of $x$ have to be equal w.r.t. $S$ under sense $\lambda$. This constraint has to be transmitted to the equivalence classes that intersect with $x$ when select senses for them, and the constraint has to be satisfied. 

  

% For a given equivalence class $x$, we select the pairwise values that have the top$-m$ maximum coverage in $x$ with descending order. The idea of selecting the value of $m$ derives from setting the \lit{warm-up period} of the Secretary Problem~\cite{julia18}, and $m = \left \lfloor \frac{N}{e} \right \rfloor$. Here, $N$ is the number of pairwise values, and $e$ is the mathematical constant. For each selected pairwise values $(u, v)$, if there is a sense contains both $u$ and $v$, $(u, v)$ is expanded with one new value $w$ (in the domain($A$) of $x$) at a time, and compute the coverage with the new equation $u=v=w$ according to the previous step. The algorithm repeats until there is no sense contains all the values in the new equation. Finally, we select the sense that has the maximum coverage for $x$.

% \blue{To efficiently evaluate whether there exist senses contains all the values in a given equation, we index each value exists in the ontology with the set of senses that contain the value (Figure~\ref{fig:selectsense}(a)), and compute the set intersections for the values in the equation. The senses exist if the set intersection is not empty, otherwise, there is no sense exists.}

% \blue{\begin{example} \label{ex:selectsense}
% Continue with Example~\ref{ex:ecg} and we randomly start with equivalence class $x_1$. We select (1) $\lambda_1$ and (2) $\lambda_2$ for equivalence class $x_1$, since $\lambda_1$ and $\lambda_2$ dominate other senses based on the vector dominate definition. \fei{highlight these domination pairs in your example for readability.} If we select $\lambda_1$ for $x_1$ and based on BFS approach, we select sense for equivalence class $x_4$ and $x_2$ in the next step. For $x_4$, since value $c_2$ exists in both domain($\lambda_1$) and domain($C$) of $x_1 \cap x_4$, we consider $\lambda_1$, $\lambda_2$, $\lambda_4$ and $\lambda_5$ as the candidate senses since all of them contain value $c_1$. We select $\lambda_4$ for $x_4$ as $\lambda_4$ dominates the others. Similarly, we select $\lambda_1$ for $x_2$ and $\lambda_4$ for $x_3$. Thus, one senses selection result for $(x_1, x_4, x_2, x_3)$ is $(\lambda_1, \lambda_4, \lambda_1, \lambda_4)$. Similarly, if we select $\lambda_2$ for $x_1$, the result is $(\lambda_2, \lambda_2, \lambda_2, \lambda_4)$. Our approach keeps both results for the data and ontology repair in the further steps.
% \end{example}}

% \fei{This example needs to have a figure that shows each step of your decision making process.  Currently, it is not clear what criteria you use to select a sense for $x$, and then which node to visit next.  Each of these steps needs to be visually shown to make it easier to understand.  The current text is hard to follow unfortunately.  We can talk about how best to represent this more clearly with a figure.}

% $m =\left \lfloor \frac{6}{e} \right \rfloor = 2$, we order the pairwise values w.r.t. the coverage in $x_4$ as shown in Figure~\ref{fig:selectsense}(b). For $(c_2, c_4)$, we search the ontology indexes in Figure~\ref{fig:selectsense}(a) and sense $\lambda_2$ contains both $c_2$ and $c_4$. However, there is no sense contains all the values if $(c_2, c_4)$ expands with either $c_3$ or $c_5$. Then our approach stops and returns $\lambda_2$ as a potential solution and the coverage is 4. For $(c_2, c_3)$, there are two senses $\lambda_1$ and $\lambda_4$ contain both $c_2$ and $c_3$, and we can further expand $(c_2, c_3)$ with $c_5$ where all three values are covered by sense $\lambda_4$. Since there is no sense contains all the values if $(c_2, c_3, c_5)$ expands with $c_4$, the algorithm returns $\lambda_4$ as another potential solution and the coverage is 5. Finally, we select sense $\lambda_4$ for $x_4$ since it has the maximum coverage, which is 5.

% \blue{\subsection{Optimization} 
% Since selecting sense for an equivalence class $x_1$ will not impact the sense selection for equivalence class $x_2$ if $x_1$ does not interact with $x_2$ (i.e., $x_1 \cap x_2 = \emptyset$), we can reuse the sense selection results of any two equivalence class that has interaction if they are visited already. If there exists an edge between equivalence classes $x_1$ and $x_2$ in the undirected graph, we label $\lambda_1 \rightarrow \lambda_2$ on the edge if our approach selected sense $\lambda_1$ for $x_1$ first which was followed by selecting sense $\lambda_2$ for $x_2$. The result can be directly reused in the condition that equivalence classes $x_1$ and $x_2$ are revisited, and sense $\lambda_1$ is assigned to $x_1$.} 
% \fei{Isn't this assignment conditional on the prior visited nodes?  If I assign $\lambda_1$ to $x_1$, it may be due to requirements from prior visited nodes.  So does the traversed path of nodes prior to arriving to $x_1$ matter?}

% \fei{I would like to see an optimization that allows us to not consider all possible assignments exhaustively.  You did not say this in the text, but it seems implied by the BFS search. I'm also not sure that if you select a different starting point, that you will always end up with the same solution at the end.  I'd like to discuss variants of the assignment algorithm based on different choices for (1) starting node; and (2) graph traversal.}

% \blue{\begin{example} \label{ex:opt}
% In Example~\label{ex:selectsense}, we start with equivalence class $x_1$ and label the edges as shown in Figure~\ref{fig:ecg}(c). In the next iteration, assume we start with equivalence class $x_2$ and we select sense $\lambda_1$ since it dominates the others. Our approach traverses Table~\ref{tab:uncover} and selects $\lambda_1$ for equivalence class $x_1$. Since there exists a label $\lambda_1 \rightarrow \lambda_4$ between $x_1$ and $x_4$, and a label $\lambda_4 \rightarrow \lambda_4$ between $x_4$ and $x_3$. Thus, we directly select sense $\lambda_4$ for $x_4$ and $\lambda_4$ for $x_3$ without traversing the results in Table~\ref{tab:uncover}.
% \end{example}}
% \fei{What is the savings here?  Just a check for domination?}

% \blue{\subsection{Sense Transmit} After selecting a sense $\lambda \in \Lambda$ of OFD $X \rightarrow_{syn} A$ for a given equivalence class $x$, the values in the domain($A$) of $x$ have to be equal w.r.t. $S$. This constraint has to be transmitted to the equivalence classes that intersect with $x$, and the constraint has to be satisfied. Therefore, we have to consider the transmitted constraint to select the sense for those equivalence classes, as shown in the following example.}

% \blue{\begin{example}
% In Example~\ref{ex:selectsense}, we select sense $\lambda_4$ for equivalence class $x_4$, and delete the corresponding vertex (marked with purple color) in Figure~\ref{fig:ecg} (c). In the next step, we select sense for equivalence class $x_1$ whose degree is 1, and the transmit constraint from $x_4$ is $c_2 = c_5$. Thus, we only expand pairwise values $(c_2, c_5)$ for $x_1$. According to the previous step, there are two potential solutions, which are $(c_1, c_2, c_5)$ with the coverage is 4 and $(c_2, c_3, c_5)$ with the coverage is 2. Finally, we select sense $\lambda_5$ for $x_1$ by searching the ontology indexes.
% \end{example}}


% Given a candidate ontology repair, we require a sense to interpret the candidate value. Since an ontology $S$ may contain multiple senses, we evaluate these senses for each equivalence class $x$ of an OFD and select one sense such that the synonym class \emph{synonyms}$(E)$ (for synonym OFD) or the LCA tree (for inheritance OFD) in that sense has the maximal coverage over $x$. The intuition behind this is that the maximal coverage of $x$ leads to the minimal number of cell changes. The exhaustive approach finds the solution by traversing all the synonym classes (or LCA trees) of all senses, which is expensive and the complexity is $O(|x| \times K)$. Here, $|x|$ is the number of tuples in $x$ and $K$ is the number of synonyms in \emph{synonyms}$(E)$ (or LCA trees) over all the senses.



% We propose a solution by pre-computing the frequency of each distinct value in $x$. For example, consider an equivalence class of OFD: $X \rightarrow A$ shown in Figure~\ref{fig:selectsense}(a), we compute the frequency of each distinct value that exists in $x$ shown in Figure~\ref{fig:selectsense}(b). After that, we build the ternary search trees (TST)~\cite{tst98} based on the pre-computed frequencies, and find the synonym class $E$ (or LCA tree) that has the maximal coverage. A TST is a type of {\em trie}  where nodes are arranged in a manner similar to a binary search tree, but with up to three children. Each node in a TST is an object, and a sequence consists of multiple nodes along with the paths that connect them. The purpose of building the TST with sequences is to search the sequences efficiently if the sequences overlap with each other. 

% \noindent\textbf{Building TST for a synonym OFD.} For each equivalence class $x$ of a synonym OFD, each sense may contain multiple synonym classes. For example, Figure~\ref{fig:selectsense}(c) shows a synonym ontology with 4 senses over attribute $A$ for OFD: $X \rightarrow A$, the values in the same cycle (synonym class) of each sense are synonyms. We model each value in the synonym ontology as an object in the TST, and all the values in each synonym class as a sequence. The intuition behind this is that the synonym classes in different senses often have overlaps with each other (e.g., synonym class $\{a, b, c\}$ in $sense_2$ has overlap with $\{a, b\}$ in $sense_4$). We use the number on the right top corner of each object to show the coverage of the corresponding sequence over $x$.
% \begin{example}
% For example, the red lines in Figure~\ref{fig:selectsense}(d) shows the sequence of the synonym class $\{a, b, c\}$ in $sense_2$ (Figure~\ref{fig:selectsense}(c)), and the coverage is 4. Note that, by computing the coverage of synonym class $\{a, b, c\}$, the coverage of $\{a, b\}$ (i.e., 3) is also computed, which will directly return the coverage when we check the synonym class $\{a, b\}$ in $sense_4$.
% \end{example} 


% \noindent\blue{\textbf{Building TST for an inheritance OFD.} Similar to the synonym OFD, for each equivalence class, we consider an LCA tree (with a given $\theta$) of an inheritance ontology (under a specific sense) as the same as a synonym class of a synonym ontology. The difference is that for a synonym OFD, we search all the synonym classes to build TST, while for an inheritance OFD, we search all the LCA trees of the inheritance ontology to build TST. However, the complexity of these two cases is in the same order.}

% \blue{The complexity of computing the frequency of each distinct value in $x$ is $O(|x|)$, and the average complexity of building and searching TST is $O(\log M)$ ($M$ is the number of nodes in TST, which is in the same order with $K$). Thus, the total complexity for all equivalence classes is $\sum O(|x|+\log M)$, which is $O(N \times \log M$) in the worst case.}

% \begin{algorithm}[t]
%   \begin{small}
%     \caption{Selecting$\_$Senses ($I$, $\Sigma$, $S$, $k$) }\label{pc:selectsense}
%     \begin{algorithmic}[1]
%     \STATE
%     \end{algorithmic}
%   \end{small}
% \end{algorithm}

%*********************


